A magnetic massive star has experienced a stellar merger

Massive stars (those larger than 8 solar masses at formation) have radiative envelopes that cannot sustain a dynamo, the mechanism that produces magnetic fields in lower-mass stars. Despite this, approximately 7\% of massive stars have observed magnetic fields, the origin of which is debated. We used multi-epoch interferometric and spectroscopic observations to characterize HD 148937, a binary system of two massive stars. We found that only one star is magnetic and that it appears younger than its companion. The system properties and a surrounding bipolar nebula can be reproduced with a model in which two stars merged (in a previous triple system) to produce the magnetic massive star. Our results provide observational evidence that magnetic fields form in at least some massive stars through stellar mergers.

==> bib2.tex <==
% scibib.bib

% This is the .bib file used to compile the document "A simple Science
% template" (scifile.tex).  It is not intended as an example of how to
% set up your BibTeX file.

% ------------------------------------------------------------------------
% SAMPLE BIBLIOGRAPHY FILE
% ------------------------------------------------------------------------
% ------------------------------------------------------------------------
% SAMPLE BIBLIOGRAPHY FILE
% ------------------------------------------------------------------------
% scibib.bib

% This is the .bib file used to compile the document "A simple Science
% template" (scifile.tex).  It is not intended as an example of how to
% set up your BibTeX file.

% ------------------------------------------------------------------------
% SAMPLE BIBLIOGRAPHY FILE
% ------------------------------------------------------------------------

@ARTICLE{fabry2021,
       author = {Fabry, M. and {Crawford}, C. and {Mahy}, L. and {Marchant}, P.  and {Bouquin}, L.~B.  and {Sana}, H. },
        title = "{Mass discrepancy in 9 Sgr}",
      journal = {\aap},
     keywords = {stars: early-type, stars: individual (9 Sgr)},
         year = {subm.},
        month = Feb,
       volume = {},
          eid = {subm.},
        pages = (subm.)
        }
        
@ARTICLE{bodensteiner2021,
       author = {Bodensteiner, J. and {Sana}, H. and {Mahy}, L. and {Wang}, C.  and {Langer}, N.  and {De Mink}, S. },
        title = "{NGC 330: binarityr}",
      journal = {\aap},
     keywords = {stars: early-type, stars: individual (NGC330)},
         year = {subm.},
        month = Feb,
       volume = {},
          eid = (subm.),
        pages = (subm.)
        }
        
@ARTICLE{nazehd108,
       author = {{Naz{\'e}}, Y. and {Walborn}, N.~R. and {Martins}, F.},
        title = "{The mysterious Of?p class and the magnetic O-star {\ensuremath{\theta}}$^{1}$ Ori C: confronting observations}",
      journal = {\rmxaa},
     keywords = {stars: early-type, stars: individual (HD 108, HD 148937, HD 191612, {\ensuremath{\theta}} 1 Ori C), stars: variables: other, Astrophysics},
         year = 2008,
        month = oct,
       volume = {44},
        pages = {331-340},
archivePrefix = {arXiv},
       eprint = {0807.3496},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008RMxAA..44..331N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{powr,
       author = {{Sander}, A. and {Shenar}, T. and {Hainich}, R. and {G{\'\i}menez-Garc{\'\i}a}, A. and {Todt}, H. and {Hamann}, W. -R.},
        title = "{On the consistent treatment of the quasi-hydrostatic layers in hot star atmospheres}",
      journal = {\aap},
     keywords = {stars: early-type, stars: mass-loss, stars: winds, outflows, stars: atmospheres, stars: fundamental parameters, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = may,
       volume = {577},
          eid = {A13},
        pages = {A13},
          doi = {10.1051/0004-6361/201425356},
archivePrefix = {arXiv},
       eprint = {1503.01338},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...577A..13S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hirai,
       author = {{Hirai}, Ryosuke and {Podsiadlowski}, Philipp and {Owocki}, Stanley P. and {Schneider}, Fabian R.~N. and {Smith}, Nathan},
        title = "{Modelling Eta Carinae's Great Eruption and its surrounding nebula}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = nov,
          eid = {arXiv:2011.12434},
        pages = {arXiv:2011.12434},
archivePrefix = {arXiv},
       eprint = {2011.12434},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201112434H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Article{glebbeek08,
  Title                    = {{Evolution of stellar collision products in open clusters. II. A grid of low-mass collisions}},
  Author                   = {{Glebbeek}, E. and {Pols}, O.~R.},
  Journal                  = {\aap},
  Year                     = {2008},

  Month                    = sep,
  Pages                    = {1017-1025},
  Volume                   = {488},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2008A%26A...488.1017G},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1051/0004-6361:200809931},
  Eprint                   = {0806.0865},
  File                     = {Published version:2008A&A...488.1017G.pdf:PDF},
  Keywords                 = {stars: blue stragglers, stars: formation, methods: numerical, methods: N-body simulations, Galaxy: open clusters and associations: general}
}


@Article{glebbeek13,
  Title                    = {{Structure and evolution of high-mass stellar mergers}},
  Author                   = {{Glebbeek}, E. and {Gaburov}, E. and {Portegies Zwart}, S. and {Pols}, O.~R.},
  Journal                  = {\mnras},
  Year                     = {2013},

  Month                    = oct,
  Pages                    = {3497-3510},
  Volume                   = {434},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2013MNRAS.434.3497G},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1093/mnras/stt1268},
  Eprint                   = {1307.2445},
  File                     = {Published version:2013MNRAS.434.3497G.pdf:PDF},
  Keywords                 = {blue stragglers, stars: evolution, stars: general, stars: interior, globular clusters: general},
  Primaryclass             = {astro-ph.SR}
}


@Article{fab15,
  Title                    = {{Evolution of Mass Functions of Coeval Stars through Wind Mass Loss and Binary Interactions}},
  Author                   = {{Schneider}, F.~R.~N. and {Izzard}, R.~G. and {Langer}, N. and {de Mink}, S.~E.},
  Journal                  = {\apj},
  Year                     = {2015},

  Month                    = may,
  Pages                    = {20},
  Volume                   = {805},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015ApJ...805...20S},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/805/1/20},
  Eid                      = {20},
  Eprint                   = {1504.01735},
  File                     = {Published version:2015ApJ...805...20S.pdf:PDF},
  Keywords                 = {binaries: general, blue stragglers, stars: luminosity function, mass function, stars: mass-loss},
  Primaryclass             = {astro-ph.SR}
}


@Article{fab16,
  Title                    = {{Rejuvenation of stellar mergers and the origin of magnetic fields in massive stars}},
  Author                   = {{Schneider}, F.~R.~N. and {Podsiadlowski}, P. and {Langer}, N. and {Castro}, N. and {Fossati}, L.},
  Journal                  = {\mnras},
  Year                     = {2016},

  Month                    = apr,
  Pages                    = {2355-2365},
  Volume                   = {457},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2016MNRAS.457.2355S},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1093/mnras/stw148},
  Eprint                   = {1601.05084},
  File                     = {Published version:2016MNRAS.457.2355S.pdf:PDF},
  Keywords                 = {binaries: general, blue stragglers, stars: general, stars: individual: {$\tau$} Sco, stars: individual: HR 2949},
  Primaryclass             = {astro-ph.SR}
}


@ARTICLE{fab20,
       author = {{Schneider}, F.~R.~N. and {Ohlmann}, S.~T. and {Podsiadlowski}, Ph and {R{\"o}pke}, F.~K. and {Balbus}, S.~A. and {Pakmor}, R.},
        title = "{Long-term evolution of a magnetic massive merger product}",
      journal = {\mnras},
     keywords = {binaries: general, blue stragglers, stars: evolution, stars: individual: {\ensuremath{\tau}} Sco, stars: magnetic field, stars: massive, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = may,
       volume = {495},
       number = {3},
        pages = {2796-2812},
          doi = {10.1093/mnras/staa1326},
archivePrefix = {arXiv},
       eprint = {2005.05335},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.495.2796S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fabnat,
       author = {{Schneider}, Fabian R.~N. and {Ohlmann}, Sebastian T. and {Podsiadlowski}, Philipp and {R{\"o}pke}, Friedrich K. and {Balbus}, Steven A. and {Pakmor}, R{\"u}diger and {Springel}, Volker},
        title = "{Stellar mergers as the origin of magnetic massive stars}",
      journal = {\nat},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = oct,
       volume = {574},
       number = {7777},
        pages = {211-214},
          doi = {10.1038/s41586-019-1621-5},
archivePrefix = {arXiv},
       eprint = {1910.14058},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019Natur.574..211S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Article{morris06,
  Title                    = {{Anisotropic mass ejection in binary mergers}},
  Author                   = {{Morris}, T. and {Podsiadlowski}, P.},
  Journal                  = {\mnras},
  Year                     = {2006},

  Month                    = jan,
  Pages                    = {2-10},
  Volume                   = {365},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2006MNRAS.365....2M},
  Doi                      = {10.1111/j.1365-2966.2005.09645.x},
  Eprint                   = {astro-ph/0502288},
  File                     = {:2006MNRAS.365....2M.pdf:PDF},
  Keywords                 = {hydrodynamics, binaries: close, circumstellar matter, supernovae: individual: SN1987A}
}


@Article{macleod18,
  author        = {{MacLeod}, Morgan and {Ostriker}, Eve C. and {Stone}, James M.},
  title         = {{Bound Outflows, Unbound Ejecta, and the Shaping of Bipolar Remnants during Stellar Coalescence}},
  journal       = {\apj},
  year          = {2018},
  volume        = {868},
  number        = {2},
  pages         = {136},
  month         = {Dec},
  adsnote       = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl        = {https://ui.adsabs.harvard.edu/abs/2018ApJ...868..136M},
  archiveprefix = {arXiv},
  doi           = {10.3847/1538-4357/aae9eb},
  eid           = {136},
  eprint        = {1808.05950},
  file          = {:2018ApJ...868..136M.pdf:PDF},
  keywords      = {binaries: close, hydrodynamics, methods: numerical, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
  primaryclass  = {astro-ph.SR},
}


@ARTICLE{wade19,
       author = {{Wade}, G.~A. and {Smoker}, J.~V. and {Evans}, C.~J. and
         {Howarth}, I.~D. and {Barba}, R. and {Cox}, N.~L.~J. and {Morrell}, N. and
         {Naz{\'e}}, Y. and {Cami}, J. and {Farhang}, A. and {Walborn}, N.~R. and
         {Arias}, J. and {Gamen}, R.},
        title = "{A remarkable change of the spectrum of the magnetic Of?p star HD 148937 reveals evidence of an eccentric, high-mass binary}",
      journal = {\mnras},
     keywords = {binaries: spectroscopic, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {483},
       number = {2},
        pages = {2581-2591},
          doi = {10.1093/mnras/sty3304},
archivePrefix = {arXiv},
       eprint = {1811.11153},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483.2581W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{zin02,
       author = {{Zinnecker}, Hans},
        title = "{Formation of massive binaries}",
     keywords = {Astrophysics},
    booktitle = {A Massive Star Odyssey: From Main Sequence to Supernova},
         year = 2003,
       editor = {{van der Hucht}, Karel and {Herrero}, Artemio and {Esteban}, C{\'e}sar},
       volume = {212},
        month = jan,
        pages = {80},
archivePrefix = {arXiv},
       eprint = {astro-ph/0301078},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003IAUS..212...80Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moss,
       author = {{Moss}, D.},
        title = "{The survival of fossil magnetic fields during pre-main sequence evolution}",
      journal = {\aap},
     keywords = {magnetic fields, magnetohydrodynamics (MHD), stars: evolution, stars: chemically peculiar},
         year = 2003,
        month = may,
       volume = {403},
        pages = {693-697},
          doi = {10.1051/0004-6361:20030431},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...403..693M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{laurenthd,
       author = {{Mahy}, L. and {Hutsem{\'e}kers}, D. and {Naz{\'e}}, Y. and {Royer}, P. and
         {Lebouteiller}, V. and {Waelkens}, C.},
        title = "{Evolutionary status of the Of?p star HD 148937 and of its surrounding nebula NGC 6164/5}",
      journal = {\aap},
     keywords = {infrared: stars, stars: individual: HD 148937, ISM: individual objects: NGC 6164/5, stars: abundances, circumstellar matter, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {A61},
        pages = {A61},
          doi = {10.1051/0004-6361/201629585},
archivePrefix = {arXiv},
       eprint = {1611.07257},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599A..61M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{sana12,
       author = {{Sana}, H. and {Dunstall}, P.~R. and {H{\'e}nault-Brunet}, V. and {Walborn}, N.~R. and {de Koter}, A. and {de Mink}, S.~E. and {Dufton}, P.~L. and {Evans}, C.~J. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Taylor}, W.~D. and {Vink}, J.~S.},
        title = "{The VLT-FLAMES Tarantula Survey: Multiplicity and Dynamics of the Massive Stars in 30 Dor}",
    booktitle = {Proceedings of a Scientific Meeting in Honor of Anthony F. J. Moffat},
         year = 2012,
       editor = {{Drissen}, L. and {Robert}, C. and {St-Louis}, N. and {Moffat}, A.~F.~J.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {465},
        month = dec,
        pages = {284},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ASPC..465..284S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smash,
       author = {{Sana}, H. and {Le Bouquin}, J. -B. and {Lacour}, S. and
         {Berger}, J. -P. and {Duvert}, G. and {Gauchet}, L. and {Norris}, B. and
         {Olofsson}, J. and {Pickel}, D. and {Zins}, G. and {Absil}, O. and
         {de Koter}, A. and {Kratter}, K. and {Schnurr}, O. and {Zinnecker}, H.},
        title = "{Southern Massive Stars at High Angular Resolution: Observational Campaign and Companion Detection}",
      journal = {\apjs},
     keywords = {binaries: visual, stars: early-type, stars: imaging, surveys, techniques: high angular resolution, techniques: interferometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = nov,
       volume = {215},
       number = {1},
          eid = {15},
        pages = {15},
          doi = {10.1088/0067-0049/215/1/15},
archivePrefix = {arXiv},
       eprint = {1409.6304},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJS..215...15S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{walborn72,
       author = {{Walborn}, N.~R.},
        title = "{Spectral classification of OB stars in both hemispheres and the absolute-magnitude calibration.}",
      journal = {\aj},
         year = 1972,
        month = may,
       volume = {77},
        pages = {312-318},
          doi = {10.1086/111285},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972AJ.....77..312W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze08,
       author = {{Naz{\'e}}, Ya{\"e}l and {Walborn}, Nolan R. and {Rauw}, Gregor and
         {Martins}, Fabrice and {Pollock}, A.~M.~T. and {Bond}, Howard E.},
        title = "{HD 148937: A Multiwavelength Study of the Third Galactic Member of the Of?p Class}",
      journal = {\aj},
     keywords = {stars: early-type, stars: individual: HD 148937, X-rays: individual: HD 148937, X-rays: stars, Astrophysics},
         year = 2008,
        month = may,
       volume = {135},
       number = {5},
        pages = {1946-1957},
          doi = {10.1088/0004-6256/135/5/1946},
archivePrefix = {arXiv},
       eprint = {0803.0605},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008AJ....135.1946N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze12,
       author = {{Naz{\'e}}, Ya{\"e}l and {Zhekov}, Svetozar A. and {Walborn}, Nolan R.},
        title = "{High-resolution X-Ray Spectroscopy of the Magnetic Of?p Star HD 148937}",
      journal = {\apj},
     keywords = {stars: early-type, stars: individual: HD148937, stars: massive, X-rays: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = feb,
       volume = {746},
       number = {2},
          eid = {142},
        pages = {142},
          doi = {10.1088/0004-637X/746/2/142},
archivePrefix = {arXiv},
       eprint = {1111.7186},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...746..142N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{conti,
       author = {{Conti}, Peter S. and {Alschuler}, William R.},
        title = "{Spectroscopic Studies of O-Type Stars. I. Classification and Absolute Magnitudes}",
      journal = {\apj},
         year = 1971,
        month = dec,
       volume = {170},
        pages = {325},
          doi = {10.1086/151218},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971ApJ...170..325C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mathys,
       author = {{Mathys}, G.},
        title = "{The upper main sequence of OB associations. I. Spectral types and lines of C and N of southern single-lined O stars.}",
      journal = {\aaps},
     keywords = {Abundance, Blue Stars, Carbon, Nitrogen, O Stars, Stellar Spectra, Astronomical Catalogs, Evolution, Spectral Line Width, Stellar Luminosity, Astrophysics},
         year = 1988,
        month = dec,
       volume = {76},
        pages = {427-444},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988A&AS...76..427M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martins05,
       author = {{Martins}, Lucimara P. and {Gonz{\'a}lez Delgado}, Rosa M. and {Leitherer}, Claus and {Cervi{\~n}o}, Miguel and {Hauschildt}, Peter},
        title = "{A high-resolution stellar library for evolutionary population synthesis}",
      journal = {\mnras},
     keywords = {stars: atmospheres, stars: evolution, Astrophysics},
         year = 2005,
        month = mar,
       volume = {358},
       number = {1},
        pages = {49-65},
          doi = {10.1111/j.1365-2966.2005.08703.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0501225},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.358...49M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wade11,
       author = {{Wade}, G.~A. and {Howarth}, I.~D. and {Townsend}, R.~H.~D. and {Grunhut}, J.~H. and {Shultz}, M. and {Bouret}, J. -C. and {Fullerton}, A. and {Marcolino}, W. and {Martins}, F. and {Naz{\'e}}, Y. and {Ud Doula}, A. and {Walborn}, N.~R. and {Donati}, J. -F.},
        title = "{Confirmation of the magnetic oblique rotator model for the Of?p star HD 191612}",
      journal = {\mnras},
     keywords = {stars: individual: HD 191612, stars: magnetic field, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = oct,
       volume = {416},
       number = {4},
        pages = {3160-3169},
          doi = {10.1111/j.1365-2966.2011.19265.x},
archivePrefix = {arXiv},
       eprint = {1106.3008},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.416.3160W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petit13,
       author = {{Petit}, V. and {Owocki}, S.~P. and {Wade}, G.~A. and {Cohen}, D.~H. and {Sundqvist}, J.~O. and {Gagn{\'e}}, M. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Oksala}, M.~E. and {Bohlender}, D.~A. and {Rivinius}, T. and {Henrichs}, H.~F. and {Alecian}, E. and {Townsend}, R.~H.~D. and {ud-Doula}, A. and {MiMeS Collaboration}},
        title = "{A magnetic confinement versus rotation classification of massive-star magnetospheres}",
      journal = {\mnras},
     keywords = {circumstellar matter, stars: early-type, stars: fundamental parameters, stars: magnetic fields, stars: mass-loss, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = feb,
       volume = {429},
       number = {1},
        pages = {398-422},
          doi = {10.1093/mnras/sts344},
archivePrefix = {arXiv},
       eprint = {1211.0282},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.429..398P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{flames,
       author = {{Pasquini}, L. and {Avila}, G. and {Blecha}, A. and {Cacciari}, C. and {Cayatte}, V. and {Colless}, M. and {Damiani}, F. and {de Propris}, R. and {Dekker}, H. and {di Marcantonio}, P. and {Farrell}, T. and {Gillingham}, P. and {Guinouard}, I. and {Hammer}, F. and {Kaufer}, A. and {Hill}, V. and {Marteaud}, M. and {Modigliani}, A. and {Mulas}, G. and {North}, P. and {Popovic}, D. and {Rossetti}, E. and {Royer}, F. and {Santin}, P. and {Schmutzer}, R. and {Simond}, G. and {Vola}, P. and {Waller}, L. and {Zoccali}, M.},
        title = "{Installation and commissioning of FLAMES, the VLT Multifibre Facility}",
      journal = {The Messenger},
     keywords = {Spectrographs, VLT},
         year = 2002,
        month = dec,
       volume = {110},
        pages = {1-9},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002Msngr.110....1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mp,
       author = {{Martins}, F. and {Plez}, B.},
        title = "{UBVJHK synthetic photometry of Galactic O stars}",
      journal = {\aap},
     keywords = {stars: fundamental parameters, stars: atmospheres, stars: early-type, Astrophysics},
         year = 2006,
        month = oct,
       volume = {457},
       number = {2},
        pages = {637-644},
          doi = {10.1051/0004-6361:20065753},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606587},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...457..637M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bonnsai,
       author = {{Schneider}, F.~R.~N. and {Langer}, N. and {de Koter}, A. and {Brott}, I. and {Izzard}, R.~G. and {Lau}, H.~H.~B.},
        title = "{Bonnsai: a Bayesian tool for comparing stars with stellar evolution models}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: statistical, stars: general, stars: fundamental parameters, stars: rotation, binaries: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = oct,
       volume = {570},
          eid = {A66},
        pages = {A66},
          doi = {10.1051/0004-6361/201424286},
archivePrefix = {arXiv},
       eprint = {1408.3409},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...570A..66S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sana11,
       author = {{Sana}, H. and {Le Bouquin}, J. -B. and {De Becker}, M. and {Berger}, J. -P. and {de Koter}, A. and {M{\'e}rand}, A.},
        title = "{The Non-thermal Radio Emitter HD 93250 Resolved by Long Baseline Interferometry}",
      journal = {\apjl},
     keywords = {radiation mechanisms: non-thermal, stars: early-type, stars: individual: HD93250, stars: massive, techniques: interferometric, X-rays: individual: HD93250, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = oct,
       volume = {740},
       number = {2},
          eid = {L43},
        pages = {L43},
          doi = {10.1088/2041-8205/740/2/L43},
archivePrefix = {arXiv},
       eprint = {1110.0831},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...740L..43S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sana17,
       author = {{Sana}, H. and {Ram{\'\i}rez-Tannus}, M.~C. and {de Koter}, A. and {Kaper}, L. and {Tramper}, F. and {Bik}, A.},
        title = "{A dearth of short-period massive binaries in the young massive star forming region M 17. Evidence for a large orbital separation at birth?}",
      journal = {\aap},
     keywords = {binaries: spectroscopic, stars: early-type, stars: formation, open clusters and associations: individual: M 17, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {L9},
        pages = {L9},
          doi = {10.1051/0004-6361/201630087},
archivePrefix = {arXiv},
       eprint = {1702.02153},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599L...9S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jb17,
       author = {{Le Bouquin}, J. -B. and {Sana}, H. and {Gosset}, E. and
         {De Becker}, M. and {Duvert}, G. and {Absil}, O. and {Anthonioz}, F. and
         {Berger}, J. -P. and {Ertel}, S. and {Grellmann}, R. and {Guieu}, S. and
         {Kervella}, P. and {Rabus}, M. and {Willson}, M.},
        title = "{Resolved astrometric orbits of ten O-type binaries}",
      journal = {\aap},
     keywords = {stars: massive, binaries: general, methods: observational, techniques: high angular resolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = may,
       volume = {601},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201629260},
archivePrefix = {arXiv},
       eprint = {1608.03525},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...601A..34L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jb17,
       author = {{Le Bouquin}, J. -B. and {Sana}, H. and {Gosset}, E. and {De Becker}, M. and {Duvert}, G. and {Absil}, O. and {Anthonioz}, F. and {Berger}, J. -P. and {Ertel}, S. and {Grellmann}, R. and {Guieu}, S. and {Kervella}, P. and {Rabus}, M. and {Willson}, M.},
        title = "{Resolved astrometric orbits of ten O-type binaries}",
      journal = {\aap},
     keywords = {stars: massive, binaries: general, methods: observational, techniques: high angular resolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = may,
       volume = {601},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201629260},
archivePrefix = {arXiv},
       eprint = {1608.03525},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...601A..34L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shenar2020,
       author = {{Shenar}, T. and {Bodensteiner}, J. and {Abdul-Masih}, M. and {Fabry}, M. and {Mahy}, L. and {Marchant}, P. and {Banyard}, G. and {Bowman}, D.~M. and {Dsilva}, K. and {Hawcroft}, C. and {Reggiani}, M. and {Sana}, H.},
        title = "{The ``hidden'' companion in LB-1 unveiled by spectral disentangling}",
      journal = {\aap},
     keywords = {stars: early-type, stars: emission-line, Be, binaries: spectroscopic, binaries: close, stars: individual: LS V+22 25, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {639},
          eid = {L6},
        pages = {L6},
          doi = {10.1051/0004-6361/202038275},
archivePrefix = {arXiv},
       eprint = {2004.12882},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...639L...6S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{banyard2022,
       author = {{Banyard}, G. and {Sana}, H. and {Mahy}, L. and {Bodensteiner}, J. and {Villase{\~n}or}, J.~I. and {Evans}, C.~J.},
        title = "{The observed multiplicity properties of B-type stars in the Galactic young open cluster NGC 6231}",
      journal = {\aap},
     keywords = {binaries: spectroscopic, stars: early-type, stars: massive, open clusters and associations: individual: NGC 6231, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = feb,
       volume = {658},
          eid = {A69},
        pages = {A69},
          doi = {10.1051/0004-6361/202141037},
archivePrefix = {arXiv},
       eprint = {2108.07814},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...658A..69B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{gravpipe,
       author = {{Lapeyrere}, V. and {Kervella}, P. and {Lacour}, S. and {Azouaoui}, N. and
         {Garcia-Dabo}, C.~E. and {Perrin}, G. and {Eisenhauer}, F. and
         {Perraut}, K. and {Straubmeier}, C. and {Amorim}, A. and {Brandner}, W.},
        title = "{GRAVITY data reduction software}",
    booktitle = {\procspie},
         year = 2014,
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9146},
        month = jul,
          eid = {91462D},
        pages = {91462D},
          doi = {10.1117/12.2056850},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SPIE.9146E..2DL},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze10,
       author = {{Naz{\'e}}, Y. and {Ud-Doula}, A. and {Spano}, M. and {Rauw}, G. and
         {De Becker}, M. and {Walborn}, N.~R.},
        title = "{New findings on the prototypical Of?p stars}",
      journal = {\aap},
     keywords = {X-rays: stars, stars: individual: HD 108, stars: individual: HD 148937, stars: individual: HD 191612, stars: emission-line, Be, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = sep,
       volume = {520},
          eid = {A59},
        pages = {A59},
          doi = {10.1051/0004-6361/201014333},
archivePrefix = {arXiv},
       eprint = {1006.2054},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...520A..59N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{georgy17,
       author = {{Georgy}, Cyril and {Meynet}, Georges and {Ekstr{\"o}m}, Sylvia and
         {Wade}, Gregg A. and {Petit}, V{\'e}ronique and {Keszthelyi}, Zsolt and
         {Hirschi}, Raphael},
        title = "{Possible pair-instability supernovae at solar metallicity from magnetic stellar progenitors}",
      journal = {\aap},
     keywords = {stars: evolution, stars: magnetic field, stars: massive, stars: mass-loss, supernovae: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {L5},
        pages = {L5},
          doi = {10.1051/0004-6361/201730401},
archivePrefix = {arXiv},
       eprint = {1702.02340},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599L...5G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{edibles,
       author = {{Cox}, Nick L.~J. and {Cami}, Jan and {Farhang}, Amin and
         {Smoker}, Jonathan and {Monreal-Ibero}, Ana and {Lallement}, Rosine and
         {Sarre}, Peter J. and {Marshall}, Charlotte C.~M. and
         {Smith}, Keith T. and {Evans}, Christopher J. and {Royer}, Pierre and
         {Linnartz}, Harold and {Cordiner}, Martin A. and {Joblin}, Christine and
         {van Loon}, Jacco Th. and {Foing}, Bernard H. and {Bhatt}, Neil H. and
         {Bron}, Emeric and {Elyajouri}, Meriem and {de Koter}, Alex and
         {Ehrenfreund}, Pascale and {Javadi}, Atefeh and {Kaper}, Lex and
         {Khosroshadi}, Habib G. and {Laverick}, Mike and {Le Petit}, Franck and
         {Mulas}, Giacomo and {Roueff}, Evelyne and {Salama}, Farid and
         {Spaans}, Marco},
        title = "{The ESO Diffuse Interstellar Bands Large Exploration Survey (EDIBLES) . I. Project description, survey sample, and quality assessment}",
      journal = {\aap},
     keywords = {ISM: lines and bands, ISM: clouds, ISM: molecules, dust, extinction, stars: early-type, local insterstellar matter, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = oct,
       volume = {606},
          eid = {A76},
        pages = {A76},
          doi = {10.1051/0004-6361/201730912},
archivePrefix = {arXiv},
       eprint = {1708.01429},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...606A..76C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{langerrev,
       author = {{Langer}, N.},
        title = "{Presupernova Evolution of Massive Single and Binary Stars}",
      journal = {\araa},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = sep,
       volume = {50},
        pages = {107-164},
          doi = {10.1146/annurev-astro-081811-125534},
archivePrefix = {arXiv},
       eprint = {1206.5443},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ARA&A..50..107L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mahy17,
       author = {{Mahy}, L. and {Hutsem{\'e}kers}, D. and {Naz{\'e}}, Y. and {Royer}, P. and
         {Lebouteiller}, V. and {Waelkens}, C.},
        title = "{Evolutionary status of the Of?p star HD 148937 and of its surrounding nebula NGC 6164/5}",
      journal = {\aap},
     keywords = {infrared: stars, stars: individual: HD 148937, ISM: individual objects: NGC 6164/5, stars: abundances, circumstellar matter, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {A61},
        pages = {A61},
          doi = {10.1051/0004-6361/201629585},
archivePrefix = {arXiv},
       eprint = {1611.07257},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599A..61M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hubrig11,
       author = {{Hubrig}, S. and {Sch{\"o}ller}, M. and {Kharchenko}, N.~V. and
         {Langer}, N. and {de Wit}, W.~J. and {Ilyin}, I. and
         {Kholtygin}, A.~F. and {Piskunov}, A.~E. and {Przybilla}, N. and
         {Magori Collaboration}},
        title = "{Exploring the origin of magnetic fields in massive stars: a survey of O-type stars in clusters and in the field}",
      journal = {\aap},
     keywords = {polarization, stars: magnetic field, stars: kinematics and dynamics, open clusters and associations: general, stars: early-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = apr,
       volume = {528},
          eid = {A151},
        pages = {A151},
          doi = {10.1051/0004-6361/201016345},
archivePrefix = {arXiv},
       eprint = {1102.2503},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...528A.151H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wade12,
       author = {{Wade}, G.~A. and {Grunhut}, J. and {Gr{\"a}fener}, G. and
         {Howarth}, I.~D. and {Martins}, F. and {Petit}, V. and {Vink}, J.~S. and
         {Bagnulo}, S. and {Folsom}, C.~P. and {Naz{\'e}}, Y. and
         {Walborn}, N.~R. and {Townsend}, R.~H.~D. and {Evans}, C.~J.},
        title = "{The spectral variability and magnetic field characteristics of the Of?p star HD 148937}",
      journal = {\mnras},
     keywords = {binaries: spectroscopic, stars: early-type, stars: magnetic fields, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jan,
       volume = {419},
       number = {3},
        pages = {2459-2471},
          doi = {10.1111/j.1365-2966.2011.19897.x},
archivePrefix = {arXiv},
       eprint = {1108.4847},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.419.2459W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petit17,
       author = {{Petit}, V. and {Keszthelyi}, Z. and {MacInnis}, R. and {Cohen}, D.~H. and
         {Townsend}, R.~H.~D. and {Wade}, G.~A. and {Thomas}, S.~L. and
         {Owocki}, S.~P. and {Puls}, J. and {ud-Doula}, A.},
        title = "{Magnetic massive stars as progenitors of `heavy' stellar-mass black holes}",
      journal = {\mnras},
     keywords = {stars: black holes, stars: early-type, stars: evolution, stars: magnetic field, stars: massive, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {466},
       number = {1},
        pages = {1052-1060},
          doi = {10.1093/mnras/stw3126},
archivePrefix = {arXiv},
       eprint = {1611.08964},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.1052P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{donati02,
       author = {{Donati}, J. -F. and {Babel}, J. and {Harries}, T.~J. and
         {Howarth}, I.~D. and {Petit}, P. and {Semel}, M.},
        title = "{The magnetic field and wind confinement of {\ensuremath{\theta}}$^{1}$ Orionis C}",
      journal = {\mnras},
     keywords = {stars: individual: {\ensuremath{\theta}}1 Ori C, stars: magnetic fields, stars: rotation, stars: winds, outflows},
         year = 2002,
        month = jun,
       volume = {333},
       number = {1},
        pages = {55-70},
          doi = {10.1046/j.1365-8711.2002.05379.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.333...55D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{leith,
   author = {{Leitherer}, C.},
    title = "{Massive Stars in Starburst Galaxies and the Origin of Galactic Superwinds.}",
booktitle = {Reviews in Modern Astronomy},
     year = 1994,
   series = {Reviews in Modern Astronomy},
   volume = 7,
   editor = {{Klare}, G.},
    pages = {73-102},
   adsurl = {http://adsabs.harvard.edu/abs/1994RvMA....7...73L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{oiutils1,
       author = {{Kervella}, P. and {Bigot}, L. and {Gallenne}, A. and {Th{\'e}venin}, F.},
        title = "{The radii and limb darkenings of {\ensuremath{\alpha}} Centauri A and B . Interferometric measurements with VLTI/PIONIER}",
      journal = {\aap},
     keywords = {stars: individual: Alpha Centauri, techniques: interferometric, stars: solar-type, stars: fundamental parameters, binaries: visual, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {597},
          eid = {A137},
        pages = {A137},
          doi = {10.1051/0004-6361/201629505},
archivePrefix = {arXiv},
       eprint = {1610.06185},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...597A.137K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{oiutils2,
       author = {{Liu}, Hauyu Baobab and {M{\'e}rand}, Antoine and {Green}, Joel D. and
         {P{\'e}rez}, Sebasti{\'a}n and {Hales}, Antonio S. and {Yang}, Yao-Lun and
         {Dunham}, Michael M. and {Hasegawa}, Yasuhiro and {Henning}, Thomas and
         {Galv{\'a}n-Madrid}, Roberto and {K{\'o}sp{\'a}l}, {\'A}gnes and
         {Takami}, Michihiro and {Vorobyov}, Eduard I. and {Zhu}, Zhaohuan},
        title = "{Diagnosing 0.1-10 au Scale Morphology of the FU Ori Disk Using ALMA and VLTI/GRAVITY}",
      journal = {\apj},
     keywords = {protoplanetary disks, stars: individual: FU Ori, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {884},
       number = {1},
          eid = {97},
        pages = {97},
          doi = {10.3847/1538-4357/ab391c},
archivePrefix = {arXiv},
       eprint = {1908.02981},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884...97L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{gravity,
       author = {{Eisenhauer}, F. and {Perrin}, G. and {Brandner}, W. and
         {Straubmeier}, C. and {Perraut}, K. and {Amorim}, A. and
         {Sch{\"o}ller}, M. and {Gillessen}, S. and {Kervella}, P. and
         {Benisty}, M. and {Araujo-Hauck}, C. and {Jocou}, L. and {Lima}, J. and
         {Jakob}, G. and {Haug}, M. and {Cl{\'e}net}, Y. and {Henning}, T. and
         {Eckart}, A. and {Berger}, J. -P. and {Garcia}, P. and {Abuter}, R. and
         {Kellner}, S. and {Paumard}, T. and {Hippler}, S. and {Fischer}, S. and
         {Moulin}, T. and {Villate}, J. and {Avila}, G. and {Gr{\"a}ter}, A. and
         {Lacour}, S. and {Huber}, A. and {Wiest}, M. and {Nolot}, A. and
         {Carvas}, P. and {Dorn}, R. and {Pfuhl}, O. and {Gendron}, E. and
         {Kendrew}, S. and {Yazici}, S. and {Anton}, S. and {Jung}, Y. and
         {Thiel}, M. and {Choquet}, {\'E}. and {Klein}, R. and {Teixeira}, P. and
         {Gitton}, P. and {Moch}, D. and {Vincent}, F. and {Kudryavtseva}, N. and
         {Str{\"o}bele}, S. and {Sturm}, S. and {F{\'e}dou}, P. and
         {Lenzen}, R. and {Jolley}, P. and {Kister}, C. and {Lapeyr{\`e}re}, V. and
         {Naranjo}, V. and {Lucuix}, C. and {Hofmann}, R. and {Chapron}, F. and
         {Neumann}, U. and {Mehrgan}, L. and {Hans}, O. and {Rousset}, G. and
         {Ramos}, J. and {Suarez}, M. and {Lederer}, R. and {Reess}, J. -M. and
         {Rohloff}, R. -R. and {Haguenauer}, P. and {Bartko}, H. and
         {Sevin}, A. and {Wagner}, K. and {Lizon}, J. -L. and {Rabien}, S. and
         {Collin}, C. and {Finger}, G. and {Davies}, R. and {Rouan}, D. and
         {Wittkowski}, M. and {Dodds-Eden}, K. and {Ziegler}, D. and
         {Cassaing}, F. and {Bonnet}, H. and {Casali}, M. and {Genzel}, R. and
         {Lena}, P.},
        title = "{GRAVITY: Observing the Universe in Motion}",
      journal = {The Messenger},
         year = 2011,
        month = mar,
       volume = {143},
        pages = {16-24},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011Msngr.143...16E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hillier98,
       author = {{Hillier}, D. John and {Miller}, D.~L.},
        title = "{The Treatment of Non-LTE Line Blanketing in Spherically Expanding Outflows}",
      journal = {\apj},
     keywords = {RADIATIVE TRANSFER, STARS: EMISSION-LINE, BE, LINE: FORMATION, STARS: MASS LOSS, STARS: WOLF-RAYET, Line: Formation, Radiative Transfer, Stars: Emission-Line, Be, Stars: Mass Loss, Stars: Wolf-Rayet},
         year = 1998,
        month = mar,
       volume = {496},
       number = {1},
        pages = {407-427},
          doi = {10.1086/305350},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...496..407H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vink01,
       author = {{Vink}, Jorick S. and {de Koter}, A. and {Lamers}, H.~J.~G.~L.~M.},
        title = "{Mass-loss predictions for O and B stars as a function of metallicity}",
      journal = {\aap},
     keywords = {STARS: EARLY-TYPE, STARS: MASS-LOSS, STARS: SUPERGIANTS, STARS: WINDS, STARS: EVOLUTION, Astrophysics},
         year = 2001,
        month = apr,
       volume = {369},
        pages = {574-588},
          doi = {10.1051/0004-6361:20010127},
archivePrefix = {arXiv},
       eprint = {astro-ph/0101509},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...369..574V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sd14,
       author = {{Sim{\'o}n-D{\'\i}az}, S. and {Herrero}, A.},
        title = "{The IACOB project. I. Rotational velocities in northern Galactic O- and early B-type stars revisited. The impact of other sources of line-broadening}",
      journal = {\aap},
     keywords = {stars: early-type, stars: rotation, techniques: spectroscopic, line: profiles, astronomical databases: miscellaneous, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = feb,
       volume = {562},
          eid = {A135},
        pages = {A135},
          doi = {10.1051/0004-6361/201322758},
archivePrefix = {arXiv},
       eprint = {1311.3360},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...562A.135S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{grevesse10,
       author = {{Grevesse}, N. and {Asplund}, M. and {Sauval}, A.~J. and {Scott}, P.},
        title = "{The chemical composition of the Sun}",
      journal = {\apss},
     keywords = {Solar abundances},
         year = 2010,
        month = jul,
       volume = {328},
       number = {1-2},
        pages = {179-183},
          doi = {10.1007/s10509-010-0288-z},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Ap&SS.328..179G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hillier03,
       author = {{Hillier}, D. John and {Lanz}, T. and {Heap}, S.~R. and {Hubeny}, I. and {Smith}, L.~J. and {Evans}, C.~J. and {Lennon}, D.~J. and {Bouret}, J.~C.},
        title = "{A Tale of Two Stars: The Extreme O7 Iaf+ Supergiant AV 83 and the OC7.5 III((f)) star AV 69}",
      journal = {\apj},
     keywords = {Galaxies: Magellanic Clouds, Stars: Abundances, Stars: Atmospheres, Stars: Individual: Alphanumeric: AV 69, Stars: Individual: Alphanumeric: AV 83, Ultraviolet: Stars},
         year = 2003,
        month = may,
       volume = {588},
       number = {2},
        pages = {1039-1063},
          doi = {10.1086/374329},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...588.1039H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{brott,
       author = {{Brott}, I. and {de Mink}, S.~E. and {Cantiello}, M. and {Langer}, N. and {de Koter}, A. and {Evans}, C.~J. and {Hunter}, I. and {Trundle}, C. and {Vink}, J.~S.},
        title = "{Rotating massive main-sequence stars. I. Grids of evolutionary models and isochrones}",
      journal = {\aap},
     keywords = {stars: abundances, stars: evolution, stars: early-type, stars: rotation, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = jun,
       volume = {530},
          eid = {A115},
        pages = {A115},
          doi = {10.1051/0004-6361/201016113},
archivePrefix = {arXiv},
       eprint = {1102.0530},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...530A.115B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moss,
       author = {{Moss}, D.},
        title = "{The survival of fossil magnetic fields during pre-main sequence evolution}",
      journal = {\aap},
     keywords = {magnetic fields, magnetohydrodynamics (MHD), stars: evolution, stars: chemically peculiar},
         year = 2003,
        month = may,
       volume = {403},
        pages = {693-697},
          doi = {10.1051/0004-6361:20030431},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...403..693M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{edibles,
       author = {{Cox}, Nick L.~J. and {Cami}, Jan and {Farhang}, Amin and {Smoker}, Jonathan and {Monreal-Ibero}, Ana and {Lallement}, Rosine and {Sarre}, Peter J. and {Marshall}, Charlotte C.~M. and {Smith}, Keith T. and {Evans}, Christopher J. and {Royer}, Pierre and {Linnartz}, Harold and {Cordiner}, Martin A. and {Joblin}, Christine and {van Loon}, Jacco Th. and {Foing}, Bernard H. and {Bhatt}, Neil H. and {Bron}, Emeric and {Elyajouri}, Meriem and {de Koter}, Alex and {Ehrenfreund}, Pascale and {Javadi}, Atefeh and {Kaper}, Lex and {Khosroshadi}, Habib G. and {Laverick}, Mike and {Le Petit}, Franck and {Mulas}, Giacomo and {Roueff}, Evelyne and {Salama}, Farid and {Spaans}, Marco},
        title = "{The ESO Diffuse Interstellar Bands Large Exploration Survey (EDIBLES) . I. Project description, survey sample, and quality assessment}",
      journal = {\aap},
     keywords = {ISM: lines and bands, ISM: clouds, ISM: molecules, dust, extinction, stars: early-type, local insterstellar matter, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = oct,
       volume = {606},
          eid = {A76},
        pages = {A76},
          doi = {10.1051/0004-6361/201730912},
archivePrefix = {arXiv},
       eprint = {1708.01429},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...606A..76C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{magfrac1,
       author = {{Fossati}, L. and {Castro}, N. and {Sch{\"o}ller}, M. and {Hubrig}, S. and {Langer}, N. and {Morel}, T. and {Briquet}, M. and {Herrero}, A. and {Przybilla}, N. and {Sana}, H. and {Schneider}, F.~R.~N. and {de Koter}, A. and {BOB Collaboration}},
        title = "{B fields in OB stars (BOB): Low-resolution FORS2 spectropolarimetry of the first sample of 50 massive stars}",
      journal = {\aap},
     keywords = {stars: magnetic field, stars: early-type, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = oct,
       volume = {582},
          eid = {A45},
        pages = {A45},
          doi = {10.1051/0004-6361/201526725},
archivePrefix = {arXiv},
       eprint = {1508.00750},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...582A..45F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{magfrac2,
       author = {{Grunhut}, J.~H. and {Wade}, G.~A. and {Neiner}, C. and {Oksala}, M.~E. and {Petit}, V. and {Alecian}, E. and {Bohlender}, D.~A. and {Bouret}, J. -C. and {Henrichs}, H.~F. and {Hussain}, G.~A.~J. and {Kochukhov}, O. and {MiMeS Collaboration}},
        title = "{The MiMeS survey of Magnetism in Massive Stars: magnetic analysis of the O-type stars}",
      journal = {\mnras},
     keywords = {instrumentation: polarimeters, surveys, stars: early-type, stars: magnetic field, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = feb,
       volume = {465},
       number = {2},
        pages = {2432-2470},
          doi = {10.1093/mnras/stw2743},
archivePrefix = {arXiv},
       eprint = {1610.07895},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465.2432G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gw,
       author = {{Abbott}, B.~P. and {Abbott}, R. and {Abbott}, T.~D. and {Abernathy}, M.~R. and {Acernese}, F. and {Ackley}, K. and {Adams}, C. and {Adams}, T. and {Addesso}, P. and {Adhikari}, R.~X. and {Adya}, V.~B. and {Affeldt}, C. and {Agathos}, M. and {Agatsuma}, K. and {Aggarwal}, N. and {Aguiar}, O.~D. and {Aiello}, L. and {Ain}, A. and {Ajith}, P. and {Allen}, B. and {Allocca}, A. and {Altin}, P.~A. and {Anderson}, S.~B. and {Anderson}, W.~G. and {Arai}, K. and {Arain}, M.~A. and {Araya}, M.~C. and {Arceneaux}, C.~C. and {Areeda}, J.~S. and {Arnaud}, N. and {Arun}, K.~G. and {Ascenzi}, S. and {Ashton}, G. and {Ast}, M. and {Aston}, S.~M. and {Astone}, P. and {Aufmuth}, P. and {Aulbert}, C. and {Babak}, S. and {Bacon}, P. and {Bader}, M.~K.~M. and {Baker}, P.~T. and {Baldaccini}, F. and {Ballardin}, G. and {Ballmer}, S.~W. and {Barayoga}, J.~C. and {Barclay}, S.~E. and {Barish}, B.~C. and {Barker}, D. and {Barone}, F. and {Barr}, B. and {Barsotti}, L. and {Barsuglia}, M. and {Barta}, D. and {Bartlett}, J. and {Barton}, M.~A. and {Bartos}, I. and {Bassiri}, R. and {Basti}, A. and {Batch}, J.~C. and {Baune}, C. and {Bavigadda}, V. and {Bazzan}, M. and {Behnke}, B. and {Bejger}, M. and {Belczynski}, C. and {Bell}, A.~S. and {Bell}, C.~J. and {Berger}, B.~K. and {Bergman}, J. and {Bergmann}, G. and {Berry}, C.~P.~L. and {Bersanetti}, D. and {Bertolini}, A. and {Betzwieser}, J. and {Bhagwat}, S. and {Bhandare}, R. and {Bilenko}, I.~A. and {Billingsley}, G. and {Birch}, J. and {Birney}, R. and {Birnholtz}, O. and {Biscans}, S. and {Bisht}, A. and {Bitossi}, M. and {Biwer}, C. and {Bizouard}, M.~A. and {Blackburn}, J.~K. and {Blair}, C.~D. and {Blair}, D.~G. and {Blair}, R.~M. and {Bloemen}, S. and {Bock}, O. and {Bodiya}, T.~P. and {Boer}, M. and {Bogaert}, G. and {Bogan}, C. and {Bohe}, A. and {Bojtos}, P. and {Bond}, C. and {Bondu}, F. and {Bonnand}, R. and {Boom}, B.~A. and {Bork}, R. and {Boschi}, V. and {Bose}, S. and {Bouffanais}, Y. and {Bozzi}, A. and {Bradaschia}, C. and {Brady}, P.~R. and {Braginsky}, V.~B. and {Branchesi}, M. and {Brau}, J.~E. and {Briant}, T. and {Brillet}, A. and {Brinkmann}, M. and {Brisson}, V. and {Brockill}, P. and {Brooks}, A.~F. and {Brown}, D.~A. and {Brown}, D.~D. and {Brown}, N.~M. and {Buchanan}, C.~C. and {Buikema}, A. and {Bulik}, T. and {Bulten}, H.~J. and {Buonanno}, A. and {Buskulic}, D. and {Buy}, C. and {Byer}, R.~L. and {Cabero}, M. and {Cadonati}, L. and {Cagnoli}, G. and {Cahillane}, C. and {Bustillo}, J. Calder{\'o}n and {Callister}, T. and {Calloni}, E. and {Camp}, J.~B. and {Cannon}, K.~C. and {Cao}, J. and {Capano}, C.~D. and {Capocasa}, E. and {Carbognani}, F. and {Caride}, S. and {Casanueva Diaz}, J. and {Casentini}, C. and {Caudill}, S. and {Cavagli{\`a}}, M. and {Cavalier}, F. and {Cavalieri}, R. and {Cella}, G. and {Cepeda}, C.~B. and {Baiardi}, L. Cerboni and {Cerretani}, G. and {Cesarini}, E. and {Chakraborty}, R. and {Chalermsongsak}, T. and {Chamberlin}, S.~J. and {Chan}, M. and {Chao}, S. and {Charlton}, P. and {Chassande-Mottin}, E. and {Chen}, H.~Y. and {Chen}, Y. and {Cheng}, C. and {Chincarini}, A. and {Chiummo}, A. and {Cho}, H.~S. and {Cho}, M. and {Chow}, J.~H. and {Christensen}, N. and {Chu}, Q. and {Chua}, S. and {Chung}, S. and {Ciani}, G. and {Clara}, F. and {Clark}, J.~A. and {Cleva}, F. and {Coccia}, E. and {Cohadon}, P. -F. and {Colla}, A. and {Collette}, C.~G. and {Cominsky}, L. and {Constancio}, M. and {Conte}, A. and {Conti}, L. and {Cook}, D. and {Corbitt}, T.~R. and {Cornish}, N. and {Corsi}, A. and {Cortese}, S. and {Costa}, C.~A. and {Coughlin}, M.~W. and {Coughlin}, S.~B. and {Coulon}, J. -P. and {Countryman}, S.~T. and {Couvares}, P. and {Cowan}, E.~E. and {Coward}, D.~M. and {Cowart}, M.~J. and {Coyne}, D.~C. and {Coyne}, R. and {Craig}, K. and {Creighton}, J.~D.~E. and {Creighton}, T.~D. and {Cripe}, J. and {Crowder}, S.~G. and {Cruise}, A.~M. and {Cumming}, A. and {Cunningham}, L. and {Cuoco}, E. and {Dal Canton}, T. and {Danilishin}, S.~L. and {D'Antonio}, S. and {Danzmann}, K. and {Darman}, N.~S. and {Da Silva Costa}, C.~F. and {Dattilo}, V. and {Dave}, I. and {Daveloza}, H.~P. and {Davier}, M. and {Davies}, G.~S. and {Daw}, E.~J. and {Day}, R. and {De}, S. and {DeBra}, D. and {Debreczeni}, G. and {Degallaix}, J. and {De Laurentis}, M. and {Del{\'e}glise}, S. and {Del Pozzo}, W. and {Denker}, T. and {Dent}, T. and {Dereli}, H. and {Dergachev}, V. and {DeRosa}, R.~T. and {De Rosa}, R. and {DeSalvo}, R. and {Dhurandhar}, S. and {D{\'\i}az}, M.~C. and {Di Fiore}, L. and {Di Giovanni}, M. and {Di Lieto}, A. and {Di Pace}, S. and {Di Palma}, I. and {Di Virgilio}, A. and {Dojcinoski}, G. and {Dolique}, V. and {Donovan}, F. and {Dooley}, K.~L. and {Doravari}, S. and {Douglas}, R. and {Downes}, T.~P. and {Drago}, M. and {Drever}, R.~W.~P. and {Driggers}, J.~C. and {Du}, Z. and {Ducrot}, M. and {Dwyer}, S.~E. and {Edo}, T.~B. and {Edwards}, M.~C. and {Effler}, A. and {Eggenstein}, H. -B. and {Ehrens}, P. and {Eichholz}, J. and {Eikenberry}, S.~S. and {Engels}, W. and {Essick}, R.~C. and {Etzel}, T. and {Evans}, M. and {Evans}, T.~M. and {Everett}, R. and {Factourovich}, M. and {Fafone}, V. and {Fair}, H. and {Fairhurst}, S. and {Fan}, X. and {Fang}, Q. and {Farinon}, S. and {Farr}, B. and {Farr}, W.~M. and {Favata}, M. and {Fays}, M. and {Fehrmann}, H. and {Fejer}, M.~M. and {Feldbaum}, D. and {Ferrante}, I. and {Ferreira}, E.~C. and {Ferrini}, F. and {Fidecaro}, F. and {Finn}, L.~S. and {Fiori}, I. and {Fiorucci}, D. and {Fisher}, R.~P. and {Flaminio}, R. and {Fletcher}, M. and {Fong}, H. and {Fournier}, J. -D. and {Franco}, S. and {Frasca}, S. and {Frasconi}, F. and {Frede}, M. and {Frei}, Z. and {Freise}, A. and {Frey}, R. and {Frey}, V. and {Fricke}, T.~T. and {Fritschel}, P. and {Frolov}, V.~V. and {Fulda}, P. and {Fyffe}, M. and {Gabbard}, H.~A.~G. and {Gair}, J.~R. and {Gammaitoni}, L. and {Gaonkar}, S.~G. and {Garufi}, F. and {Gatto}, A. and {Gaur}, G. and {Gehrels}, N. and {Gemme}, G. and {Gendre}, B. and {Genin}, E. and {Gennai}, A. and {George}, J. and {Gergely}, L. and {Germain}, V. and {Ghosh}, Abhirup and {Ghosh}, Archisman and {Ghosh}, S. and {Giaime}, J.~A. and {Giardina}, K.~D. and {Giazotto}, A. and {Gill}, K. and {Glaefke}, A. and {Gleason}, J.~R. and {Goetz}, E. and {Goetz}, R. and {Gondan}, L. and {Gonz{\'a}lez}, G. and {Castro}, J.~M. Gonzalez and {Gopakumar}, A. and {Gordon}, N.~A. and {Gorodetsky}, M.~L. and {Gossan}, S.~E. and {Gosselin}, M. and {Gouaty}, R. and {Graef}, C. and {Graff}, P.~B. and {Granata}, M. and {Grant}, A. and {Gras}, S. and {Gray}, C. and {Greco}, G. and {Green}, A.~C. and {Greenhalgh}, R.~J.~S. and {Groot}, P. and {Grote}, H. and {Grunewald}, S. and {Guidi}, G.~M. and {Guo}, X. and {Gupta}, A. and {Gupta}, M.~K. and {Gushwa}, K.~E. and {Gustafson}, E.~K. and {Gustafson}, R. and {Hacker}, J.~J. and {Hall}, B.~R. and {Hall}, E.~D. and {Hammond}, G. and {Haney}, M. and {Hanke}, M.~M. and {Hanks}, J. and {Hanna}, C. and {Hannam}, M.~D. and {Hanson}, J. and {Hardwick}, T. and {Harms}, J. and {Harry}, G.~M. and {Harry}, I.~W. and {Hart}, M.~J. and {Hartman}, M.~T. and {Haster}, C. -J. and {Haughian}, K. and {Healy}, J. and {Heefner}, J. and {Heidmann}, A. and {Heintze}, M.~C. and {Heinzel}, G. and {Heitmann}, H. and {Hello}, P. and {Hemming}, G. and {Hendry}, M. and {Heng}, I.~S. and {Hennig}, J. and {Heptonstall}, A.~W. and {Heurs}, M. and {Hild}, S. and {Hoak}, D. and {Hodge}, K.~A. and {Hofman}, D. and {Hollitt}, S.~E. and {Holt}, K. and {Holz}, D.~E. and {Hopkins}, P. and {Hosken}, D.~J. and {Hough}, J. and {Houston}, E.~A. and {Howell}, E.~J. and {Hu}, Y.~M. and {Huang}, S. and {Huerta}, E.~A. and {Huet}, D. and {Hughey}, B. and {Husa}, S. and {Huttner}, S.~H. and {Huynh-Dinh}, T. and {Idrisy}, A. and {Indik}, N. and {Ingram}, D.~R. and {Inta}, R. and {Isa}, H.~N. and {Isac}, J. -M. and {Isi}, M. and {Islas}, G. and {Isogai}, T. and {Iyer}, B.~R. and {Izumi}, K. and {Jacobson}, M.~B. and {Jacqmin}, T. and {Jang}, H. and {Jani}, K. and {Jaranowski}, P. and {Jawahar}, S. and {Jim{\'e}nez-Forteza}, F. and {Johnson}, W.~W. and {Johnson-McDaniel}, N.~K. and {Jones}, D.~I. and {Jones}, R. and {Jonker}, R.~J.~G. and {Ju}, L. and {Haris}, K. and {Kalaghatgi}, C.~V. and {Kalogera}, V. and {Kandhasamy}, S. and {Kang}, G. and {Kanner}, J.~B. and {Karki}, S. and {Kasprzack}, M. and {Katsavounidis}, E. and {Katzman}, W. and {Kaufer}, S. and {Kaur}, T. and {Kawabe}, K. and {Kawazoe}, F. and {K{\'e}f{\'e}lian}, F. and {Kehl}, M.~S. and {Keitel}, D. and {Kelley}, D.~B. and {Kells}, W. and {Kennedy}, R. and {Keppel}, D.~G. and {Key}, J.~S. and {Khalaidovski}, A. and {Khalili}, F.~Y. and {Khan}, I. and {Khan}, S. and {Khan}, Z. and {Khazanov}, E.~A. and {Kijbunchoo}, N. and {Kim}, C. and {Kim}, J. and {Kim}, K. and {Kim}, Nam-Gyu and {Kim}, Namjun and {Kim}, Y. -M. and {King}, E.~J. and {King}, P.~J. and {Kinzel}, D.~L. and {Kissel}, J.~S. and {Kleybolte}, L. and {Klimenko}, S. and {Koehlenbeck}, S.~M. and {Kokeyama}, K. and {Koley}, S. and {Kondrashov}, V. and {Kontos}, A. and {Koranda}, S. and {Korobko}, M. and {Korth}, W.~Z. and {Kowalska}, I. and {Kozak}, D.~B. and {Kringel}, V. and {Krishnan}, B. and {Kr{\'o}lak}, A. and {Krueger}, C. and {Kuehn}, G. and {Kumar}, P. and {Kumar}, R. and {Kuo}, L. and {Kutynia}, A. and {Kwee}, P. and {Lackey}, B.~D. and {Landry}, M. and {Lange}, J. and {Lantz}, B. and {Lasky}, P.~D. and {Lazzarini}, A. and {Lazzaro}, C. and {Leaci}, P. and {Leavey}, S. and {Lebigot}, E.~O. and {Lee}, C.~H. and {Lee}, H.~K. and {Lee}, H.~M. and {Lee}, K. and {Lenon}, A. and {Leonardi}, M. and {Leong}, J.~R. and {Leroy}, N. and {Letendre}, N. and {Levin}, Y. and {Levine}, B.~M. and {Li}, T.~G.~F. and {Libson}, A. and {Littenberg}, T.~B. and {Lockerbie}, N.~A. and {Logue}, J. and {Lombardi}, A.~L. and {London}, L.~T. and {Lord}, J.~E. and {Lorenzini}, M. and {Loriette}, V. and {Lormand}, M. and {Losurdo}, G. and {Lough}, J.~D. and {Lousto}, C.~O. and {Lovelace}, G. and {L{\"u}ck}, H. and {Lundgren}, A.~P. and {Luo}, J. and {Lynch}, R. and {Ma}, Y. and {MacDonald}, T. and {Machenschalk}, B. and {MacInnis}, M. and {Macleod}, D.~M. and {Maga{\~n}a-Sandoval}, F. and {Magee}, R.~M. and {Mageswaran}, M. and {Majorana}, E. and {Maksimovic}, I. and {Malvezzi}, V. and {Man}, N. and {Mandel}, I. and {Mandic}, V. and {Mangano}, V. and {Mansell}, G.~L. and {Manske}, M. and {Mantovani}, M. and {Marchesoni}, F. and {Marion}, F. and {M{\'a}rka}, S. and {M{\'a}rka}, Z. and {Markosyan}, A.~S. and {Maros}, E. and {Martelli}, F. and {Martellini}, L. and {Martin}, I.~W. and {Martin}, R.~M. and {Martynov}, D.~V. and {Marx}, J.~N. and {Mason}, K. and {Masserot}, A. and {Massinger}, T.~J. and {Masso-Reid}, M. and {Matichard}, F. and {Matone}, L. and {Mavalvala}, N. and {Mazumder}, N. and {Mazzolo}, G. and {McCarthy}, R. and {McClelland}, D.~E. and {McCormick}, S. and {McGuire}, S.~C. and {McIntyre}, G. and {McIver}, J. and {McManus}, D.~J. and {McWilliams}, S.~T. and {Meacher}, D. and {Meadors}, G.~D. and {Meidam}, J. and {Melatos}, A. and {Mendell}, G. and {Mendoza-Gandara}, D. and {Mercer}, R.~A. and {Merilh}, E. and {Merzougui}, M. and {Meshkov}, S. and {Messenger}, C. and {Messick}, C. and {Meyers}, P.~M. and {Mezzani}, F. and {Miao}, H. and {Michel}, C. and {Middleton}, H. and {Mikhailov}, E.~E. and {Milano}, L. and {Miller}, J. and {Millhouse}, M. and {Minenkov}, Y. and {Ming}, J. and {Mirshekari}, S. and {Mishra}, C. and {Mitra}, S. and {Mitrofanov}, V.~P. and {Mitselmakher}, G. and {Mittleman}, R. and {Moggi}, A. and {Mohan}, M. and {Mohapatra}, S.~R.~P. and {Montani}, M. and {Moore}, B.~C. and {Moore}, C.~J. and {Moraru}, D. and {Moreno}, G. and {Morriss}, S.~R. and {Mossavi}, K. and {Mours}, B. and {Mow-Lowry}, C.~M. and {Mueller}, C.~L. and {Mueller}, G. and {Muir}, A.~W. and {Mukherjee}, Arunava and {Mukherjee}, D. and {Mukherjee}, S. and {Mukund}, N. and {Mullavey}, A. and {Munch}, J. and {Murphy}, D.~J. and {Murray}, P.~G. and {Mytidis}, A. and {Nardecchia}, I. and {Naticchioni}, L. and {Nayak}, R.~K. and {Necula}, V. and {Nedkova}, K. and {Nelemans}, G. and {Neri}, M. and {Neunzert}, A. and {Newton}, G. and {Nguyen}, T.~T. and {Nielsen}, A.~B. and {Nissanke}, S. and {Nitz}, A. and {Nocera}, F. and {Nolting}, D. and {Normandin}, M.~E.~N. and {Nuttall}, L.~K. and {Oberling}, J. and {Ochsner}, E. and {O'Dell}, J. and {Oelker}, E. and {Ogin}, G.~H. and {Oh}, J.~J. and {Oh}, S.~H. and {Ohme}, F. and {Oliver}, M. and {Oppermann}, P. and {Oram}, Richard J. and {O'Reilly}, B. and {O'Shaughnessy}, R. and {Ott}, C.~D. and {Ottaway}, D.~J. and {Ottens}, R.~S. and {Overmier}, H. and {Owen}, B.~J. and {Pai}, A. and {Pai}, S.~A. and {Palamos}, J.~R. and {Palashov}, O. and {Palomba}, C. and {Pal-Singh}, A. and {Pan}, H. and {Pan}, Y. and {Pankow}, C. and {Pannarale}, F. and {Pant}, B.~C. and {Paoletti}, F. and {Paoli}, A. and {Papa}, M.~A. and {Paris}, H.~R. and {Parker}, W. and {Pascucci}, D. and {Pasqualetti}, A. and {Passaquieti}, R. and {Passuello}, D. and {Patricelli}, B. and {Patrick}, Z. and {Pearlstone}, B.~L. and {Pedraza}, M. and {Pedurand}, R. and {Pekowsky}, L. and {Pele}, A. and {Penn}, S. and {Perreca}, A. and {Pfeiffer}, H.~P. and {Phelps}, M. and {Piccinni}, O. and {Pichot}, M. and {Pickenpack}, M. and {Piergiovanni}, F. and {Pierro}, V. and {Pillant}, G. and {Pinard}, L. and {Pinto}, I.~M. and {Pitkin}, M. and {Poeld}, J.~H. and {Poggiani}, R. and {Popolizio}, P. and {Post}, A. and {Powell}, J. and {Prasad}, J. and {Predoi}, V. and {Premachandra}, S.~S. and {Prestegard}, T. and {Price}, L.~R. and {Prijatelj}, M. and {Principe}, M. and {Privitera}, S. and {Prix}, R. and {Prodi}, G.~A. and {Prokhorov}, L. and {Puncken}, O. and {Punturo}, M. and {Puppo}, P. and {P{\"u}rrer}, M. and {Qi}, H. and {Qin}, J. and {Quetschke}, V. and {Quintero}, E.~A. and {Quitzow-James}, R. and {Raab}, F.~J. and {Rabeling}, D.~S. and {Radkins}, H. and {Raffai}, P. and {Raja}, S. and {Rakhmanov}, M. and {Ramet}, C.~R. and {Rapagnani}, P. and {Raymond}, V. and {Razzano}, M. and {Re}, V. and {Read}, J. and {Reed}, C.~M. and {Regimbau}, T. and {Rei}, L. and {Reid}, S. and {Reitze}, D.~H. and {Rew}, H. and {Reyes}, S.~D. and {Ricci}, F. and {Riles}, K. and {Robertson}, N.~A. and {Robie}, R. and {Robinet}, F. and {Rocchi}, A. and {Rolland}, L. and {Rollins}, J.~G. and {Roma}, V.~J. and {Romano}, J.~D. and {Romano}, R. and {Romanov}, G. and {Romie}, J.~H. and {Rosi{\'n}ska}, D. and {Rowan}, S. and {R{\"u}diger}, A. and {Ruggi}, P. and {Ryan}, K. and {Sachdev}, S. and {Sadecki}, T. and {Sadeghian}, L. and {Salconi}, L. and {Saleem}, M. and {Salemi}, F. and {Samajdar}, A. and {Sammut}, L. and {Sampson}, L.~M. and {Sanchez}, E.~J. and {Sandberg}, V. and {Sandeen}, B. and {Sanders}, G.~H. and {Sanders}, J.~R. and {Sassolas}, B. and {Sathyaprakash}, B.~S. and {Saulson}, P.~R. and {Sauter}, O. and {Savage}, R.~L. and {Sawadsky}, A. and {Schale}, P. and {Schilling}, R. and {Schmidt}, J. and {Schmidt}, P. and {Schnabel}, R. and {Schofield}, R.~M.~S. and {Sch{\"o}nbeck}, A. and {Schreiber}, E. and {Schuette}, D. and {Schutz}, B.~F. and {Scott}, J. and {Scott}, S.~M. and {Sellers}, D. and {Sengupta}, A.~S. and {Sentenac}, D. and {Sequino}, V. and {Sergeev}, A. and {Serna}, G. and {Setyawati}, Y. and {Sevigny}, A. and {Shaddock}, D.~A. and {Shaffer}, T. and {Shah}, S. and {Shahriar}, M.~S. and {Shaltev}, M. and {Shao}, Z. and {Shapiro}, B. and {Shawhan}, P. and {Sheperd}, A. and {Shoemaker}, D.~H. and {Shoemaker}, D.~M. and {Siellez}, K. and {Siemens}, X. and {Sigg}, D. and {Silva}, A.~D. and {Simakov}, D. and {Singer}, A. and {Singer}, L.~P. and {Singh}, A. and {Singh}, R. and {Singhal}, A. and {Sintes}, A.~M. and {Slagmolen}, B.~J.~J. and {Smith}, J.~R. and {Smith}, M.~R. and {Smith}, N.~D. and {Smith}, R.~J.~E. and {Son}, E.~J. and {Sorazu}, B. and {Sorrentino}, F. and {Souradeep}, T. and {Srivastava}, A.~K. and {Staley}, A. and {Steinke}, M. and {Steinlechner}, J. and {Steinlechner}, S. and {Steinmeyer}, D. and {Stephens}, B.~C. and {Stevenson}, S.~P. and {Stone}, R. and {Strain}, K.~A. and {Straniero}, N. and {Stratta}, G. and {Strauss}, N.~A. and {Strigin}, S. and {Sturani}, R. and {Stuver}, A.~L. and {Summerscales}, T.~Z. and {Sun}, L. and {Sutton}, P.~J. and {Swinkels}, B.~L. and {Szczepa{\'n}czyk}, M.~J. and {Tacca}, M. and {Talukder}, D. and {Tanner}, D.~B. and {T{\'a}pai}, M. and {Tarabrin}, S.~P. and {Taracchini}, A. and {Taylor}, R. and {Theeg}, T. and {Thirugnanasambandam}, M.~P. and {Thomas}, E.~G. and {Thomas}, M. and {Thomas}, P. and {Thorne}, K.~A. and {Thorne}, K.~S. and {Thrane}, E. and {Tiwari}, S. and {Tiwari}, V. and {Tokmakov}, K.~V. and {Tomlinson}, C. and {Tonelli}, M. and {Torres}, C.~V. and {Torrie}, C.~I. and {T{\"o}yr{\"a}}, D. and {Travasso}, F. and {Traylor}, G. and {Trifir{\`o}}, D. and {Tringali}, M.~C. and {Trozzo}, L. and {Tse}, M. and {Turconi}, M. and {Tuyenbayev}, D. and {Ugolini}, D. and {Unnikrishnan}, C.~S. and {Urban}, A.~L. and {Usman}, S.~A. and {Vahlbruch}, H. and {Vajente}, G. and {Valdes}, G. and {Vallisneri}, M. and {van Bakel}, N. and {van Beuzekom}, M. and {van den Brand}, J.~F.~J. and {Van Den Broeck}, C. and {Vander-Hyde}, D.~C. and {van der Schaaf}, L. and {van Heijningen}, J.~V. and {van Veggel}, A.~A. and {Vardaro}, M. and {Vass}, S. and {Vas{\'u}th}, M. and {Vaulin}, R. and {Vecchio}, A. and {Vedovato}, G. and {Veitch}, J. and {Veitch}, P.~J. and {Venkateswara}, K. and {Verkindt}, D. and {Vetrano}, F. and {Vicer{\'e}}, A. and {Vinciguerra}, S. and {Vine}, D.~J. and {Vinet}, J. -Y. and {Vitale}, S. and {Vo}, T. and {Vocca}, H. and {Vorvick}, C. and {Voss}, D. and {Vousden}, W.~D. and {Vyatchanin}, S.~P. and {Wade}, A.~R. and {Wade}, L.~E. and {Wade}, M. and {Waldman}, S.~J. and {Walker}, M. and {Wallace}, L. and {Walsh}, S. and {Wang}, G. and {Wang}, H. and {Wang}, M. and {Wang}, X. and {Wang}, Y. and {Ward}, H. and {Ward}, R.~L. and {Warner}, J. and {Was}, M. and {Weaver}, B. and {Wei}, L. -W. and {Weinert}, M. and {Weinstein}, A.~J. and {Weiss}, R. and {Welborn}, T. and {Wen}, L. and {We{\ss}els}, P. and {Westphal}, T. and {Wette}, K. and {Whelan}, J.~T. and {Whitcomb}, S.~E. and {White}, D.~J. and {Whiting}, B.~F. and {Wiesner}, K. and {Wilkinson}, C. and {Willems}, P.~A. and {Williams}, L. and {Williams}, R.~D. and {Williamson}, A.~R. and {Willis}, J.~L. and {Willke}, B. and {Wimmer}, M.~H. and {Winkelmann}, L. and {Winkler}, W. and {Wipf}, C.~C. and {Wiseman}, A.~G. and {Wittel}, H. and {Woan}, G. and {Worden}, J. and {Wright}, J.~L. and {Wu}, G. and {Yablon}, J. and {Yakushin}, I. and {Yam}, W. and {Yamamoto}, H. and {Yancey}, C.~C. and {Yap}, M.~J. and {Yu}, H. and {Yvert}, M. and {Zadro{\.Z}ny}, A. and {Zangrando}, L. and {Zanolin}, M. and {Zendri}, J. -P. and {Zevin}, M. and {Zhang}, F. and {Zhang}, L. and {Zhang}, M. and {Zhang}, Y. and {Zhao}, C. and {Zhou}, M. and {Zhou}, Z. and {Zhu}, X.~J. and {Zucker}, M.~E. and {Zuraw}, S.~E. and {Zweizig}, J. and {LIGO Scientific Collaboration} and {Virgo Collaboration}},
        title = "{Observation of Gravitational Waves from a Binary Black Hole Merger}",
      journal = {\prl},
     keywords = {General Relativity and Quantum Cosmology, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = feb,
       volume = {116},
       number = {6},
          eid = {061102},
        pages = {061102},
          doi = {10.1103/PhysRevLett.116.061102},
archivePrefix = {arXiv},
       eprint = {1602.03837},
 primaryClass = {gr-qc},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016PhRvL.116f1102A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bj,
       author = {{Bailer-Jones}, C.~A.~L. and {Rybizki}, J. and {Fouesneau}, M. and {Demleitner}, M. and {Andrae}, R.},
        title = "{Estimating distances from parallaxes. V: Geometric and photogeometric distances to 1.47 billion stars in Gaia Early Data Release 3}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.05220},
        pages = {arXiv:2012.05220},
archivePrefix = {arXiv},
       eprint = {2012.05220},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201205220B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shultz15,
       author = {{Shultz}, M. and {Wade}, G.~A. and {Alecian}, E. and {BinaMIcS Collaboration}},
        title = "{Detection of magnetic fields in both B-type components of the {\ensuremath{\in}} Lupi system: a new constraint on the origin of fossil fields?}",
      journal = {\mnras},
     keywords = {binaries: close, stars: early-type, stars: individual: {\ensuremath{\in}} Lupi, stars: magnetic field, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = nov,
       volume = {454},
       number = {1},
        pages = {L1-L5},
          doi = {10.1093/mnrasl/slv096},
archivePrefix = {arXiv},
       eprint = {1507.05084},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.454L...1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{doula,
       author = {{Ud-Doula}, Asif and {Owocki}, Stanley P. and {Townsend}, Richard H.~D.},
        title = "{Dynamical simulations of magnetically channelled line-driven stellar winds - II. The effects of field-aligned rotation}",
      journal = {\mnras},
     keywords = {MHD, stars: early-type, stars: magnetic fields, stars: mass-loss, stars: rotation, stars: winds, outflows, Astrophysics},
         year = 2008,
        month = mar,
       volume = {385},
       number = {1},
        pages = {97-108},
          doi = {10.1111/j.1365-2966.2008.12840.x},
archivePrefix = {arXiv},
       eprint = {0712.2780},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.385...97U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heavybh,
       author = {{Petit}, V. and {Keszthelyi}, Z. and {MacInnis}, R. and {Cohen}, D.~H. and {Townsend}, R.~H.~D. and {Wade}, G.~A. and {Thomas}, S.~L. and {Owocki}, S.~P. and {Puls}, J. and {ud-Doula}, A.},
        title = "{Magnetic massive stars as progenitors of `heavy' stellar-mass black holes}",
      journal = {\mnras},
     keywords = {stars: black holes, stars: early-type, stars: evolution, stars: magnetic field, stars: massive, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {466},
       number = {1},
        pages = {1052-1060},
          doi = {10.1093/mnras/stw3126},
archivePrefix = {arXiv},
       eprint = {1611.08964},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.1052P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shultz19,
       author = {{Shultz}, M.~E. and {Johnston}, C. and {Labadie-Bartz}, J. and {Petit}, V. and {David-Uraz}, A. and {Kochukhov}, {\O}. and {Wade}, G.~A. and {Pepper}, J. and {Stassun}, K.~G. and {Rodriguez}, J.~E. and {Lund}, M.~B. and {James}, D.~J.},
        title = "{MOBSTER - III. HD 62658: a magnetic Bp star in an eclipsing binary with a non-magnetic `identical twin'}",
      journal = {\mnras},
     keywords = {binaries: eclipsing, stars: chemically peculiar, stars: early-type, stars: individual: HD 62658, stars: magnetic field, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {490},
       number = {3},
        pages = {4154-4165},
          doi = {10.1093/mnras/stz2846},
archivePrefix = {arXiv},
       eprint = {1910.02928},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.490.4154S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{domnat,
       author = {{Bowman}, Dominic M. and {Burssens}, Siemen and {Pedersen}, May G. and {Johnston}, Cole and {Aerts}, Conny and {Buysschaert}, Bram and {Michielsen}, Mathias and {Tkachenko}, Andrew and {Rogers}, Tamara M. and {Edelmann}, Philipp V.~F. and {Ratnasingam}, Rathish P. and {Sim{\'o}n-D{\'\i}az}, Sergio and {Castro}, Norberto and {Moravveji}, Ehsan and {Pope}, Benjamin J.~S. and {White}, Timothy R. and {De Cat}, Peter},
        title = "{Low-frequency gravity waves in blue supergiants revealed by high-precision space photometry}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = may,
       volume = {3},
        pages = {760-765},
          doi = {10.1038/s41550-019-0768-1},
archivePrefix = {arXiv},
       eprint = {1905.02120},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NatAs...3..760B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{domaa2020,
       author = {{Bowman}, D.~M. and {Burssens}, S. and {Sim{\'o}n-D{\'\i}az}, S. and {Edelmann}, P.~V.~F. and {Rogers}, T.~M. and {Horst}, L. and {R{\"o}pke}, F.~K. and {Aerts}, C.},
        title = "{Photometric detection of internal gravity waves in upper main-sequence stars. II. Combined TESS photometry and high-resolution spectroscopy}",
      journal = {\aap},
     keywords = {asteroseismology, stars: early-type, stars: oscillations, stars: evolution, stars: rotation, stars: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = aug,
       volume = {640},
          eid = {A36},
        pages = {A36},
          doi = {10.1051/0004-6361/202038224},
archivePrefix = {arXiv},
       eprint = {2006.03012},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...640A..36B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{deem,
       author = {{Deeming}, T.~J.},
        title = "{Fourier Analysis with Unequally-Spaced Data}",
      journal = {\apss},
         year = 1975,
        month = aug,
       volume = {36},
       number = {1},
        pages = {137-158},
          doi = {10.1007/BF00681947},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1975Ap&SS..36..137D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kurtz,
       author = {{Kurtz}, D.~W.},
        title = "{An algorithm for significantly reducing the time necessary to computea Discrete Fourier Transform periodogram of unequally spaced data.}",
      journal = {\mnras},
     keywords = {Algorithms, Fourier Transformation, Run Time (Computers), Stellar Oscillations, Discrete Functions, Fortran, Frequency Distribution, Light Curve, Astronomy},
         year = 1985,
        month = apr,
       volume = {213},
        pages = {773-776},
          doi = {10.1093/mnras/213.4.773},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985MNRAS.213..773K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{jenk,
       author = {{Jenkins}, Jon M. and {Twicken}, Joseph D. and {McCauliff}, Sean and {Campbell}, Jennifer and {Sanderfer}, Dwight and {Lung}, David and {Mansouri-Samani}, Masoud and {Girouard}, Forrest and {Tenenbaum}, Peter and {Klaus}, Todd and {Smith}, Jeffrey C. and {Caldwell}, Douglas A. and {Chacon}, A.~D. and {Henze}, Christopher and {Heiges}, Cory and {Latham}, David W. and {Morgan}, Edward and {Swade}, Daryl and {Rinehart}, Stephen and {Vanderspek}, Roland},
        title = "{The TESS science processing operations center}",
    booktitle = {Software and Cyberinfrastructure for Astronomy IV},
         year = 2016,
       editor = {{Chiozzi}, Gianluca and {Guzman}, Juan C.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9913},
        month = aug,
          eid = {99133E},
        pages = {99133E},
          doi = {10.1117/12.2233418},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SPIE.9913E..3EJ},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dr3,
       author = {{Bailer-Jones}, C.~A.~L. and {Rybizki}, J. and {Fouesneau}, M. and {Demleitner}, M. and {Andrae}, R.},
        title = "{Estimating distances from parallaxes. V: Geometric and photogeometric distances to 1.47 billion stars in Gaia Early Data Release 3}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.05220},
        pages = {arXiv:2012.05220},
archivePrefix = {arXiv},
       eprint = {2012.05220},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201205220B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cp70,
       author = {{Catchpole}, R.~M. and {Feast}, M.~W.},
        title = "{Nebulosities ejected from the star HD 148937}",
      journal = {The Observatory},
         year = 1970,
        month = aug,
       volume = {90},
        pages = {136-141},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1970Obs....90..136C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{vlti,
       author = {{Haguenauer}, Pierre and {Alonso}, Jaime and {Bourget}, Pierre and
         {Brillant}, Stephane and {Gitton}, Philippe and {Guisard}, Stephane and
         {Poupar}, S{\'e}bastien and {Schuhler}, Nicolas and {Abuter}, Roberto and
         {Andolfato}, Luigi and {Blanchard}, Guillaume and
         {Berger}, Jean-Philippe and {Cortes}, Angela and
         {D{\'e}rie}, Fr{\'e}d{\'e}ric and {Delplancke}, Fran{\c{c}}oise and
         {Di Lieto}, Nicola and {Dupuy}, Christophe and {Gilli}, Bruno and
         {Glindemann}, Andreas and {Guniat}, Serge and {Huedepohl}, Gerhard and
         {Kaufer}, Andreas and {Le Bouquin}, Jean-Baptiste and
         {L{\'e}vque}, Samuel and {M{\'e}nardi}, Serge and {M{\'e}rand
        }, Antoine and {Morel}, Sebastien and {Percheron}, Isabelle and
         {Phan Duc}, Than and {Pino}, Andres and {Ramirez}, Andres and
         {Rengaswamy}, Sridharan and {Richichi}, Andrea and {Rivinius}, Thomas and
         {Sahlmann}, Johannes and {Schoeller}, Markus and {Schmid}, Christian and
         {Stefl}, Stan and {Valdes}, Guillermo and {van Belle}, Gerard and
         {Wehner}, Stefan and {Wittkowski}, Markus},
        title = "{The very large telescope Interferometer: 2010 edition}",
    booktitle = {\procspie},
         year = 2010,
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7734},
        month = jul,
          eid = {773404},
        pages = {773404},
          doi = {10.1117/12.857070},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010SPIE.7734E..04H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{pionier,
       author = {{Le Bouquin}, J. -B. and {Berger}, J. -P. and {Lazareff}, B. and
         {Zins}, G. and {Haguenauer}, P. and {Jocou}, L. and {Kern}, P. and
         {Millan-Gabet}, R. and {Traub}, W. and {Absil}, O. and
         {Augereau}, J. -C. and {Benisty}, M. and {Blind}, N. and {Bonfils}, X. and
         {Bourget}, P. and {Delboulbe}, A. and {Feautrier}, P. and
         {Germain}, M. and {Gitton}, P. and {Gillier}, D. and {Kiekebusch}, M. and
         {Kluska}, J. and {Knudstrup}, J. and {Labeye}, P. and {Lizon}, J. -L. and
         {Monin}, J. -L. and {Magnard}, Y. and {Malbet}, F. and {Maurel}, D. and
         {M{\'e}nard}, F. and {Micallef}, M. and {Michaud}, L. and
         {Montagnier}, G. and {Morel}, S. and {Moulin}, T. and {Perraut}, K. and
         {Popovic}, D. and {Rabou}, P. and {Rochat}, S. and {Rojas}, C. and
         {Roussel}, F. and {Roux}, A. and {Stadler}, E. and {Stefl}, S. and
         {Tatulli}, E. and {Ventura}, N.},
        title = "{PIONIER: a 4-telescope visitor instrument at VLTI}",
      journal = {\aap},
     keywords = {instrumentation: interferometers, techniques: interferometric, techniques: high angular resolution, instrumentation: high angular resolution, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = nov,
       volume = {535},
          eid = {A67},
        pages = {A67},
          doi = {10.1051/0004-6361/201117586},
archivePrefix = {arXiv},
       eprint = {1109.1918},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...535A..67L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{jamesbarron,
       author = {{Barron}, J. and {Wade}, G.~A. and {Bowman}, D.~M. and {David-Uraz}, A. and {Munoz}, M.~S. and {Pablo}, H. and {Sim{\'o}n-D{\'\i}z}, S.},
        title = "{MOBSTER: Identifying Candidate Magnetic O Stars through Rotational Modulation of TESS Photometry}",
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Stellar Magnetism: A Workshop in Honour of the Career and Contributions of John D. Landstreet},
         year = 2020,
       editor = {{Wade}, Gregg and {Alecian}, Evelyne and {Bohlender}, David and {Sigut}, Aaron},
       volume = {11},
        month = nov,
        pages = {226-235},
archivePrefix = {arXiv},
       eprint = {2001.04534},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020pase.conf..226B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nazehd108,
       author = {{Naz{\'e}}, Y. and {Walborn}, N.~R. and {Martins}, F.},
        title = "{The mysterious Of?p class and the magnetic O-star {\ensuremath{\theta}}$^{1}$ Ori C: confronting observations}",
      journal = {\rmxaa},
     keywords = {stars: early-type, stars: individual (HD 108, HD 148937, HD 191612, {\ensuremath{\theta}} 1 Ori C), stars: variables: other, Astrophysics},
         year = 2008,
        month = oct,
       volume = {44},
        pages = {331-340},
archivePrefix = {arXiv},
       eprint = {0807.3496},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008RMxAA..44..331N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{powr,
       author = {{Sander}, A. and {Shenar}, T. and {Hainich}, R. and {G{\'\i}menez-Garc{\'\i}a}, A. and {Todt}, H. and {Hamann}, W. -R.},
        title = "{On the consistent treatment of the quasi-hydrostatic layers in hot star atmospheres}",
      journal = {\aap},
     keywords = {stars: early-type, stars: mass-loss, stars: winds, outflows, stars: atmospheres, stars: fundamental parameters, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = may,
       volume = {577},
          eid = {A13},
        pages = {A13},
          doi = {10.1051/0004-6361/201425356},
archivePrefix = {arXiv},
       eprint = {1503.01338},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...577A..13S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hirai,
       author = {{Hirai}, Ryosuke and {Podsiadlowski}, Philipp and {Owocki}, Stanley P. and {Schneider}, Fabian R.~N. and {Smith}, Nathan},
        title = "{Modelling Eta Carinae's Great Eruption and its surrounding nebula}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = nov,
          eid = {arXiv:2011.12434},
        pages = {arXiv:2011.12434},
archivePrefix = {arXiv},
       eprint = {2011.12434},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201112434H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fab20,
       author = {{Schneider}, F.~R.~N. and {Ohlmann}, S.~T. and {Podsiadlowski}, Ph and {R{\"o}pke}, F.~K. and {Balbus}, S.~A. and {Pakmor}, R.},
        title = "{Long-term evolution of a magnetic massive merger product}",
      journal = {\mnras},
     keywords = {binaries: general, blue stragglers, stars: evolution, stars: individual: {\ensuremath{\tau}} Sco, stars: magnetic field, stars: massive, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = may,
       volume = {495},
       number = {3},
        pages = {2796-2812},
          doi = {10.1093/mnras/staa1326},
archivePrefix = {arXiv},
       eprint = {2005.05335},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.495.2796S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fabnat,
       author = {{Schneider}, Fabian R.~N. and {Ohlmann}, Sebastian T. and {Podsiadlowski}, Philipp and {R{\"o}pke}, Friedrich K. and {Balbus}, Steven A. and {Pakmor}, R{\"u}diger and {Springel}, Volker},
        title = "{Stellar mergers as the origin of magnetic massive stars}",
      journal = {\nat},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = oct,
       volume = {574},
       number = {7777},
        pages = {211-214},
          doi = {10.1038/s41586-019-1621-5},
archivePrefix = {arXiv},
       eprint = {1910.14058},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019Natur.574..211S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wade19,
       author = {{Wade}, G.~A. and {Smoker}, J.~V. and {Evans}, C.~J. and
         {Howarth}, I.~D. and {Barba}, R. and {Cox}, N.~L.~J. and {Morrell}, N. and
         {Naz{\'e}}, Y. and {Cami}, J. and {Farhang}, A. and {Walborn}, N.~R. and
         {Arias}, J. and {Gamen}, R.},
        title = "{A remarkable change of the spectrum of the magnetic Of?p star HD 148937 reveals evidence of an eccentric, high-mass binary}",
      journal = {\mnras},
     keywords = {binaries: spectroscopic, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {483},
       number = {2},
        pages = {2581-2591},
          doi = {10.1093/mnras/sty3304},
archivePrefix = {arXiv},
       eprint = {1811.11153},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483.2581W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{zin02,
       author = {{Zinnecker}, Hans},
        title = "{Formation of massive binaries}",
     keywords = {Astrophysics},
    booktitle = {A Massive Star Odyssey: From Main Sequence to Supernova},
         year = 2003,
       editor = {{van der Hucht}, Karel and {Herrero}, Artemio and {Esteban}, C{\'e}sar},
       volume = {212},
        month = jan,
        pages = {80},
archivePrefix = {arXiv},
       eprint = {astro-ph/0301078},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003IAUS..212...80Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moss,
       author = {{Moss}, D.},
        title = "{The survival of fossil magnetic fields during pre-main sequence evolution}",
      journal = {\aap},
     keywords = {magnetic fields, magnetohydrodynamics (MHD), stars: evolution, stars: chemically peculiar},
         year = 2003,
        month = may,
       volume = {403},
        pages = {693-697},
          doi = {10.1051/0004-6361:20030431},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...403..693M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{laurenthd,
       author = {{Mahy}, L. and {Hutsem{\'e}kers}, D. and {Naz{\'e}}, Y. and {Royer}, P. and
         {Lebouteiller}, V. and {Waelkens}, C.},
        title = "{Evolutionary status of the Of?p star HD 148937 and of its surrounding nebula NGC 6164/5}",
      journal = {\aap},
     keywords = {infrared: stars, stars: individual: HD 148937, ISM: individual objects: NGC 6164/5, stars: abundances, circumstellar matter, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {A61},
        pages = {A61},
          doi = {10.1051/0004-6361/201629585},
archivePrefix = {arXiv},
       eprint = {1611.07257},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599A..61M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{sana12,
       author = {{Sana}, H. and {Dunstall}, P.~R. and {H{\'e}nault-Brunet}, V. and {Walborn}, N.~R. and {de Koter}, A. and {de Mink}, S.~E. and {Dufton}, P.~L. and {Evans}, C.~J. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Taylor}, W.~D. and {Vink}, J.~S.},
        title = "{The VLT-FLAMES Tarantula Survey: Multiplicity and Dynamics of the Massive Stars in 30 Dor}",
    booktitle = {Proceedings of a Scientific Meeting in Honor of Anthony F. J. Moffat},
         year = 2012,
       editor = {{Drissen}, L. and {Robert}, C. and {St-Louis}, N. and {Moffat}, A.~F.~J.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {465},
        month = dec,
        pages = {284},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ASPC..465..284S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smash,
       author = {{Sana}, H. and {Le Bouquin}, J. -B. and {Lacour}, S. and
         {Berger}, J. -P. and {Duvert}, G. and {Gauchet}, L. and {Norris}, B. and
         {Olofsson}, J. and {Pickel}, D. and {Zins}, G. and {Absil}, O. and
         {de Koter}, A. and {Kratter}, K. and {Schnurr}, O. and {Zinnecker}, H.},
        title = "{Southern Massive Stars at High Angular Resolution: Observational Campaign and Companion Detection}",
      journal = {\apjs},
     keywords = {binaries: visual, stars: early-type, stars: imaging, surveys, techniques: high angular resolution, techniques: interferometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = nov,
       volume = {215},
       number = {1},
          eid = {15},
        pages = {15},
          doi = {10.1088/0067-0049/215/1/15},
archivePrefix = {arXiv},
       eprint = {1409.6304},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJS..215...15S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{walborn72,
       author = {{Walborn}, N.~R.},
        title = "{Spectral classification of OB stars in both hemispheres and the absolute-magnitude calibration.}",
      journal = {\aj},
         year = 1972,
        month = may,
       volume = {77},
        pages = {312-318},
          doi = {10.1086/111285},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972AJ.....77..312W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze08,
       author = {{Naz{\'e}}, Ya{\"e}l and {Walborn}, Nolan R. and {Rauw}, Gregor and
         {Martins}, Fabrice and {Pollock}, A.~M.~T. and {Bond}, Howard E.},
        title = "{HD 148937: A Multiwavelength Study of the Third Galactic Member of the Of?p Class}",
      journal = {\aj},
     keywords = {stars: early-type, stars: individual: HD 148937, X-rays: individual: HD 148937, X-rays: stars, Astrophysics},
         year = 2008,
        month = may,
       volume = {135},
       number = {5},
        pages = {1946-1957},
          doi = {10.1088/0004-6256/135/5/1946},
archivePrefix = {arXiv},
       eprint = {0803.0605},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008AJ....135.1946N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze12,
       author = {{Naz{\'e}}, Ya{\"e}l and {Zhekov}, Svetozar A. and {Walborn}, Nolan R.},
        title = "{High-resolution X-Ray Spectroscopy of the Magnetic Of?p Star HD 148937}",
      journal = {\apj},
     keywords = {stars: early-type, stars: individual: HD148937, stars: massive, X-rays: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = feb,
       volume = {746},
       number = {2},
          eid = {142},
        pages = {142},
          doi = {10.1088/0004-637X/746/2/142},
archivePrefix = {arXiv},
       eprint = {1111.7186},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...746..142N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{conti,
       author = {{Conti}, Peter S. and {Alschuler}, William R.},
        title = "{Spectroscopic Studies of O-Type Stars. I. Classification and Absolute Magnitudes}",
      journal = {\apj},
         year = 1971,
        month = dec,
       volume = {170},
        pages = {325},
          doi = {10.1086/151218},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971ApJ...170..325C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mathys,
       author = {{Mathys}, G.},
        title = "{The upper main sequence of OB associations. I. Spectral types and lines of C and N of southern single-lined O stars.}",
      journal = {\aaps},
     keywords = {Abundance, Blue Stars, Carbon, Nitrogen, O Stars, Stellar Spectra, Astronomical Catalogs, Evolution, Spectral Line Width, Stellar Luminosity, Astrophysics},
         year = 1988,
        month = dec,
       volume = {76},
        pages = {427-444},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988A&AS...76..427M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martins05,
       author = {{Martins}, Lucimara P. and {Gonz{\'a}lez Delgado}, Rosa M. and {Leitherer}, Claus and {Cervi{\~n}o}, Miguel and {Hauschildt}, Peter},
        title = "{A high-resolution stellar library for evolutionary population synthesis}",
      journal = {\mnras},
     keywords = {stars: atmospheres, stars: evolution, Astrophysics},
         year = 2005,
        month = mar,
       volume = {358},
       number = {1},
        pages = {49-65},
          doi = {10.1111/j.1365-2966.2005.08703.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0501225},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.358...49M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wade11,
       author = {{Wade}, G.~A. and {Howarth}, I.~D. and {Townsend}, R.~H.~D. and {Grunhut}, J.~H. and {Shultz}, M. and {Bouret}, J. -C. and {Fullerton}, A. and {Marcolino}, W. and {Martins}, F. and {Naz{\'e}}, Y. and {Ud Doula}, A. and {Walborn}, N.~R. and {Donati}, J. -F.},
        title = "{Confirmation of the magnetic oblique rotator model for the Of?p star HD 191612}",
      journal = {\mnras},
     keywords = {stars: individual: HD 191612, stars: magnetic field, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = oct,
       volume = {416},
       number = {4},
        pages = {3160-3169},
          doi = {10.1111/j.1365-2966.2011.19265.x},
archivePrefix = {arXiv},
       eprint = {1106.3008},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.416.3160W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petit13,
       author = {{Petit}, V. and {Owocki}, S.~P. and {Wade}, G.~A. and {Cohen}, D.~H. and {Sundqvist}, J.~O. and {Gagn{\'e}}, M. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Oksala}, M.~E. and {Bohlender}, D.~A. and {Rivinius}, T. and {Henrichs}, H.~F. and {Alecian}, E. and {Townsend}, R.~H.~D. and {ud-Doula}, A. and {MiMeS Collaboration}},
        title = "{A magnetic confinement versus rotation classification of massive-star magnetospheres}",
      journal = {\mnras},
     keywords = {circumstellar matter, stars: early-type, stars: fundamental parameters, stars: magnetic fields, stars: mass-loss, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = feb,
       volume = {429},
       number = {1},
        pages = {398-422},
          doi = {10.1093/mnras/sts344},
archivePrefix = {arXiv},
       eprint = {1211.0282},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.429..398P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mp,
       author = {{Martins}, F. and {Plez}, B.},
        title = "{UBVJHK synthetic photometry of Galactic O stars}",
      journal = {\aap},
     keywords = {stars: fundamental parameters, stars: atmospheres, stars: early-type, Astrophysics},
         year = 2006,
        month = oct,
       volume = {457},
       number = {2},
        pages = {637-644},
          doi = {10.1051/0004-6361:20065753},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606587},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...457..637M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bonnsai,
       author = {{Schneider}, F.~R.~N. and {Langer}, N. and {de Koter}, A. and {Brott}, I. and {Izzard}, R.~G. and {Lau}, H.~H.~B.},
        title = "{Bonnsai: a Bayesian tool for comparing stars with stellar evolution models}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: statistical, stars: general, stars: fundamental parameters, stars: rotation, binaries: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = oct,
       volume = {570},
          eid = {A66},
        pages = {A66},
          doi = {10.1051/0004-6361/201424286},
archivePrefix = {arXiv},
       eprint = {1408.3409},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...570A..66S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sana11,
       author = {{Sana}, H. and {Le Bouquin}, J. -B. and {De Becker}, M. and {Berger}, J. -P. and {de Koter}, A. and {M{\'e}rand}, A.},
        title = "{The Non-thermal Radio Emitter HD 93250 Resolved by Long Baseline Interferometry}",
      journal = {\apjl},
     keywords = {radiation mechanisms: non-thermal, stars: early-type, stars: individual: HD93250, stars: massive, techniques: interferometric, X-rays: individual: HD93250, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = oct,
       volume = {740},
       number = {2},
          eid = {L43},
        pages = {L43},
          doi = {10.1088/2041-8205/740/2/L43},
archivePrefix = {arXiv},
       eprint = {1110.0831},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...740L..43S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sana17,
       author = {{Sana}, H. and {Ram{\'\i}rez-Tannus}, M.~C. and {de Koter}, A. and {Kaper}, L. and {Tramper}, F. and {Bik}, A.},
        title = "{A dearth of short-period massive binaries in the young massive star forming region M 17. Evidence for a large orbital separation at birth?}",
      journal = {\aap},
     keywords = {binaries: spectroscopic, stars: early-type, stars: formation, open clusters and associations: individual: M 17, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {L9},
        pages = {L9},
          doi = {10.1051/0004-6361/201630087},
archivePrefix = {arXiv},
       eprint = {1702.02153},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599L...9S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jb17,
       author = {{Le Bouquin}, J. -B. and {Sana}, H. and {Gosset}, E. and
         {De Becker}, M. and {Duvert}, G. and {Absil}, O. and {Anthonioz}, F. and
         {Berger}, J. -P. and {Ertel}, S. and {Grellmann}, R. and {Guieu}, S. and
         {Kervella}, P. and {Rabus}, M. and {Willson}, M.},
        title = "{Resolved astrometric orbits of ten O-type binaries}",
      journal = {\aap},
     keywords = {stars: massive, binaries: general, methods: observational, techniques: high angular resolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = may,
       volume = {601},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201629260},
archivePrefix = {arXiv},
       eprint = {1608.03525},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...601A..34L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jb17,
       author = {{Le Bouquin}, J. -B. and {Sana}, H. and {Gosset}, E. and {De Becker}, M. and {Duvert}, G. and {Absil}, O. and {Anthonioz}, F. and {Berger}, J. -P. and {Ertel}, S. and {Grellmann}, R. and {Guieu}, S. and {Kervella}, P. and {Rabus}, M. and {Willson}, M.},
        title = "{Resolved astrometric orbits of ten O-type binaries}",
      journal = {\aap},
     keywords = {stars: massive, binaries: general, methods: observational, techniques: high angular resolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = may,
       volume = {601},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201629260},
archivePrefix = {arXiv},
       eprint = {1608.03525},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...601A..34L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shenar2020,
       author = {{Shenar}, T. and {Bodensteiner}, J. and {Abdul-Masih}, M. and {Fabry}, M. and {Mahy}, L. and {Marchant}, P. and {Banyard}, G. and {Bowman}, D.~M. and {Dsilva}, K. and {Hawcroft}, C. and {Reggiani}, M. and {Sana}, H.},
        title = "{The ``hidden'' companion in LB-1 unveiled by spectral disentangling}",
      journal = {\aap},
     keywords = {stars: early-type, stars: emission-line, Be, binaries: spectroscopic, binaries: close, stars: individual: LS V+22 25, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {639},
          eid = {L6},
        pages = {L6},
          doi = {10.1051/0004-6361/202038275},
archivePrefix = {arXiv},
       eprint = {2004.12882},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...639L...6S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{julia2020,
       author = {{Bodensteiner}, J. and {Shenar}, T. and {Mahy}, L. and {Fabry}, M. and {Marchant}, P. and {Abdul-Masih}, M. and {Banyard}, G. and {Bowman}, D.~M. and {Dsilva}, K. and {Frost}, A.~J. and {Hawcroft}, C. and {Reggiani}, M. and {Sana}, H.},
        title = "{Is HR 6819 a triple system containing a black hole?. An alternative explanation}",
      journal = {\aap},
     keywords = {stars: massive, stars: early-type, stars: emission-line, Be, binaries: close, binaries: spectroscopic, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A43},
        pages = {A43},
          doi = {10.1051/0004-6361/202038682},
archivePrefix = {arXiv},
       eprint = {2006.10770},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A..43B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{julia2021,
       author = {{Bodensteiner}, J. and {Sana}, H. and {Wang}, C. and {Langer}, N. and {Mahy}, L. and {Banyard}, G. and {de Koter}, A. and {de Mink}, S.~E. and {Evans}, C.~J. and {G{\"o}tberg}, Y. and {Patrick}, L.~R. and {Schneider}, F.~R.~N. and {Tramper}, F.},
        title = "{The young massive SMC cluster NGC 330 seen by MUSE. II. Multiplicity properties of the massive-star population}",
      journal = {\aap},
     keywords = {stars: massive, stars: emission-line, Be, binaries: spectroscopic, blue stragglers, open clusters and associations: individual: NGC 330, Magellanic Clouds, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = aug,
       volume = {652},
          eid = {A70},
        pages = {A70},
          doi = {10.1051/0004-6361/202140507},
archivePrefix = {arXiv},
       eprint = {2104.13409},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...652A..70B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ricker,
       author = {{Ricker}, George R. and {Winn}, Joshua N. and {Vanderspek}, Roland and {Latham}, David W. and {Bakos}, G{\'a}sp{\'a}r {\'A}. and {Bean}, Jacob L. and {Berta-Thompson}, Zachory K. and {Brown}, Timothy M. and {Buchhave}, Lars and {Butler}, Nathaniel R. and {Butler}, R. Paul and {Chaplin}, William J. and {Charbonneau}, David and {Christensen-Dalsgaard}, J{\o}rgen and {Clampin}, Mark and {Deming}, Drake and {Doty}, John and {De Lee}, Nathan and {Dressing}, Courtney and {Dunham}, Edward W. and {Endl}, Michael and {Fressin}, Francois and {Ge}, Jian and {Henning}, Thomas and {Holman}, Matthew J. and {Howard}, Andrew W. and {Ida}, Shigeru and {Jenkins}, Jon M. and {Jernigan}, Garrett and {Johnson}, John Asher and {Kaltenegger}, Lisa and {Kawai}, Nobuyuki and {Kjeldsen}, Hans and {Laughlin}, Gregory and {Levine}, Alan M. and {Lin}, Douglas and {Lissauer}, Jack J. and {MacQueen}, Phillip and {Marcy}, Geoffrey and {McCullough}, Peter R. and {Morton}, Timothy D. and {Narita}, Norio and {Paegert}, Martin and {Palle}, Enric and {Pepe}, Francesco and {Pepper}, Joshua and {Quirrenbach}, Andreas and {Rinehart}, Stephen A. and {Sasselov}, Dimitar and {Sato}, Bun'ei and {Seager}, Sara and {Sozzetti}, Alessandro and {Stassun}, Keivan G. and {Sullivan}, Peter and {Szentgyorgyi}, Andrew and {Torres}, Guillermo and {Udry}, Stephane and {Villasenor}, Joel},
        title = "{Transiting Exoplanet Survey Satellite (TESS)}",
      journal = {Journal of Astronomical Telescopes, Instruments, and Systems},
         year = 2015,
        month = jan,
       volume = {1},
          eid = {014003},
        pages = {014003},
          doi = {10.1117/1.JATIS.1.1.014003},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015JATIS...1a4003R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{gravpipe,
       author = {{Lapeyrere}, V. and {Kervella}, P. and {Lacour}, S. and {Azouaoui}, N. and
         {Garcia-Dabo}, C.~E. and {Perrin}, G. and {Eisenhauer}, F. and
         {Perraut}, K. and {Straubmeier}, C. and {Amorim}, A. and {Brandner}, W.},
        title = "{GRAVITY data reduction software}",
    booktitle = {\procspie},
         year = 2014,
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9146},
        month = jul,
          eid = {91462D},
        pages = {91462D},
          doi = {10.1117/12.2056850},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SPIE.9146E..2DL},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze10,
       author = {{Naz{\'e}}, Y. and {Ud-Doula}, A. and {Spano}, M. and {Rauw}, G. and
         {De Becker}, M. and {Walborn}, N.~R.},
        title = "{New findings on the prototypical Of?p stars}",
      journal = {\aap},
     keywords = {X-rays: stars, stars: individual: HD 108, stars: individual: HD 148937, stars: individual: HD 191612, stars: emission-line, Be, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = sep,
       volume = {520},
          eid = {A59},
        pages = {A59},
          doi = {10.1051/0004-6361/201014333},
archivePrefix = {arXiv},
       eprint = {1006.2054},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...520A..59N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{georgy17,
       author = {{Georgy}, Cyril and {Meynet}, Georges and {Ekstr{\"o}m}, Sylvia and
         {Wade}, Gregg A. and {Petit}, V{\'e}ronique and {Keszthelyi}, Zsolt and
         {Hirschi}, Raphael},
        title = "{Possible pair-instability supernovae at solar metallicity from magnetic stellar progenitors}",
      journal = {\aap},
     keywords = {stars: evolution, stars: magnetic field, stars: massive, stars: mass-loss, supernovae: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {L5},
        pages = {L5},
          doi = {10.1051/0004-6361/201730401},
archivePrefix = {arXiv},
       eprint = {1702.02340},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599L...5G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{edibles,
       author = {{Cox}, Nick L.~J. and {Cami}, Jan and {Farhang}, Amin and
         {Smoker}, Jonathan and {Monreal-Ibero}, Ana and {Lallement}, Rosine and
         {Sarre}, Peter J. and {Marshall}, Charlotte C.~M. and
         {Smith}, Keith T. and {Evans}, Christopher J. and {Royer}, Pierre and
         {Linnartz}, Harold and {Cordiner}, Martin A. and {Joblin}, Christine and
         {van Loon}, Jacco Th. and {Foing}, Bernard H. and {Bhatt}, Neil H. and
         {Bron}, Emeric and {Elyajouri}, Meriem and {de Koter}, Alex and
         {Ehrenfreund}, Pascale and {Javadi}, Atefeh and {Kaper}, Lex and
         {Khosroshadi}, Habib G. and {Laverick}, Mike and {Le Petit}, Franck and
         {Mulas}, Giacomo and {Roueff}, Evelyne and {Salama}, Farid and
         {Spaans}, Marco},
        title = "{The ESO Diffuse Interstellar Bands Large Exploration Survey (EDIBLES) . I. Project description, survey sample, and quality assessment}",
      journal = {\aap},
     keywords = {ISM: lines and bands, ISM: clouds, ISM: molecules, dust, extinction, stars: early-type, local insterstellar matter, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = oct,
       volume = {606},
          eid = {A76},
        pages = {A76},
          doi = {10.1051/0004-6361/201730912},
archivePrefix = {arXiv},
       eprint = {1708.01429},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...606A..76C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{langerrev,
       author = {{Langer}, N.},
        title = "{Presupernova Evolution of Massive Single and Binary Stars}",
      journal = {\araa},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = sep,
       volume = {50},
        pages = {107-164},
          doi = {10.1146/annurev-astro-081811-125534},
archivePrefix = {arXiv},
       eprint = {1206.5443},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ARA&A..50..107L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mahy17,
       author = {{Mahy}, L. and {Hutsem{\'e}kers}, D. and {Naz{\'e}}, Y. and {Royer}, P. and
         {Lebouteiller}, V. and {Waelkens}, C.},
        title = "{Evolutionary status of the Of?p star HD 148937 and of its surrounding nebula NGC 6164/5}",
      journal = {\aap},
     keywords = {infrared: stars, stars: individual: HD 148937, ISM: individual objects: NGC 6164/5, stars: abundances, circumstellar matter, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {A61},
        pages = {A61},
          doi = {10.1051/0004-6361/201629585},
archivePrefix = {arXiv},
       eprint = {1611.07257},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599A..61M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hubrig11,
       author = {{Hubrig}, S. and {Sch{\"o}ller}, M. and {Kharchenko}, N.~V. and
         {Langer}, N. and {de Wit}, W.~J. and {Ilyin}, I. and
         {Kholtygin}, A.~F. and {Piskunov}, A.~E. and {Przybilla}, N. and
         {Magori Collaboration}},
        title = "{Exploring the origin of magnetic fields in massive stars: a survey of O-type stars in clusters and in the field}",
      journal = {\aap},
     keywords = {polarization, stars: magnetic field, stars: kinematics and dynamics, open clusters and associations: general, stars: early-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = apr,
       volume = {528},
          eid = {A151},
        pages = {A151},
          doi = {10.1051/0004-6361/201016345},
archivePrefix = {arXiv},
       eprint = {1102.2503},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...528A.151H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wade12,
       author = {{Wade}, G.~A. and {Grunhut}, J. and {Gr{\"a}fener}, G. and
         {Howarth}, I.~D. and {Martins}, F. and {Petit}, V. and {Vink}, J.~S. and
         {Bagnulo}, S. and {Folsom}, C.~P. and {Naz{\'e}}, Y. and
         {Walborn}, N.~R. and {Townsend}, R.~H.~D. and {Evans}, C.~J.},
        title = "{The spectral variability and magnetic field characteristics of the Of?p star HD 148937}",
      journal = {\mnras},
     keywords = {binaries: spectroscopic, stars: early-type, stars: magnetic fields, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jan,
       volume = {419},
       number = {3},
        pages = {2459-2471},
          doi = {10.1111/j.1365-2966.2011.19897.x},
archivePrefix = {arXiv},
       eprint = {1108.4847},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.419.2459W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petit17,
       author = {{Petit}, V. and {Keszthelyi}, Z. and {MacInnis}, R. and {Cohen}, D.~H. and
         {Townsend}, R.~H.~D. and {Wade}, G.~A. and {Thomas}, S.~L. and
         {Owocki}, S.~P. and {Puls}, J. and {ud-Doula}, A.},
        title = "{Magnetic massive stars as progenitors of `heavy' stellar-mass black holes}",
      journal = {\mnras},
     keywords = {stars: black holes, stars: early-type, stars: evolution, stars: magnetic field, stars: massive, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {466},
       number = {1},
        pages = {1052-1060},
          doi = {10.1093/mnras/stw3126},
archivePrefix = {arXiv},
       eprint = {1611.08964},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.1052P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{donati02,
       author = {{Donati}, J. -F. and {Babel}, J. and {Harries}, T.~J. and
         {Howarth}, I.~D. and {Petit}, P. and {Semel}, M.},
        title = "{The magnetic field and wind confinement of {\ensuremath{\theta}}$^{1}$ Orionis C}",
      journal = {\mnras},
     keywords = {stars: individual: {\ensuremath{\theta}}1 Ori C, stars: magnetic fields, stars: rotation, stars: winds, outflows},
         year = 2002,
        month = jun,
       volume = {333},
       number = {1},
        pages = {55-70},
          doi = {10.1046/j.1365-8711.2002.05379.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.333...55D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{leith,
   author = {{Leitherer}, C.},
    title = "{Massive Stars in Starburst Galaxies and the Origin of Galactic Superwinds.}",
booktitle = {Reviews in Modern Astronomy},
     year = 1994,
   series = {Reviews in Modern Astronomy},
   volume = 7,
   editor = {{Klare}, G.},
    pages = {73-102},
   adsurl = {http://adsabs.harvard.edu/abs/1994RvMA....7...73L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{oiutils1,
       author = {{Kervella}, P. and {Bigot}, L. and {Gallenne}, A. and {Th{\'e}venin}, F.},
        title = "{The radii and limb darkenings of {\ensuremath{\alpha}} Centauri A and B . Interferometric measurements with VLTI/PIONIER}",
      journal = {\aap},
     keywords = {stars: individual: Alpha Centauri, techniques: interferometric, stars: solar-type, stars: fundamental parameters, binaries: visual, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {597},
          eid = {A137},
        pages = {A137},
          doi = {10.1051/0004-6361/201629505},
archivePrefix = {arXiv},
       eprint = {1610.06185},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...597A.137K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{oiutils2,
       author = {{Liu}, Hauyu Baobab and {M{\'e}rand}, Antoine and {Green}, Joel D. and
         {P{\'e}rez}, Sebasti{\'a}n and {Hales}, Antonio S. and {Yang}, Yao-Lun and
         {Dunham}, Michael M. and {Hasegawa}, Yasuhiro and {Henning}, Thomas and
         {Galv{\'a}n-Madrid}, Roberto and {K{\'o}sp{\'a}l}, {\'A}gnes and
         {Takami}, Michihiro and {Vorobyov}, Eduard I. and {Zhu}, Zhaohuan},
        title = "{Diagnosing 0.1-10 au Scale Morphology of the FU Ori Disk Using ALMA and VLTI/GRAVITY}",
      journal = {\apj},
     keywords = {protoplanetary disks, stars: individual: FU Ori, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {884},
       number = {1},
          eid = {97},
        pages = {97},
          doi = {10.3847/1538-4357/ab391c},
archivePrefix = {arXiv},
       eprint = {1908.02981},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884...97L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{gravity,
       author = {{Eisenhauer}, F. and {Perrin}, G. and {Brandner}, W. and
         {Straubmeier}, C. and {Perraut}, K. and {Amorim}, A. and
         {Sch{\"o}ller}, M. and {Gillessen}, S. and {Kervella}, P. and
         {Benisty}, M. and {Araujo-Hauck}, C. and {Jocou}, L. and {Lima}, J. and
         {Jakob}, G. and {Haug}, M. and {Cl{\'e}net}, Y. and {Henning}, T. and
         {Eckart}, A. and {Berger}, J. -P. and {Garcia}, P. and {Abuter}, R. and
         {Kellner}, S. and {Paumard}, T. and {Hippler}, S. and {Fischer}, S. and
         {Moulin}, T. and {Villate}, J. and {Avila}, G. and {Gr{\"a}ter}, A. and
         {Lacour}, S. and {Huber}, A. and {Wiest}, M. and {Nolot}, A. and
         {Carvas}, P. and {Dorn}, R. and {Pfuhl}, O. and {Gendron}, E. and
         {Kendrew}, S. and {Yazici}, S. and {Anton}, S. and {Jung}, Y. and
         {Thiel}, M. and {Choquet}, {\'E}. and {Klein}, R. and {Teixeira}, P. and
         {Gitton}, P. and {Moch}, D. and {Vincent}, F. and {Kudryavtseva}, N. and
         {Str{\"o}bele}, S. and {Sturm}, S. and {F{\'e}dou}, P. and
         {Lenzen}, R. and {Jolley}, P. and {Kister}, C. and {Lapeyr{\`e}re}, V. and
         {Naranjo}, V. and {Lucuix}, C. and {Hofmann}, R. and {Chapron}, F. and
         {Neumann}, U. and {Mehrgan}, L. and {Hans}, O. and {Rousset}, G. and
         {Ramos}, J. and {Suarez}, M. and {Lederer}, R. and {Reess}, J. -M. and
         {Rohloff}, R. -R. and {Haguenauer}, P. and {Bartko}, H. and
         {Sevin}, A. and {Wagner}, K. and {Lizon}, J. -L. and {Rabien}, S. and
         {Collin}, C. and {Finger}, G. and {Davies}, R. and {Rouan}, D. and
         {Wittkowski}, M. and {Dodds-Eden}, K. and {Ziegler}, D. and
         {Cassaing}, F. and {Bonnet}, H. and {Casali}, M. and {Genzel}, R. and
         {Lena}, P.},
        title = "{GRAVITY: Observing the Universe in Motion}",
      journal = {The Messenger},
         year = 2011,
        month = mar,
       volume = {143},
        pages = {16-24},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011Msngr.143...16E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{vlti,
       author = {{Haguenauer}, Pierre and {Alonso}, Jaime and {Bourget}, Pierre and
         {Brillant}, Stephane and {Gitton}, Philippe and {Guisard}, Stephane and
         {Poupar}, S{\'e}bastien and {Schuhler}, Nicolas and {Abuter}, Roberto and
         {Andolfato}, Luigi and {Blanchard}, Guillaume and
         {Berger}, Jean-Philippe and {Cortes}, Angela and
         {D{\'e}rie}, Fr{\'e}d{\'e}ric and {Delplancke}, Fran{\c{c}}oise and
         {Di Lieto}, Nicola and {Dupuy}, Christophe and {Gilli}, Bruno and
         {Glindemann}, Andreas and {Guniat}, Serge and {Huedepohl}, Gerhard and
         {Kaufer}, Andreas and {Le Bouquin}, Jean-Baptiste and
         {L{\'e}vque}, Samuel and {M{\'e}nardi}, Serge and {M{\'e}rand
        }, Antoine and {Morel}, Sebastien and {Percheron}, Isabelle and
         {Phan Duc}, Than and {Pino}, Andres and {Ramirez}, Andres and
         {Rengaswamy}, Sridharan and {Richichi}, Andrea and {Rivinius}, Thomas and
         {Sahlmann}, Johannes and {Schoeller}, Markus and {Schmid}, Christian and
         {Stefl}, Stan and {Valdes}, Guillermo and {van Belle}, Gerard and
         {Wehner}, Stefan and {Wittkowski}, Markus},
        title = "{The very large telescope Interferometer: 2010 edition}",
    booktitle = {\procspie},
         year = 2010,
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7734},
        month = jul,
          eid = {773404},
        pages = {773404},
          doi = {10.1117/12.857070},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010SPIE.7734E..04H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{pionier,
       author = {{Le Bouquin}, J. -B. and {Berger}, J. -P. and {Lazareff}, B. and
         {Zins}, G. and {Haguenauer}, P. and {Jocou}, L. and {Kern}, P. and
         {Millan-Gabet}, R. and {Traub}, W. and {Absil}, O. and
         {Augereau}, J. -C. and {Benisty}, M. and {Blind}, N. and {Bonfils}, X. and
         {Bourget}, P. and {Delboulbe}, A. and {Feautrier}, P. and
         {Germain}, M. and {Gitton}, P. and {Gillier}, D. and {Kiekebusch}, M. and
         {Kluska}, J. and {Knudstrup}, J. and {Labeye}, P. and {Lizon}, J. -L. and
         {Monin}, J. -L. and {Magnard}, Y. and {Malbet}, F. and {Maurel}, D. and
         {M{\'e}nard}, F. and {Micallef}, M. and {Michaud}, L. and
         {Montagnier}, G. and {Morel}, S. and {Moulin}, T. and {Perraut}, K. and
         {Popovic}, D. and {Rabou}, P. and {Rochat}, S. and {Rojas}, C. and
         {Roussel}, F. and {Roux}, A. and {Stadler}, E. and {Stefl}, S. and
         {Tatulli}, E. and {Ventura}, N.},
        title = "{PIONIER: a 4-telescope visitor instrument at VLTI}",
      journal = {\aap},
     keywords = {instrumentation: interferometers, techniques: interferometric, techniques: high angular resolution, instrumentation: high angular resolution, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = nov,
       volume = {535},
          eid = {A67},
        pages = {A67},
          doi = {10.1051/0004-6361/201117586},
archivePrefix = {arXiv},
       eprint = {1109.1918},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...535A..67L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hadrava95,
       author = {{Hadrava}, P.},
        title = "{Orbital elements of multiple spectroscopic stars.}",
      journal = {\aaps},
     keywords = {STARS: BINARIES SPECTROSCOPIC, METHODS: NUMERICAL},
         year = 1995,
        month = dec,
       volume = {114},
        pages = {393},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995A&AS..114..393H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mahy10,
       author = {{Mahy}, L. and {Rauw}, G. and {Martins}, F. and {Naz{\'e}}, Y. and {Gosset}, E. and {De Becker}, M. and {Sana}, H. and {Eenens}, P.},
        title = "{A New Investigation of the Binary HD 48099}",
      journal = {\apj},
     keywords = {binaries: spectroscopic, stars: fundamental parameters, stars: individual: HD 48099, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = jan,
       volume = {708},
       number = {2},
        pages = {1537-1544},
          doi = {10.1088/0004-637X/708/2/1537},
archivePrefix = {arXiv},
       eprint = {0912.0605},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...708.1537M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mahy11,
       author = {{Mahy}, L. and {Martins}, F. and {Machado}, C. and {Donati}, J. -F. and {Bouret}, J. -C.},
        title = "{The two components of the evolved massive binary LZ Cephei. Testing the effects of binarity on stellar evolution}",
      journal = {\aap},
     keywords = {stars: early-type, binaries: general, stars: fundamental parameters, stars: winds, outflows, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = sep,
       volume = {533},
          eid = {A9},
        pages = {A9},
          doi = {10.1051/0004-6361/201116993},
archivePrefix = {arXiv},
       eprint = {1106.6162},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...533A...9M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martins17,
       author = {{Martins}, F. and {Mahy}, L. and {Herv{\'e}}, A.},
        title = "{Properties of six short-period massive binaries: A study of the effects of binarity on surface chemical abundances}",
      journal = {\aap},
     keywords = {stars: massive, binaries: close, binaries: spectroscopic, stars: atmospheres, stars: abundances, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = nov,
       volume = {607},
          eid = {A82},
        pages = {A82},
          doi = {10.1051/0004-6361/201731593},
archivePrefix = {arXiv},
       eprint = {1709.00937},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...607A..82M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{marchenko98,
       author = {{Marchenko}, Sergey V. and {Moffat}, Anthony F.~J. and {Eenens}, Philippe R.~J.},
        title = "{The Wolf-Rayet Binary WR 141 (WN5O + O5 V-III) Revisited}",
      journal = {\pasp},
     keywords = {STARS: BINARIES: SPECTROSCOPIC, STARS: WOLF-RAYET, STARS: INDIVIDUAL: ALPHANUMERIC: WR 141},
         year = 1998,
        month = dec,
       volume = {110},
       number = {754},
        pages = {1416-1422},
          doi = {10.1086/316280},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998PASP..110.1416M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gonzalez06,
       author = {{Gonz{\'a}lez}, J.~F. and {Levato}, H.},
        title = "{Separation of composite spectra: the spectroscopic detection of an eclipsing binary star}",
      journal = {\aap},
     keywords = {techniques: radial velocities, stars: binaries: spectroscopic, stars: fundamental parameters, stars: individual: HD 143511, Galaxy: open clusters and associations: individual: NGC 6025},
         year = 2006,
        month = mar,
       volume = {448},
       number = {1},
        pages = {283-292},
          doi = {10.1051/0004-6361:20053177},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...448..283G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{demink14,
       author = {{de Mink}, S.~E. and {Sana}, H. and {Langer}, N. and {Izzard}, R.~G. and {Schneider}, F.~R.~N.},
        title = "{The Incidence of Stellar Mergers and Mass Gainers among Massive Stars}",
      journal = {\apj},
     keywords = {binaries: close, Galaxy: stellar content, stars: early-type, stars: massive, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = feb,
       volume = {782},
       number = {1},
          eid = {7},
        pages = {7},
          doi = {10.1088/0004-637X/782/1/7},
archivePrefix = {arXiv},
       eprint = {1312.3650},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...782....7D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lb1tomer,
       author = {{Shenar}, T. and {Bodensteiner}, J. and {Abdul-Masih}, M. and {Fabry}, M. and {Mahy}, L. and {Marchant}, P. and {Banyard}, G. and {Bowman}, D.~M. and {Dsilva}, K. and {Hawcroft}, C. and {Reggiani}, M. and {Sana}, H.},
        title = "{The ``hidden'' companion in LB-1 unveiled by spectral disentangling}",
      journal = {\aap},
     keywords = {stars: early-type, stars: emission-line, Be, binaries: spectroscopic, binaries: close, stars: individual: LS V+22 25, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {639},
          eid = {L6},
        pages = {L6},
          doi = {10.1051/0004-6361/202038275},
archivePrefix = {arXiv},
       eprint = {2004.12882},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...639L...6S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{laurent22,
       author = {{Mahy}, L. and {Sana}, H. and {Shenar}, T. and {Sen}, K. and {Langer}, N. and {Marchant}, P. and {Abdul-Masih}, M. and {Banyard}, G. and {Bodensteiner}, J. and {Bowman}, D.~M. and {Dsilva}, K. and {Fabry}, M. and {Hawcroft}, C. and {Janssens}, S. and {Van Reeth}, T. and {Eldridge}, C.},
        title = "{Identifying quiescent compact objects in massive Galactic single-lined spectroscopic binaries}",
      journal = {\aap},
     keywords = {binaries: general, binaries: spectroscopic, stars: early-type, stars: evolution, stars: black holes, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2022,
        month = aug,
       volume = {664},
          eid = {A159},
        pages = {A159},
          doi = {10.1051/0004-6361/202243147},
archivePrefix = {arXiv},
       eprint = {2207.07752},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...664A.159M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{simondiaz14,
       author = {{Sim{\'o}n-D{\'\i}az}, S. and {Herrero}, A.},
        title = "{The IACOB project. I. Rotational velocities in northern Galactic O- and early B-type stars revisited. The impact of other sources of line-broadening}",
      journal = {\aap},
     keywords = {stars: early-type, stars: rotation, techniques: spectroscopic, line: profiles, astronomical databases: miscellaneous, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = feb,
       volume = {562},
          eid = {A135},
        pages = {A135},
          doi = {10.1051/0004-6361/201322758},
archivePrefix = {arXiv},
       eprint = {1311.3360},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...562A.135S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{fabry2021,
       author = {Fabry, M. and {Crawford}, C. and {Mahy}, L. and {Marchant}, P.  and {Bouquin}, L.~B.  and {Sana}, H. },
        title = "{Mass discrepancy in 9 Sgr}",
      journal = {\aap},
     keywords = {stars: early-type, stars: individual (9 Sgr)},
         year = {subm.},
        month = Feb,
       volume = {},
          eid = {subm.},
        pages = (subm.)
        }
        
@INPROCEEDINGS{wade09a,
       author = {{Wade}, Gregg A. and {Alecian}, E. and {Bohlender}, D.~A. and {Bouret}, J. -C. and {Grunhut}, J.~H. and {Henrichs}, H. and {Neiner}, C. and {Petit}, V. and {Louis}, N. St. and {Auri{\`e}re}, M. and {Kochukhov}, O. and {Silvester}, J. and {ud-Doula}, A. and {ud-Doula}},
        title = "{The MiMeS project: magnetism in massive stars}",
     keywords = {Magnetic fields, massive stars, hot stars, star formation, stellar evolution, stellar winds, spectropolarimetry, Astrophysics},
    booktitle = {Cosmic Magnetic Fields: From Planets, to Stars and Galaxies},
         year = 2009,
       editor = {{Strassmeier}, Klaus G. and {Kosovichev}, Alexander G. and {Beckman}, John E.},
       volume = {259},
        month = apr,
        pages = {333-338},
          doi = {10.1017/S1743921309030695},
archivePrefix = {arXiv},
       eprint = {0812.4078},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009IAUS..259..333W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
        
@ARTICLE{bodensteiner2021,
       author = {Bodensteiner, J. and {Sana}, H. and {Mahy}, L. and {Wang}, C.  and {Langer}, N.  and {De Mink}, S. },
        title = "{NGC 330: binarityr}",
      journal = {\aap},
     keywords = {stars: early-type, stars: individual (NGC330)},
         year = {subm.},
        month = Feb,
       volume = {},
          eid = (subm.),
        pages = (subm.)
        }
        
@ARTICLE{nazehd108,
       author = {{Naz{\'e}}, Y. and {Walborn}, N.~R. and {Martins}, F.},
        title = "{The mysterious Of?p class and the magnetic O-star {\ensuremath{\theta}}$^{1}$ Ori C: confronting observations}",
      journal = {\rmxaa},
     keywords = {stars: early-type, stars: individual (HD 108, HD 148937, HD 191612, {\ensuremath{\theta}} 1 Ori C), stars: variables: other, Astrophysics},
         year = 2008,
        month = oct,
       volume = {44},
        pages = {331-340},
archivePrefix = {arXiv},
       eprint = {0807.3496},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008RMxAA..44..331N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{powr,
       author = {{Sander}, A. and {Shenar}, T. and {Hainich}, R. and {G{\'\i}menez-Garc{\'\i}a}, A. and {Todt}, H. and {Hamann}, W. -R.},
        title = "{On the consistent treatment of the quasi-hydrostatic layers in hot star atmospheres}",
      journal = {\aap},
     keywords = {stars: early-type, stars: mass-loss, stars: winds, outflows, stars: atmospheres, stars: fundamental parameters, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = may,
       volume = {577},
          eid = {A13},
        pages = {A13},
          doi = {10.1051/0004-6361/201425356},
archivePrefix = {arXiv},
       eprint = {1503.01338},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...577A..13S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hirai,
       author = {{Hirai}, Ryosuke and {Podsiadlowski}, Philipp and {Owocki}, Stanley P. and {Schneider}, Fabian R.~N. and {Smith}, Nathan},
        title = "{Modelling Eta Carinae's Great Eruption and its surrounding nebula}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = nov,
          eid = {arXiv:2011.12434},
        pages = {arXiv:2011.12434},
archivePrefix = {arXiv},
       eprint = {2011.12434},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201112434H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Article{glebbeek08,
  Title                    = {{Evolution of stellar collision products in open clusters. II. A grid of low-mass collisions}},
  Author                   = {{Glebbeek}, E. and {Pols}, O.~R.},
  Journal                  = {\aap},
  Year                     = {2008},

  Month                    = sep,
  Pages                    = {1017-1025},
  Volume                   = {488},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2008A%26A...488.1017G},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1051/0004-6361:200809931},
  Eprint                   = {0806.0865},
  File                     = {Published version:2008A&A...488.1017G.pdf:PDF},
  Keywords                 = {stars: blue stragglers, stars: formation, methods: numerical, methods: N-body simulations, Galaxy: open clusters and associations: general}
}


@Article{glebbeek13,
  Title                    = {{Structure and evolution of high-mass stellar mergers}},
  Author                   = {{Glebbeek}, E. and {Gaburov}, E. and {Portegies Zwart}, S. and {Pols}, O.~R.},
  Journal                  = {\mnras},
  Year                     = {2013},

  Month                    = oct,
  Pages                    = {3497-3510},
  Volume                   = {434},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2013MNRAS.434.3497G},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1093/mnras/stt1268},
  Eprint                   = {1307.2445},
  File                     = {Published version:2013MNRAS.434.3497G.pdf:PDF},
  Keywords                 = {blue stragglers, stars: evolution, stars: general, stars: interior, globular clusters: general},
  Primaryclass             = {astro-ph.SR}
}


@Article{fab15,
  Title                    = {{Evolution of Mass Functions of Coeval Stars through Wind Mass Loss and Binary Interactions}},
  Author                   = {{Schneider}, F.~R.~N. and {Izzard}, R.~G. and {Langer}, N. and {de Mink}, S.~E.},
  Journal                  = {\apj},
  Year                     = {2015},

  Month                    = may,
  Pages                    = {20},
  Volume                   = {805},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2015ApJ...805...20S},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1088/0004-637X/805/1/20},
  Eid                      = {20},
  Eprint                   = {1504.01735},
  File                     = {Published version:2015ApJ...805...20S.pdf:PDF},
  Keywords                 = {binaries: general, blue stragglers, stars: luminosity function, mass function, stars: mass-loss},
  Primaryclass             = {astro-ph.SR}
}


@Article{fab16,
  Title                    = {{Rejuvenation of stellar mergers and the origin of magnetic fields in massive stars}},
  Author                   = {{Schneider}, F.~R.~N. and {Podsiadlowski}, P. and {Langer}, N. and {Castro}, N. and {Fossati}, L.},
  Journal                  = {\mnras},
  Year                     = {2016},

  Month                    = apr,
  Pages                    = {2355-2365},
  Volume                   = {457},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2016MNRAS.457.2355S},
  Archiveprefix            = {arXiv},
  Doi                      = {10.1093/mnras/stw148},
  Eprint                   = {1601.05084},
  File                     = {Published version:2016MNRAS.457.2355S.pdf:PDF},
  Keywords                 = {binaries: general, blue stragglers, stars: general, stars: individual: {$\tau$} Sco, stars: individual: HR 2949},
  Primaryclass             = {astro-ph.SR}
}


@ARTICLE{fab20,
       author = {{Schneider}, F.~R.~N. and {Ohlmann}, S.~T. and {Podsiadlowski}, Ph and {R{\"o}pke}, F.~K. and {Balbus}, S.~A. and {Pakmor}, R.},
        title = "{Long-term evolution of a magnetic massive merger product}",
      journal = {\mnras},
     keywords = {binaries: general, blue stragglers, stars: evolution, stars: individual: {\ensuremath{\tau}} Sco, stars: magnetic field, stars: massive, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = may,
       volume = {495},
       number = {3},
        pages = {2796-2812},
          doi = {10.1093/mnras/staa1326},
archivePrefix = {arXiv},
       eprint = {2005.05335},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.495.2796S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fabnat,
       author = {{Schneider}, Fabian R.~N. and {Ohlmann}, Sebastian T. and {Podsiadlowski}, Philipp and {R{\"o}pke}, Friedrich K. and {Balbus}, Steven A. and {Pakmor}, R{\"u}diger and {Springel}, Volker},
        title = "{Stellar mergers as the origin of magnetic massive stars}",
      journal = {\nat},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = oct,
       volume = {574},
       number = {7777},
        pages = {211-214},
          doi = {10.1038/s41586-019-1621-5},
archivePrefix = {arXiv},
       eprint = {1910.14058},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019Natur.574..211S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Article{morris06,
  Title                    = {{Anisotropic mass ejection in binary mergers}},
  Author                   = {{Morris}, T. and {Podsiadlowski}, P.},
  Journal                  = {\mnras},
  Year                     = {2006},

  Month                    = jan,
  Pages                    = {2-10},
  Volume                   = {365},

  Adsnote                  = {Provided by the SAO/NASA Astrophysics Data System},
  Adsurl                   = {http://adsabs.harvard.edu/abs/2006MNRAS.365....2M},
  Doi                      = {10.1111/j.1365-2966.2005.09645.x},
  Eprint                   = {astro-ph/0502288},
  File                     = {:2006MNRAS.365....2M.pdf:PDF},
  Keywords                 = {hydrodynamics, binaries: close, circumstellar matter, supernovae: individual: SN1987A}
}


@Article{macleod18,
  author        = {{MacLeod}, Morgan and {Ostriker}, Eve C. and {Stone}, James M.},
  title         = {{Bound Outflows, Unbound Ejecta, and the Shaping of Bipolar Remnants during Stellar Coalescence}},
  journal       = {\apj},
  year          = {2018},
  volume        = {868},
  number        = {2},
  pages         = {136},
  month         = {Dec},
  adsnote       = {Provided by the SAO/NASA Astrophysics Data System},
  adsurl        = {https://ui.adsabs.harvard.edu/abs/2018ApJ...868..136M},
  archiveprefix = {arXiv},
  doi           = {10.3847/1538-4357/aae9eb},
  eid           = {136},
  eprint        = {1808.05950},
  file          = {:2018ApJ...868..136M.pdf:PDF},
  keywords      = {binaries: close, hydrodynamics, methods: numerical, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
  primaryclass  = {astro-ph.SR},
}


@ARTICLE{wade19,
       author = {{Wade}, G.~A. and {Smoker}, J.~V. and {Evans}, C.~J. and
         {Howarth}, I.~D. and {Barba}, R. and {Cox}, N.~L.~J. and {Morrell}, N. and
         {Naz{\'e}}, Y. and {Cami}, J. and {Farhang}, A. and {Walborn}, N.~R. and
         {Arias}, J. and {Gamen}, R.},
        title = "{A remarkable change of the spectrum of the magnetic Of?p star HD 148937 reveals evidence of an eccentric, high-mass binary}",
      journal = {\mnras},
     keywords = {binaries: spectroscopic, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {483},
       number = {2},
        pages = {2581-2591},
          doi = {10.1093/mnras/sty3304},
archivePrefix = {arXiv},
       eprint = {1811.11153},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483.2581W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{zin02,
       author = {{Zinnecker}, Hans},
        title = "{Formation of massive binaries}",
     keywords = {Astrophysics},
    booktitle = {A Massive Star Odyssey: From Main Sequence to Supernova},
         year = 2003,
       editor = {{van der Hucht}, Karel and {Herrero}, Artemio and {Esteban}, C{\'e}sar},
       volume = {212},
        month = jan,
        pages = {80},
archivePrefix = {arXiv},
       eprint = {astro-ph/0301078},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003IAUS..212...80Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moss,
       author = {{Moss}, D.},
        title = "{The survival of fossil magnetic fields during pre-main sequence evolution}",
      journal = {\aap},
     keywords = {magnetic fields, magnetohydrodynamics (MHD), stars: evolution, stars: chemically peculiar},
         year = 2003,
        month = may,
       volume = {403},
        pages = {693-697},
          doi = {10.1051/0004-6361:20030431},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...403..693M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{laurenthd,
       author = {{Mahy}, L. and {Hutsem{\'e}kers}, D. and {Naz{\'e}}, Y. and {Royer}, P. and
         {Lebouteiller}, V. and {Waelkens}, C.},
        title = "{Evolutionary status of the Of?p star HD 148937 and of its surrounding nebula NGC 6164/5}",
      journal = {\aap},
     keywords = {infrared: stars, stars: individual: HD 148937, ISM: individual objects: NGC 6164/5, stars: abundances, circumstellar matter, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {A61},
        pages = {A61},
          doi = {10.1051/0004-6361/201629585},
archivePrefix = {arXiv},
       eprint = {1611.07257},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599A..61M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{sana12,
       author = {{Sana}, H. and {Dunstall}, P.~R. and {H{\'e}nault-Brunet}, V. and {Walborn}, N.~R. and {de Koter}, A. and {de Mink}, S.~E. and {Dufton}, P.~L. and {Evans}, C.~J. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Taylor}, W.~D. and {Vink}, J.~S.},
        title = "{The VLT-FLAMES Tarantula Survey: Multiplicity and Dynamics of the Massive Stars in 30 Dor}",
    booktitle = {Proceedings of a Scientific Meeting in Honor of Anthony F. J. Moffat},
         year = 2012,
       editor = {{Drissen}, L. and {Robert}, C. and {St-Louis}, N. and {Moffat}, A.~F.~J.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {465},
        month = dec,
        pages = {284},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ASPC..465..284S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smash,
       author = {{Sana}, H. and {Le Bouquin}, J. -B. and {Lacour}, S. and
         {Berger}, J. -P. and {Duvert}, G. and {Gauchet}, L. and {Norris}, B. and
         {Olofsson}, J. and {Pickel}, D. and {Zins}, G. and {Absil}, O. and
         {de Koter}, A. and {Kratter}, K. and {Schnurr}, O. and {Zinnecker}, H.},
        title = "{Southern Massive Stars at High Angular Resolution: Observational Campaign and Companion Detection}",
      journal = {\apjs},
     keywords = {binaries: visual, stars: early-type, stars: imaging, surveys, techniques: high angular resolution, techniques: interferometric, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = nov,
       volume = {215},
       number = {1},
          eid = {15},
        pages = {15},
          doi = {10.1088/0067-0049/215/1/15},
archivePrefix = {arXiv},
       eprint = {1409.6304},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJS..215...15S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{walborn72,
       author = {{Walborn}, N.~R.},
        title = "{Spectral classification of OB stars in both hemispheres and the absolute-magnitude calibration.}",
      journal = {\aj},
         year = 1972,
        month = may,
       volume = {77},
        pages = {312-318},
          doi = {10.1086/111285},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1972AJ.....77..312W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze08,
       author = {{Naz{\'e}}, Ya{\"e}l and {Walborn}, Nolan R. and {Rauw}, Gregor and
         {Martins}, Fabrice and {Pollock}, A.~M.~T. and {Bond}, Howard E.},
        title = "{HD 148937: A Multiwavelength Study of the Third Galactic Member of the Of?p Class}",
      journal = {\aj},
     keywords = {stars: early-type, stars: individual: HD 148937, X-rays: individual: HD 148937, X-rays: stars, Astrophysics},
         year = 2008,
        month = may,
       volume = {135},
       number = {5},
        pages = {1946-1957},
          doi = {10.1088/0004-6256/135/5/1946},
archivePrefix = {arXiv},
       eprint = {0803.0605},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008AJ....135.1946N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze12,
       author = {{Naz{\'e}}, Ya{\"e}l and {Zhekov}, Svetozar A. and {Walborn}, Nolan R.},
        title = "{High-resolution X-Ray Spectroscopy of the Magnetic Of?p Star HD 148937}",
      journal = {\apj},
     keywords = {stars: early-type, stars: individual: HD148937, stars: massive, X-rays: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = feb,
       volume = {746},
       number = {2},
          eid = {142},
        pages = {142},
          doi = {10.1088/0004-637X/746/2/142},
archivePrefix = {arXiv},
       eprint = {1111.7186},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...746..142N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{conti,
       author = {{Conti}, Peter S. and {Alschuler}, William R.},
        title = "{Spectroscopic Studies of O-Type Stars. I. Classification and Absolute Magnitudes}",
      journal = {\apj},
         year = 1971,
        month = dec,
       volume = {170},
        pages = {325},
          doi = {10.1086/151218},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971ApJ...170..325C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mathys,
       author = {{Mathys}, G.},
        title = "{The upper main sequence of OB associations. I. Spectral types and lines of C and N of southern single-lined O stars.}",
      journal = {\aaps},
     keywords = {Abundance, Blue Stars, Carbon, Nitrogen, O Stars, Stellar Spectra, Astronomical Catalogs, Evolution, Spectral Line Width, Stellar Luminosity, Astrophysics},
         year = 1988,
        month = dec,
       volume = {76},
        pages = {427-444},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1988A&AS...76..427M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martins05,
       author = {{Martins}, Lucimara P. and {Gonz{\'a}lez Delgado}, Rosa M. and {Leitherer}, Claus and {Cervi{\~n}o}, Miguel and {Hauschildt}, Peter},
        title = "{A high-resolution stellar library for evolutionary population synthesis}",
      journal = {\mnras},
     keywords = {stars: atmospheres, stars: evolution, Astrophysics},
         year = 2005,
        month = mar,
       volume = {358},
       number = {1},
        pages = {49-65},
          doi = {10.1111/j.1365-2966.2005.08703.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0501225},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.358...49M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wade11,
       author = {{Wade}, G.~A. and {Howarth}, I.~D. and {Townsend}, R.~H.~D. and {Grunhut}, J.~H. and {Shultz}, M. and {Bouret}, J. -C. and {Fullerton}, A. and {Marcolino}, W. and {Martins}, F. and {Naz{\'e}}, Y. and {Ud Doula}, A. and {Walborn}, N.~R. and {Donati}, J. -F.},
        title = "{Confirmation of the magnetic oblique rotator model for the Of?p star HD 191612}",
      journal = {\mnras},
     keywords = {stars: individual: HD 191612, stars: magnetic field, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = oct,
       volume = {416},
       number = {4},
        pages = {3160-3169},
          doi = {10.1111/j.1365-2966.2011.19265.x},
archivePrefix = {arXiv},
       eprint = {1106.3008},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.416.3160W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petit13,
       author = {{Petit}, V. and {Owocki}, S.~P. and {Wade}, G.~A. and {Cohen}, D.~H. and {Sundqvist}, J.~O. and {Gagn{\'e}}, M. and {Ma{\'\i}z Apell{\'a}niz}, J. and {Oksala}, M.~E. and {Bohlender}, D.~A. and {Rivinius}, T. and {Henrichs}, H.~F. and {Alecian}, E. and {Townsend}, R.~H.~D. and {ud-Doula}, A. and {MiMeS Collaboration}},
        title = "{A magnetic confinement versus rotation classification of massive-star magnetospheres}",
      journal = {\mnras},
     keywords = {circumstellar matter, stars: early-type, stars: fundamental parameters, stars: magnetic fields, stars: mass-loss, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2013,
        month = feb,
       volume = {429},
       number = {1},
        pages = {398-422},
          doi = {10.1093/mnras/sts344},
archivePrefix = {arXiv},
       eprint = {1211.0282},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.429..398P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mp,
       author = {{Martins}, F. and {Plez}, B.},
        title = "{UBVJHK synthetic photometry of Galactic O stars}",
      journal = {\aap},
     keywords = {stars: fundamental parameters, stars: atmospheres, stars: early-type, Astrophysics},
         year = 2006,
        month = oct,
       volume = {457},
       number = {2},
        pages = {637-644},
          doi = {10.1051/0004-6361:20065753},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606587},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...457..637M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bonnsai,
       author = {{Schneider}, F.~R.~N. and {Langer}, N. and {de Koter}, A. and {Brott}, I. and {Izzard}, R.~G. and {Lau}, H.~H.~B.},
        title = "{Bonnsai: a Bayesian tool for comparing stars with stellar evolution models}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: statistical, stars: general, stars: fundamental parameters, stars: rotation, binaries: general, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2014,
        month = oct,
       volume = {570},
          eid = {A66},
        pages = {A66},
          doi = {10.1051/0004-6361/201424286},
archivePrefix = {arXiv},
       eprint = {1408.3409},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...570A..66S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sana11,
       author = {{Sana}, H. and {Le Bouquin}, J. -B. and {De Becker}, M. and {Berger}, J. -P. and {de Koter}, A. and {M{\'e}rand}, A.},
        title = "{The Non-thermal Radio Emitter HD 93250 Resolved by Long Baseline Interferometry}",
      journal = {\apjl},
     keywords = {radiation mechanisms: non-thermal, stars: early-type, stars: individual: HD93250, stars: massive, techniques: interferometric, X-rays: individual: HD93250, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = oct,
       volume = {740},
       number = {2},
          eid = {L43},
        pages = {L43},
          doi = {10.1088/2041-8205/740/2/L43},
archivePrefix = {arXiv},
       eprint = {1110.0831},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...740L..43S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sana17,
       author = {{Sana}, H. and {Ram{\'\i}rez-Tannus}, M.~C. and {de Koter}, A. and {Kaper}, L. and {Tramper}, F. and {Bik}, A.},
        title = "{A dearth of short-period massive binaries in the young massive star forming region M 17. Evidence for a large orbital separation at birth?}",
      journal = {\aap},
     keywords = {binaries: spectroscopic, stars: early-type, stars: formation, open clusters and associations: individual: M 17, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {L9},
        pages = {L9},
          doi = {10.1051/0004-6361/201630087},
archivePrefix = {arXiv},
       eprint = {1702.02153},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599L...9S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jb17,
       author = {{Le Bouquin}, J. -B. and {Sana}, H. and {Gosset}, E. and
         {De Becker}, M. and {Duvert}, G. and {Absil}, O. and {Anthonioz}, F. and
         {Berger}, J. -P. and {Ertel}, S. and {Grellmann}, R. and {Guieu}, S. and
         {Kervella}, P. and {Rabus}, M. and {Willson}, M.},
        title = "{Resolved astrometric orbits of ten O-type binaries}",
      journal = {\aap},
     keywords = {stars: massive, binaries: general, methods: observational, techniques: high angular resolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = may,
       volume = {601},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201629260},
archivePrefix = {arXiv},
       eprint = {1608.03525},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...601A..34L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jb17,
       author = {{Le Bouquin}, J. -B. and {Sana}, H. and {Gosset}, E. and {De Becker}, M. and {Duvert}, G. and {Absil}, O. and {Anthonioz}, F. and {Berger}, J. -P. and {Ertel}, S. and {Grellmann}, R. and {Guieu}, S. and {Kervella}, P. and {Rabus}, M. and {Willson}, M.},
        title = "{Resolved astrometric orbits of ten O-type binaries}",
      journal = {\aap},
     keywords = {stars: massive, binaries: general, methods: observational, techniques: high angular resolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = may,
       volume = {601},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201629260},
archivePrefix = {arXiv},
       eprint = {1608.03525},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...601A..34L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shenar2020,
       author = {{Shenar}, T. and {Bodensteiner}, J. and {Abdul-Masih}, M. and {Fabry}, M. and {Mahy}, L. and {Marchant}, P. and {Banyard}, G. and {Bowman}, D.~M. and {Dsilva}, K. and {Hawcroft}, C. and {Reggiani}, M. and {Sana}, H.},
        title = "{The ``hidden'' companion in LB-1 unveiled by spectral disentangling}",
      journal = {\aap},
     keywords = {stars: early-type, stars: emission-line, Be, binaries: spectroscopic, binaries: close, stars: individual: LS V+22 25, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jul,
       volume = {639},
          eid = {L6},
        pages = {L6},
          doi = {10.1051/0004-6361/202038275},
archivePrefix = {arXiv},
       eprint = {2004.12882},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...639L...6S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{julia2020,
       author = {{Bodensteiner}, J. and {Shenar}, T. and {Mahy}, L. and {Fabry}, M. and {Marchant}, P. and {Abdul-Masih}, M. and {Banyard}, G. and {Bowman}, D.~M. and {Dsilva}, K. and {Frost}, A.~J. and {Hawcroft}, C. and {Reggiani}, M. and {Sana}, H.},
        title = "{Is HR 6819 a triple system containing a black hole?. An alternative explanation}",
      journal = {\aap},
     keywords = {stars: massive, stars: early-type, stars: emission-line, Be, binaries: close, binaries: spectroscopic, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A43},
        pages = {A43},
          doi = {10.1051/0004-6361/202038682},
archivePrefix = {arXiv},
       eprint = {2006.10770},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A..43B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{gravpipe,
       author = {{Lapeyrere}, V. and {Kervella}, P. and {Lacour}, S. and {Azouaoui}, N. and
         {Garcia-Dabo}, C.~E. and {Perrin}, G. and {Eisenhauer}, F. and
         {Perraut}, K. and {Straubmeier}, C. and {Amorim}, A. and {Brandner}, W.},
        title = "{GRAVITY data reduction software}",
    booktitle = {\procspie},
         year = 2014,
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9146},
        month = jul,
          eid = {91462D},
        pages = {91462D},
          doi = {10.1117/12.2056850},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SPIE.9146E..2DL},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{naze10,
       author = {{Naz{\'e}}, Y. and {Ud-Doula}, A. and {Spano}, M. and {Rauw}, G. and
         {De Becker}, M. and {Walborn}, N.~R.},
        title = "{New findings on the prototypical Of?p stars}",
      journal = {\aap},
     keywords = {X-rays: stars, stars: individual: HD 108, stars: individual: HD 148937, stars: individual: HD 191612, stars: emission-line, Be, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2010,
        month = sep,
       volume = {520},
          eid = {A59},
        pages = {A59},
          doi = {10.1051/0004-6361/201014333},
archivePrefix = {arXiv},
       eprint = {1006.2054},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...520A..59N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{georgy17,
       author = {{Georgy}, Cyril and {Meynet}, Georges and {Ekstr{\"o}m}, Sylvia and
         {Wade}, Gregg A. and {Petit}, V{\'e}ronique and {Keszthelyi}, Zsolt and
         {Hirschi}, Raphael},
        title = "{Possible pair-instability supernovae at solar metallicity from magnetic stellar progenitors}",
      journal = {\aap},
     keywords = {stars: evolution, stars: magnetic field, stars: massive, stars: mass-loss, supernovae: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {L5},
        pages = {L5},
          doi = {10.1051/0004-6361/201730401},
archivePrefix = {arXiv},
       eprint = {1702.02340},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599L...5G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{edibles,
       author = {{Cox}, Nick L.~J. and {Cami}, Jan and {Farhang}, Amin and
         {Smoker}, Jonathan and {Monreal-Ibero}, Ana and {Lallement}, Rosine and
         {Sarre}, Peter J. and {Marshall}, Charlotte C.~M. and
         {Smith}, Keith T. and {Evans}, Christopher J. and {Royer}, Pierre and
         {Linnartz}, Harold and {Cordiner}, Martin A. and {Joblin}, Christine and
         {van Loon}, Jacco Th. and {Foing}, Bernard H. and {Bhatt}, Neil H. and
         {Bron}, Emeric and {Elyajouri}, Meriem and {de Koter}, Alex and
         {Ehrenfreund}, Pascale and {Javadi}, Atefeh and {Kaper}, Lex and
         {Khosroshadi}, Habib G. and {Laverick}, Mike and {Le Petit}, Franck and
         {Mulas}, Giacomo and {Roueff}, Evelyne and {Salama}, Farid and
         {Spaans}, Marco},
        title = "{The ESO Diffuse Interstellar Bands Large Exploration Survey (EDIBLES) . I. Project description, survey sample, and quality assessment}",
      journal = {\aap},
     keywords = {ISM: lines and bands, ISM: clouds, ISM: molecules, dust, extinction, stars: early-type, local insterstellar matter, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = oct,
       volume = {606},
          eid = {A76},
        pages = {A76},
          doi = {10.1051/0004-6361/201730912},
archivePrefix = {arXiv},
       eprint = {1708.01429},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...606A..76C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{langerrev,
       author = {{Langer}, N.},
        title = "{Presupernova Evolution of Massive Single and Binary Stars}",
      journal = {\araa},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = sep,
       volume = {50},
        pages = {107-164},
          doi = {10.1146/annurev-astro-081811-125534},
archivePrefix = {arXiv},
       eprint = {1206.5443},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ARA&A..50..107L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mahy17,
       author = {{Mahy}, L. and {Hutsem{\'e}kers}, D. and {Naz{\'e}}, Y. and {Royer}, P. and
         {Lebouteiller}, V. and {Waelkens}, C.},
        title = "{Evolutionary status of the Of?p star HD 148937 and of its surrounding nebula NGC 6164/5}",
      journal = {\aap},
     keywords = {infrared: stars, stars: individual: HD 148937, ISM: individual objects: NGC 6164/5, stars: abundances, circumstellar matter, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = mar,
       volume = {599},
          eid = {A61},
        pages = {A61},
          doi = {10.1051/0004-6361/201629585},
archivePrefix = {arXiv},
       eprint = {1611.07257},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...599A..61M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hubrig11,
       author = {{Hubrig}, S. and {Sch{\"o}ller}, M. and {Kharchenko}, N.~V. and
         {Langer}, N. and {de Wit}, W.~J. and {Ilyin}, I. and
         {Kholtygin}, A.~F. and {Piskunov}, A.~E. and {Przybilla}, N. and
         {Magori Collaboration}},
        title = "{Exploring the origin of magnetic fields in massive stars: a survey of O-type stars in clusters and in the field}",
      journal = {\aap},
     keywords = {polarization, stars: magnetic field, stars: kinematics and dynamics, open clusters and associations: general, stars: early-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = apr,
       volume = {528},
          eid = {A151},
        pages = {A151},
          doi = {10.1051/0004-6361/201016345},
archivePrefix = {arXiv},
       eprint = {1102.2503},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...528A.151H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wade12,
       author = {{Wade}, G.~A. and {Grunhut}, J. and {Gr{\"a}fener}, G. and
         {Howarth}, I.~D. and {Martins}, F. and {Petit}, V. and {Vink}, J.~S. and
         {Bagnulo}, S. and {Folsom}, C.~P. and {Naz{\'e}}, Y. and
         {Walborn}, N.~R. and {Townsend}, R.~H.~D. and {Evans}, C.~J.},
        title = "{The spectral variability and magnetic field characteristics of the Of?p star HD 148937}",
      journal = {\mnras},
     keywords = {binaries: spectroscopic, stars: early-type, stars: magnetic fields, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = jan,
       volume = {419},
       number = {3},
        pages = {2459-2471},
          doi = {10.1111/j.1365-2966.2011.19897.x},
archivePrefix = {arXiv},
       eprint = {1108.4847},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.419.2459W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petit17,
       author = {{Petit}, V. and {Keszthelyi}, Z. and {MacInnis}, R. and {Cohen}, D.~H. and
         {Townsend}, R.~H.~D. and {Wade}, G.~A. and {Thomas}, S.~L. and
         {Owocki}, S.~P. and {Puls}, J. and {ud-Doula}, A.},
        title = "{Magnetic massive stars as progenitors of `heavy' stellar-mass black holes}",
      journal = {\mnras},
     keywords = {stars: black holes, stars: early-type, stars: evolution, stars: magnetic field, stars: massive, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {466},
       number = {1},
        pages = {1052-1060},
          doi = {10.1093/mnras/stw3126},
archivePrefix = {arXiv},
       eprint = {1611.08964},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.1052P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{donati02,
       author = {{Donati}, J. -F. and {Babel}, J. and {Harries}, T.~J. and
         {Howarth}, I.~D. and {Petit}, P. and {Semel}, M.},
        title = "{The magnetic field and wind confinement of {\ensuremath{\theta}}$^{1}$ Orionis C}",
      journal = {\mnras},
     keywords = {stars: individual: {\ensuremath{\theta}}1 Ori C, stars: magnetic fields, stars: rotation, stars: winds, outflows},
         year = 2002,
        month = jun,
       volume = {333},
       number = {1},
        pages = {55-70},
          doi = {10.1046/j.1365-8711.2002.05379.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.333...55D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{leith,
   author = {{Leitherer}, C.},
    title = "{Massive Stars in Starburst Galaxies and the Origin of Galactic Superwinds.}",
booktitle = {Reviews in Modern Astronomy},
     year = 1994,
   series = {Reviews in Modern Astronomy},
   volume = 7,
   editor = {{Klare}, G.},
    pages = {73-102},
   adsurl = {http://adsabs.harvard.edu/abs/1994RvMA....7...73L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{oiutils1,
       author = {{Kervella}, P. and {Bigot}, L. and {Gallenne}, A. and {Th{\'e}venin}, F.},
        title = "{The radii and limb darkenings of {\ensuremath{\alpha}} Centauri A and B . Interferometric measurements with VLTI/PIONIER}",
      journal = {\aap},
     keywords = {stars: individual: Alpha Centauri, techniques: interferometric, stars: solar-type, stars: fundamental parameters, binaries: visual, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {597},
          eid = {A137},
        pages = {A137},
          doi = {10.1051/0004-6361/201629505},
archivePrefix = {arXiv},
       eprint = {1610.06185},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...597A.137K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{oiutils2,
       author = {{Liu}, Hauyu Baobab and {M{\'e}rand}, Antoine and {Green}, Joel D. and
         {P{\'e}rez}, Sebasti{\'a}n and {Hales}, Antonio S. and {Yang}, Yao-Lun and
         {Dunham}, Michael M. and {Hasegawa}, Yasuhiro and {Henning}, Thomas and
         {Galv{\'a}n-Madrid}, Roberto and {K{\'o}sp{\'a}l}, {\'A}gnes and
         {Takami}, Michihiro and {Vorobyov}, Eduard I. and {Zhu}, Zhaohuan},
        title = "{Diagnosing 0.1-10 au Scale Morphology of the FU Ori Disk Using ALMA and VLTI/GRAVITY}",
      journal = {\apj},
     keywords = {protoplanetary disks, stars: individual: FU Ori, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {884},
       number = {1},
          eid = {97},
        pages = {97},
          doi = {10.3847/1538-4357/ab391c},
archivePrefix = {arXiv},
       eprint = {1908.02981},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884...97L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{gravity,
       author = {{Eisenhauer}, F. and {Perrin}, G. and {Brandner}, W. and
         {Straubmeier}, C. and {Perraut}, K. and {Amorim}, A. and
         {Sch{\"o}ller}, M. and {Gillessen}, S. and {Kervella}, P. and
         {Benisty}, M. and {Araujo-Hauck}, C. and {Jocou}, L. and {Lima}, J. and
         {Jakob}, G. and {Haug}, M. and {Cl{\'e}net}, Y. and {Henning}, T. and
         {Eckart}, A. and {Berger}, J. -P. and {Garcia}, P. and {Abuter}, R. and
         {Kellner}, S. and {Paumard}, T. and {Hippler}, S. and {Fischer}, S. and
         {Moulin}, T. and {Villate}, J. and {Avila}, G. and {Gr{\"a}ter}, A. and
         {Lacour}, S. and {Huber}, A. and {Wiest}, M. and {Nolot}, A. and
         {Carvas}, P. and {Dorn}, R. and {Pfuhl}, O. and {Gendron}, E. and
         {Kendrew}, S. and {Yazici}, S. and {Anton}, S. and {Jung}, Y. and
         {Thiel}, M. and {Choquet}, {\'E}. and {Klein}, R. and {Teixeira}, P. and
         {Gitton}, P. and {Moch}, D. and {Vincent}, F. and {Kudryavtseva}, N. and
         {Str{\"o}bele}, S. and {Sturm}, S. and {F{\'e}dou}, P. and
         {Lenzen}, R. and {Jolley}, P. and {Kister}, C. and {Lapeyr{\`e}re}, V. and
         {Naranjo}, V. and {Lucuix}, C. and {Hofmann}, R. and {Chapron}, F. and
         {Neumann}, U. and {Mehrgan}, L. and {Hans}, O. and {Rousset}, G. and
         {Ramos}, J. and {Suarez}, M. and {Lederer}, R. and {Reess}, J. -M. and
         {Rohloff}, R. -R. and {Haguenauer}, P. and {Bartko}, H. and
         {Sevin}, A. and {Wagner}, K. and {Lizon}, J. -L. and {Rabien}, S. and
         {Collin}, C. and {Finger}, G. and {Davies}, R. and {Rouan}, D. and
         {Wittkowski}, M. and {Dodds-Eden}, K. and {Ziegler}, D. and
         {Cassaing}, F. and {Bonnet}, H. and {Casali}, M. and {Genzel}, R. and
         {Lena}, P.},
        title = "{GRAVITY: Observing the Universe in Motion}",
      journal = {The Messenger},
         year = 2011,
        month = mar,
       volume = {143},
        pages = {16-24},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011Msngr.143...16E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hillier98,
       author = {{Hillier}, D. John and {Miller}, D.~L.},
        title = "{The Treatment of Non-LTE Line Blanketing in Spherically Expanding Outflows}",
      journal = {\apj},
     keywords = {RADIATIVE TRANSFER, STARS: EMISSION-LINE, BE, LINE: FORMATION, STARS: MASS LOSS, STARS: WOLF-RAYET, Line: Formation, Radiative Transfer, Stars: Emission-Line, Be, Stars: Mass Loss, Stars: Wolf-Rayet},
         year = 1998,
        month = mar,
       volume = {496},
       number = {1},
        pages = {407-427},
          doi = {10.1086/305350},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998ApJ...496..407H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vink01,
       author = {{Vink}, Jorick S. and {de Koter}, A. and {Lamers}, H.~J.~G.~L.~M.},
        title = "{Mass-loss predictions for O and B stars as a function of metallicity}",
      journal = {\aap},
     keywords = {STARS: EARLY-TYPE, STARS: MASS-LOSS, STARS: SUPERGIANTS, STARS: WINDS, STARS: EVOLUTION, Astrophysics},
         year = 2001,
        month = apr,
       volume = {369},
        pages = {574-588},
          doi = {10.1051/0004-6361:20010127},
archivePrefix = {arXiv},
       eprint = {astro-ph/0101509},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...369..574V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sd14,
       author = {{Sim{\'o}n-D{\'\i}az}, S. and {Herrero}, A.},
        title = "{The IACOB project. I. Rotational velocities in northern Galactic O- and early B-type stars revisited. The impact of other sources of line-broadening}",
      journal = {\aap},
     keywords = {stars: early-type, stars: rotation, techniques: spectroscopic, line: profiles, astronomical databases: miscellaneous, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = feb,
       volume = {562},
          eid = {A135},
        pages = {A135},
          doi = {10.1051/0004-6361/201322758},
archivePrefix = {arXiv},
       eprint = {1311.3360},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...562A.135S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{grevesse10,
       author = {{Grevesse}, N. and {Asplund}, M. and {Sauval}, A.~J. and {Scott}, P.},
        title = "{The chemical composition of the Sun}",
      journal = {\apss},
     keywords = {Solar abundances},
         year = 2010,
        month = jul,
       volume = {328},
       number = {1-2},
        pages = {179-183},
          doi = {10.1007/s10509-010-0288-z},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010Ap&SS.328..179G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hillier03,
       author = {{Hillier}, D. John and {Lanz}, T. and {Heap}, S.~R. and {Hubeny}, I. and {Smith}, L.~J. and {Evans}, C.~J. and {Lennon}, D.~J. and {Bouret}, J.~C.},
        title = "{A Tale of Two Stars: The Extreme O7 Iaf+ Supergiant AV 83 and the OC7.5 III((f)) star AV 69}",
      journal = {\apj},
     keywords = {Galaxies: Magellanic Clouds, Stars: Abundances, Stars: Atmospheres, Stars: Individual: Alphanumeric: AV 69, Stars: Individual: Alphanumeric: AV 83, Ultraviolet: Stars},
         year = 2003,
        month = may,
       volume = {588},
       number = {2},
        pages = {1039-1063},
          doi = {10.1086/374329},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...588.1039H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{brott,
       author = {{Brott}, I. and {de Mink}, S.~E. and {Cantiello}, M. and {Langer}, N. and {de Koter}, A. and {Evans}, C.~J. and {Hunter}, I. and {Trundle}, C. and {Vink}, J.~S.},
        title = "{Rotating massive main-sequence stars. I. Grids of evolutionary models and isochrones}",
      journal = {\aap},
     keywords = {stars: abundances, stars: evolution, stars: early-type, stars: rotation, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = jun,
       volume = {530},
          eid = {A115},
        pages = {A115},
          doi = {10.1051/0004-6361/201016113},
archivePrefix = {arXiv},
       eprint = {1102.0530},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...530A.115B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moss,
       author = {{Moss}, D.},
        title = "{The survival of fossil magnetic fields during pre-main sequence evolution}",
      journal = {\aap},
     keywords = {magnetic fields, magnetohydrodynamics (MHD), stars: evolution, stars: chemically peculiar},
         year = 2003,
        month = may,
       volume = {403},
        pages = {693-697},
          doi = {10.1051/0004-6361:20030431},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...403..693M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{edibles,
       author = {{Cox}, Nick L.~J. and {Cami}, Jan and {Farhang}, Amin and {Smoker}, Jonathan and {Monreal-Ibero}, Ana and {Lallement}, Rosine and {Sarre}, Peter J. and {Marshall}, Charlotte C.~M. and {Smith}, Keith T. and {Evans}, Christopher J. and {Royer}, Pierre and {Linnartz}, Harold and {Cordiner}, Martin A. and {Joblin}, Christine and {van Loon}, Jacco Th. and {Foing}, Bernard H. and {Bhatt}, Neil H. and {Bron}, Emeric and {Elyajouri}, Meriem and {de Koter}, Alex and {Ehrenfreund}, Pascale and {Javadi}, Atefeh and {Kaper}, Lex and {Khosroshadi}, Habib G. and {Laverick}, Mike and {Le Petit}, Franck and {Mulas}, Giacomo and {Roueff}, Evelyne and {Salama}, Farid and {Spaans}, Marco},
        title = "{The ESO Diffuse Interstellar Bands Large Exploration Survey (EDIBLES) . I. Project description, survey sample, and quality assessment}",
      journal = {\aap},
     keywords = {ISM: lines and bands, ISM: clouds, ISM: molecules, dust, extinction, stars: early-type, local insterstellar matter, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = oct,
       volume = {606},
          eid = {A76},
        pages = {A76},
          doi = {10.1051/0004-6361/201730912},
archivePrefix = {arXiv},
       eprint = {1708.01429},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...606A..76C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{magfrac1,
       author = {{Fossati}, L. and {Castro}, N. and {Sch{\"o}ller}, M. and {Hubrig}, S. and {Langer}, N. and {Morel}, T. and {Briquet}, M. and {Herrero}, A. and {Przybilla}, N. and {Sana}, H. and {Schneider}, F.~R.~N. and {de Koter}, A. and {BOB Collaboration}},
        title = "{B fields in OB stars (BOB): Low-resolution FORS2 spectropolarimetry of the first sample of 50 massive stars}",
      journal = {\aap},
     keywords = {stars: magnetic field, stars: early-type, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = oct,
       volume = {582},
          eid = {A45},
        pages = {A45},
          doi = {10.1051/0004-6361/201526725},
archivePrefix = {arXiv},
       eprint = {1508.00750},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...582A..45F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{magfrac2,
       author = {{Grunhut}, J.~H. and {Wade}, G.~A. and {Neiner}, C. and {Oksala}, M.~E. and {Petit}, V. and {Alecian}, E. and {Bohlender}, D.~A. and {Bouret}, J. -C. and {Henrichs}, H.~F. and {Hussain}, G.~A.~J. and {Kochukhov}, O. and {MiMeS Collaboration}},
        title = "{The MiMeS survey of Magnetism in Massive Stars: magnetic analysis of the O-type stars}",
      journal = {\mnras},
     keywords = {instrumentation: polarimeters, surveys, stars: early-type, stars: magnetic field, stars: massive, stars: rotation, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = feb,
       volume = {465},
       number = {2},
        pages = {2432-2470},
          doi = {10.1093/mnras/stw2743},
archivePrefix = {arXiv},
       eprint = {1610.07895},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465.2432G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gw,
       author = {{Abbott}, B.~P. and {Abbott}, R. and {Abbott}, T.~D. and {Abernathy}, M.~R. and {Acernese}, F. and {Ackley}, K. and {Adams}, C. and {Adams}, T. and {Addesso}, P. and {Adhikari}, R.~X. and {Adya}, V.~B. and {Affeldt}, C. and {Agathos}, M. and {Agatsuma}, K. and {Aggarwal}, N. and {Aguiar}, O.~D. and {Aiello}, L. and {Ain}, A. and {Ajith}, P. and {Allen}, B. and {Allocca}, A. and {Altin}, P.~A. and {Anderson}, S.~B. and {Anderson}, W.~G. and {Arai}, K. and {Arain}, M.~A. and {Araya}, M.~C. and {Arceneaux}, C.~C. and {Areeda}, J.~S. and {Arnaud}, N. and {Arun}, K.~G. and {Ascenzi}, S. and {Ashton}, G. and {Ast}, M. and {Aston}, S.~M. and {Astone}, P. and {Aufmuth}, P. and {Aulbert}, C. and {Babak}, S. and {Bacon}, P. and {Bader}, M.~K.~M. and {Baker}, P.~T. and {Baldaccini}, F. and {Ballardin}, G. and {Ballmer}, S.~W. and {Barayoga}, J.~C. and {Barclay}, S.~E. and {Barish}, B.~C. and {Barker}, D. and {Barone}, F. and {Barr}, B. and {Barsotti}, L. and {Barsuglia}, M. and {Barta}, D. and {Bartlett}, J. and {Barton}, M.~A. and {Bartos}, I. and {Bassiri}, R. and {Basti}, A. and {Batch}, J.~C. and {Baune}, C. and {Bavigadda}, V. and {Bazzan}, M. and {Behnke}, B. and {Bejger}, M. and {Belczynski}, C. and {Bell}, A.~S. and {Bell}, C.~J. and {Berger}, B.~K. and {Bergman}, J. and {Bergmann}, G. and {Berry}, C.~P.~L. and {Bersanetti}, D. and {Bertolini}, A. and {Betzwieser}, J. and {Bhagwat}, S. and {Bhandare}, R. and {Bilenko}, I.~A. and {Billingsley}, G. and {Birch}, J. and {Birney}, R. and {Birnholtz}, O. and {Biscans}, S. and {Bisht}, A. and {Bitossi}, M. and {Biwer}, C. and {Bizouard}, M.~A. and {Blackburn}, J.~K. and {Blair}, C.~D. and {Blair}, D.~G. and {Blair}, R.~M. and {Bloemen}, S. and {Bock}, O. and {Bodiya}, T.~P. and {Boer}, M. and {Bogaert}, G. and {Bogan}, C. and {Bohe}, A. and {Bojtos}, P. and {Bond}, C. and {Bondu}, F. and {Bonnand}, R. and {Boom}, B.~A. and {Bork}, R. and {Boschi}, V. and {Bose}, S. and {Bouffanais}, Y. and {Bozzi}, A. and {Bradaschia}, C. and {Brady}, P.~R. and {Braginsky}, V.~B. and {Branchesi}, M. and {Brau}, J.~E. and {Briant}, T. and {Brillet}, A. and {Brinkmann}, M. and {Brisson}, V. and {Brockill}, P. and {Brooks}, A.~F. and {Brown}, D.~A. and {Brown}, D.~D. and {Brown}, N.~M. and {Buchanan}, C.~C. and {Buikema}, A. and {Bulik}, T. and {Bulten}, H.~J. and {Buonanno}, A. and {Buskulic}, D. and {Buy}, C. and {Byer}, R.~L. and {Cabero}, M. and {Cadonati}, L. and {Cagnoli}, G. and {Cahillane}, C. and {Bustillo}, J. Calder{\'o}n and {Callister}, T. and {Calloni}, E. and {Camp}, J.~B. and {Cannon}, K.~C. and {Cao}, J. and {Capano}, C.~D. and {Capocasa}, E. and {Carbognani}, F. and {Caride}, S. and {Casanueva Diaz}, J. and {Casentini}, C. and {Caudill}, S. and {Cavagli{\`a}}, M. and {Cavalier}, F. and {Cavalieri}, R. and {Cella}, G. and {Cepeda}, C.~B. and {Baiardi}, L. Cerboni and {Cerretani}, G. and {Cesarini}, E. and {Chakraborty}, R. and {Chalermsongsak}, T. and {Chamberlin}, S.~J. and {Chan}, M. and {Chao}, S. and {Charlton}, P. and {Chassande-Mottin}, E. and {Chen}, H.~Y. and {Chen}, Y. and {Cheng}, C. and {Chincarini}, A. and {Chiummo}, A. and {Cho}, H.~S. and {Cho}, M. and {Chow}, J.~H. and {Christensen}, N. and {Chu}, Q. and {Chua}, S. and {Chung}, S. and {Ciani}, G. and {Clara}, F. and {Clark}, J.~A. and {Cleva}, F. and {Coccia}, E. and {Cohadon}, P. -F. and {Colla}, A. and {Collette}, C.~G. and {Cominsky}, L. and {Constancio}, M. and {Conte}, A. and {Conti}, L. and {Cook}, D. and {Corbitt}, T.~R. and {Cornish}, N. and {Corsi}, A. and {Cortese}, S. and {Costa}, C.~A. and {Coughlin}, M.~W. and {Coughlin}, S.~B. and {Coulon}, J. -P. and {Countryman}, S.~T. and {Couvares}, P. and {Cowan}, E.~E. and {Coward}, D.~M. and {Cowart}, M.~J. and {Coyne}, D.~C. and {Coyne}, R. and {Craig}, K. and {Creighton}, J.~D.~E. and {Creighton}, T.~D. and {Cripe}, J. and {Crowder}, S.~G. and {Cruise}, A.~M. and {Cumming}, A. and {Cunningham}, L. and {Cuoco}, E. and {Dal Canton}, T. and {Danilishin}, S.~L. and {D'Antonio}, S. and {Danzmann}, K. and {Darman}, N.~S. and {Da Silva Costa}, C.~F. and {Dattilo}, V. and {Dave}, I. and {Daveloza}, H.~P. and {Davier}, M. and {Davies}, G.~S. and {Daw}, E.~J. and {Day}, R. and {De}, S. and {DeBra}, D. and {Debreczeni}, G. and {Degallaix}, J. and {De Laurentis}, M. and {Del{\'e}glise}, S. and {Del Pozzo}, W. and {Denker}, T. and {Dent}, T. and {Dereli}, H. and {Dergachev}, V. and {DeRosa}, R.~T. and {De Rosa}, R. and {DeSalvo}, R. and {Dhurandhar}, S. and {D{\'\i}az}, M.~C. and {Di Fiore}, L. and {Di Giovanni}, M. and {Di Lieto}, A. and {Di Pace}, S. and {Di Palma}, I. and {Di Virgilio}, A. and {Dojcinoski}, G. and {Dolique}, V. and {Donovan}, F. and {Dooley}, K.~L. and {Doravari}, S. and {Douglas}, R. and {Downes}, T.~P. and {Drago}, M. and {Drever}, R.~W.~P. and {Driggers}, J.~C. and {Du}, Z. and {Ducrot}, M. and {Dwyer}, S.~E. and {Edo}, T.~B. and {Edwards}, M.~C. and {Effler}, A. and {Eggenstein}, H. -B. and {Ehrens}, P. and {Eichholz}, J. and {Eikenberry}, S.~S. and {Engels}, W. and {Essick}, R.~C. and {Etzel}, T. and {Evans}, M. and {Evans}, T.~M. and {Everett}, R. and {Factourovich}, M. and {Fafone}, V. and {Fair}, H. and {Fairhurst}, S. and {Fan}, X. and {Fang}, Q. and {Farinon}, S. and {Farr}, B. and {Farr}, W.~M. and {Favata}, M. and {Fays}, M. and {Fehrmann}, H. and {Fejer}, M.~M. and {Feldbaum}, D. and {Ferrante}, I. and {Ferreira}, E.~C. and {Ferrini}, F. and {Fidecaro}, F. and {Finn}, L.~S. and {Fiori}, I. and {Fiorucci}, D. and {Fisher}, R.~P. and {Flaminio}, R. and {Fletcher}, M. and {Fong}, H. and {Fournier}, J. -D. and {Franco}, S. and {Frasca}, S. and {Frasconi}, F. and {Frede}, M. and {Frei}, Z. and {Freise}, A. and {Frey}, R. and {Frey}, V. and {Fricke}, T.~T. and {Fritschel}, P. and {Frolov}, V.~V. and {Fulda}, P. and {Fyffe}, M. and {Gabbard}, H.~A.~G. and {Gair}, J.~R. and {Gammaitoni}, L. and {Gaonkar}, S.~G. and {Garufi}, F. and {Gatto}, A. and {Gaur}, G. and {Gehrels}, N. and {Gemme}, G. and {Gendre}, B. and {Genin}, E. and {Gennai}, A. and {George}, J. and {Gergely}, L. and {Germain}, V. and {Ghosh}, Abhirup and {Ghosh}, Archisman and {Ghosh}, S. and {Giaime}, J.~A. and {Giardina}, K.~D. and {Giazotto}, A. and {Gill}, K. and {Glaefke}, A. and {Gleason}, J.~R. and {Goetz}, E. and {Goetz}, R. and {Gondan}, L. and {Gonz{\'a}lez}, G. and {Castro}, J.~M. Gonzalez and {Gopakumar}, A. and {Gordon}, N.~A. and {Gorodetsky}, M.~L. and {Gossan}, S.~E. and {Gosselin}, M. and {Gouaty}, R. and {Graef}, C. and {Graff}, P.~B. and {Granata}, M. and {Grant}, A. and {Gras}, S. and {Gray}, C. and {Greco}, G. and {Green}, A.~C. and {Greenhalgh}, R.~J.~S. and {Groot}, P. and {Grote}, H. and {Grunewald}, S. and {Guidi}, G.~M. and {Guo}, X. and {Gupta}, A. and {Gupta}, M.~K. and {Gushwa}, K.~E. and {Gustafson}, E.~K. and {Gustafson}, R. and {Hacker}, J.~J. and {Hall}, B.~R. and {Hall}, E.~D. and {Hammond}, G. and {Haney}, M. and {Hanke}, M.~M. and {Hanks}, J. and {Hanna}, C. and {Hannam}, M.~D. and {Hanson}, J. and {Hardwick}, T. and {Harms}, J. and {Harry}, G.~M. and {Harry}, I.~W. and {Hart}, M.~J. and {Hartman}, M.~T. and {Haster}, C. -J. and {Haughian}, K. and {Healy}, J. and {Heefner}, J. and {Heidmann}, A. and {Heintze}, M.~C. and {Heinzel}, G. and {Heitmann}, H. and {Hello}, P. and {Hemming}, G. and {Hendry}, M. and {Heng}, I.~S. and {Hennig}, J. and {Heptonstall}, A.~W. and {Heurs}, M. and {Hild}, S. and {Hoak}, D. and {Hodge}, K.~A. and {Hofman}, D. and {Hollitt}, S.~E. and {Holt}, K. and {Holz}, D.~E. and {Hopkins}, P. and {Hosken}, D.~J. and {Hough}, J. and {Houston}, E.~A. and {Howell}, E.~J. and {Hu}, Y.~M. and {Huang}, S. and {Huerta}, E.~A. and {Huet}, D. and {Hughey}, B. and {Husa}, S. and {Huttner}, S.~H. and {Huynh-Dinh}, T. and {Idrisy}, A. and {Indik}, N. and {Ingram}, D.~R. and {Inta}, R. and {Isa}, H.~N. and {Isac}, J. -M. and {Isi}, M. and {Islas}, G. and {Isogai}, T. and {Iyer}, B.~R. and {Izumi}, K. and {Jacobson}, M.~B. and {Jacqmin}, T. and {Jang}, H. and {Jani}, K. and {Jaranowski}, P. and {Jawahar}, S. and {Jim{\'e}nez-Forteza}, F. and {Johnson}, W.~W. and {Johnson-McDaniel}, N.~K. and {Jones}, D.~I. and {Jones}, R. and {Jonker}, R.~J.~G. and {Ju}, L. and {Haris}, K. and {Kalaghatgi}, C.~V. and {Kalogera}, V. and {Kandhasamy}, S. and {Kang}, G. and {Kanner}, J.~B. and {Karki}, S. and {Kasprzack}, M. and {Katsavounidis}, E. and {Katzman}, W. and {Kaufer}, S. and {Kaur}, T. and {Kawabe}, K. and {Kawazoe}, F. and {K{\'e}f{\'e}lian}, F. and {Kehl}, M.~S. and {Keitel}, D. and {Kelley}, D.~B. and {Kells}, W. and {Kennedy}, R. and {Keppel}, D.~G. and {Key}, J.~S. and {Khalaidovski}, A. and {Khalili}, F.~Y. and {Khan}, I. and {Khan}, S. and {Khan}, Z. and {Khazanov}, E.~A. and {Kijbunchoo}, N. and {Kim}, C. and {Kim}, J. and {Kim}, K. and {Kim}, Nam-Gyu and {Kim}, Namjun and {Kim}, Y. -M. and {King}, E.~J. and {King}, P.~J. and {Kinzel}, D.~L. and {Kissel}, J.~S. and {Kleybolte}, L. and {Klimenko}, S. and {Koehlenbeck}, S.~M. and {Kokeyama}, K. and {Koley}, S. and {Kondrashov}, V. and {Kontos}, A. and {Koranda}, S. and {Korobko}, M. and {Korth}, W.~Z. and {Kowalska}, I. and {Kozak}, D.~B. and {Kringel}, V. and {Krishnan}, B. and {Kr{\'o}lak}, A. and {Krueger}, C. and {Kuehn}, G. and {Kumar}, P. and {Kumar}, R. and {Kuo}, L. and {Kutynia}, A. and {Kwee}, P. and {Lackey}, B.~D. and {Landry}, M. and {Lange}, J. and {Lantz}, B. and {Lasky}, P.~D. and {Lazzarini}, A. and {Lazzaro}, C. and {Leaci}, P. and {Leavey}, S. and {Lebigot}, E.~O. and {Lee}, C.~H. and {Lee}, H.~K. and {Lee}, H.~M. and {Lee}, K. and {Lenon}, A. and {Leonardi}, M. and {Leong}, J.~R. and {Leroy}, N. and {Letendre}, N. and {Levin}, Y. and {Levine}, B.~M. and {Li}, T.~G.~F. and {Libson}, A. and {Littenberg}, T.~B. and {Lockerbie}, N.~A. and {Logue}, J. and {Lombardi}, A.~L. and {London}, L.~T. and {Lord}, J.~E. and {Lorenzini}, M. and {Loriette}, V. and {Lormand}, M. and {Losurdo}, G. and {Lough}, J.~D. and {Lousto}, C.~O. and {Lovelace}, G. and {L{\"u}ck}, H. and {Lundgren}, A.~P. and {Luo}, J. and {Lynch}, R. and {Ma}, Y. and {MacDonald}, T. and {Machenschalk}, B. and {MacInnis}, M. and {Macleod}, D.~M. and {Maga{\~n}a-Sandoval}, F. and {Magee}, R.~M. and {Mageswaran}, M. and {Majorana}, E. and {Maksimovic}, I. and {Malvezzi}, V. and {Man}, N. and {Mandel}, I. and {Mandic}, V. and {Mangano}, V. and {Mansell}, G.~L. and {Manske}, M. and {Mantovani}, M. and {Marchesoni}, F. and {Marion}, F. and {M{\'a}rka}, S. and {M{\'a}rka}, Z. and {Markosyan}, A.~S. and {Maros}, E. and {Martelli}, F. and {Martellini}, L. and {Martin}, I.~W. and {Martin}, R.~M. and {Martynov}, D.~V. and {Marx}, J.~N. and {Mason}, K. and {Masserot}, A. and {Massinger}, T.~J. and {Masso-Reid}, M. and {Matichard}, F. and {Matone}, L. and {Mavalvala}, N. and {Mazumder}, N. and {Mazzolo}, G. and {McCarthy}, R. and {McClelland}, D.~E. and {McCormick}, S. and {McGuire}, S.~C. and {McIntyre}, G. and {McIver}, J. and {McManus}, D.~J. and {McWilliams}, S.~T. and {Meacher}, D. and {Meadors}, G.~D. and {Meidam}, J. and {Melatos}, A. and {Mendell}, G. and {Mendoza-Gandara}, D. and {Mercer}, R.~A. and {Merilh}, E. and {Merzougui}, M. and {Meshkov}, S. and {Messenger}, C. and {Messick}, C. and {Meyers}, P.~M. and {Mezzani}, F. and {Miao}, H. and {Michel}, C. and {Middleton}, H. and {Mikhailov}, E.~E. and {Milano}, L. and {Miller}, J. and {Millhouse}, M. and {Minenkov}, Y. and {Ming}, J. and {Mirshekari}, S. and {Mishra}, C. and {Mitra}, S. and {Mitrofanov}, V.~P. and {Mitselmakher}, G. and {Mittleman}, R. and {Moggi}, A. and {Mohan}, M. and {Mohapatra}, S.~R.~P. and {Montani}, M. and {Moore}, B.~C. and {Moore}, C.~J. and {Moraru}, D. and {Moreno}, G. and {Morriss}, S.~R. and {Mossavi}, K. and {Mours}, B. and {Mow-Lowry}, C.~M. and {Mueller}, C.~L. and {Mueller}, G. and {Muir}, A.~W. and {Mukherjee}, Arunava and {Mukherjee}, D. and {Mukherjee}, S. and {Mukund}, N. and {Mullavey}, A. and {Munch}, J. and {Murphy}, D.~J. and {Murray}, P.~G. and {Mytidis}, A. and {Nardecchia}, I. and {Naticchioni}, L. and {Nayak}, R.~K. and {Necula}, V. and {Nedkova}, K. and {Nelemans}, G. and {Neri}, M. and {Neunzert}, A. and {Newton}, G. and {Nguyen}, T.~T. and {Nielsen}, A.~B. and {Nissanke}, S. and {Nitz}, A. and {Nocera}, F. and {Nolting}, D. and {Normandin}, M.~E.~N. and {Nuttall}, L.~K. and {Oberling}, J. and {Ochsner}, E. and {O'Dell}, J. and {Oelker}, E. and {Ogin}, G.~H. and {Oh}, J.~J. and {Oh}, S.~H. and {Ohme}, F. and {Oliver}, M. and {Oppermann}, P. and {Oram}, Richard J. and {O'Reilly}, B. and {O'Shaughnessy}, R. and {Ott}, C.~D. and {Ottaway}, D.~J. and {Ottens}, R.~S. and {Overmier}, H. and {Owen}, B.~J. and {Pai}, A. and {Pai}, S.~A. and {Palamos}, J.~R. and {Palashov}, O. and {Palomba}, C. and {Pal-Singh}, A. and {Pan}, H. and {Pan}, Y. and {Pankow}, C. and {Pannarale}, F. and {Pant}, B.~C. and {Paoletti}, F. and {Paoli}, A. and {Papa}, M.~A. and {Paris}, H.~R. and {Parker}, W. and {Pascucci}, D. and {Pasqualetti}, A. and {Passaquieti}, R. and {Passuello}, D. and {Patricelli}, B. and {Patrick}, Z. and {Pearlstone}, B.~L. and {Pedraza}, M. and {Pedurand}, R. and {Pekowsky}, L. and {Pele}, A. and {Penn}, S. and {Perreca}, A. and {Pfeiffer}, H.~P. and {Phelps}, M. and {Piccinni}, O. and {Pichot}, M. and {Pickenpack}, M. and {Piergiovanni}, F. and {Pierro}, V. and {Pillant}, G. and {Pinard}, L. and {Pinto}, I.~M. and {Pitkin}, M. and {Poeld}, J.~H. and {Poggiani}, R. and {Popolizio}, P. and {Post}, A. and {Powell}, J. and {Prasad}, J. and {Predoi}, V. and {Premachandra}, S.~S. and {Prestegard}, T. and {Price}, L.~R. and {Prijatelj}, M. and {Principe}, M. and {Privitera}, S. and {Prix}, R. and {Prodi}, G.~A. and {Prokhorov}, L. and {Puncken}, O. and {Punturo}, M. and {Puppo}, P. and {P{\"u}rrer}, M. and {Qi}, H. and {Qin}, J. and {Quetschke}, V. and {Quintero}, E.~A. and {Quitzow-James}, R. and {Raab}, F.~J. and {Rabeling}, D.~S. and {Radkins}, H. and {Raffai}, P. and {Raja}, S. and {Rakhmanov}, M. and {Ramet}, C.~R. and {Rapagnani}, P. and {Raymond}, V. and {Razzano}, M. and {Re}, V. and {Read}, J. and {Reed}, C.~M. and {Regimbau}, T. and {Rei}, L. and {Reid}, S. and {Reitze}, D.~H. and {Rew}, H. and {Reyes}, S.~D. and {Ricci}, F. and {Riles}, K. and {Robertson}, N.~A. and {Robie}, R. and {Robinet}, F. and {Rocchi}, A. and {Rolland}, L. and {Rollins}, J.~G. and {Roma}, V.~J. and {Romano}, J.~D. and {Romano}, R. and {Romanov}, G. and {Romie}, J.~H. and {Rosi{\'n}ska}, D. and {Rowan}, S. and {R{\"u}diger}, A. and {Ruggi}, P. and {Ryan}, K. and {Sachdev}, S. and {Sadecki}, T. and {Sadeghian}, L. and {Salconi}, L. and {Saleem}, M. and {Salemi}, F. and {Samajdar}, A. and {Sammut}, L. and {Sampson}, L.~M. and {Sanchez}, E.~J. and {Sandberg}, V. and {Sandeen}, B. and {Sanders}, G.~H. and {Sanders}, J.~R. and {Sassolas}, B. and {Sathyaprakash}, B.~S. and {Saulson}, P.~R. and {Sauter}, O. and {Savage}, R.~L. and {Sawadsky}, A. and {Schale}, P. and {Schilling}, R. and {Schmidt}, J. and {Schmidt}, P. and {Schnabel}, R. and {Schofield}, R.~M.~S. and {Sch{\"o}nbeck}, A. and {Schreiber}, E. and {Schuette}, D. and {Schutz}, B.~F. and {Scott}, J. and {Scott}, S.~M. and {Sellers}, D. and {Sengupta}, A.~S. and {Sentenac}, D. and {Sequino}, V. and {Sergeev}, A. and {Serna}, G. and {Setyawati}, Y. and {Sevigny}, A. and {Shaddock}, D.~A. and {Shaffer}, T. and {Shah}, S. and {Shahriar}, M.~S. and {Shaltev}, M. and {Shao}, Z. and {Shapiro}, B. and {Shawhan}, P. and {Sheperd}, A. and {Shoemaker}, D.~H. and {Shoemaker}, D.~M. and {Siellez}, K. and {Siemens}, X. and {Sigg}, D. and {Silva}, A.~D. and {Simakov}, D. and {Singer}, A. and {Singer}, L.~P. and {Singh}, A. and {Singh}, R. and {Singhal}, A. and {Sintes}, A.~M. and {Slagmolen}, B.~J.~J. and {Smith}, J.~R. and {Smith}, M.~R. and {Smith}, N.~D. and {Smith}, R.~J.~E. and {Son}, E.~J. and {Sorazu}, B. and {Sorrentino}, F. and {Souradeep}, T. and {Srivastava}, A.~K. and {Staley}, A. and {Steinke}, M. and {Steinlechner}, J. and {Steinlechner}, S. and {Steinmeyer}, D. and {Stephens}, B.~C. and {Stevenson}, S.~P. and {Stone}, R. and {Strain}, K.~A. and {Straniero}, N. and {Stratta}, G. and {Strauss}, N.~A. and {Strigin}, S. and {Sturani}, R. and {Stuver}, A.~L. and {Summerscales}, T.~Z. and {Sun}, L. and {Sutton}, P.~J. and {Swinkels}, B.~L. and {Szczepa{\'n}czyk}, M.~J. and {Tacca}, M. and {Talukder}, D. and {Tanner}, D.~B. and {T{\'a}pai}, M. and {Tarabrin}, S.~P. and {Taracchini}, A. and {Taylor}, R. and {Theeg}, T. and {Thirugnanasambandam}, M.~P. and {Thomas}, E.~G. and {Thomas}, M. and {Thomas}, P. and {Thorne}, K.~A. and {Thorne}, K.~S. and {Thrane}, E. and {Tiwari}, S. and {Tiwari}, V. and {Tokmakov}, K.~V. and {Tomlinson}, C. and {Tonelli}, M. and {Torres}, C.~V. and {Torrie}, C.~I. and {T{\"o}yr{\"a}}, D. and {Travasso}, F. and {Traylor}, G. and {Trifir{\`o}}, D. and {Tringali}, M.~C. and {Trozzo}, L. and {Tse}, M. and {Turconi}, M. and {Tuyenbayev}, D. and {Ugolini}, D. and {Unnikrishnan}, C.~S. and {Urban}, A.~L. and {Usman}, S.~A. and {Vahlbruch}, H. and {Vajente}, G. and {Valdes}, G. and {Vallisneri}, M. and {van Bakel}, N. and {van Beuzekom}, M. and {van den Brand}, J.~F.~J. and {Van Den Broeck}, C. and {Vander-Hyde}, D.~C. and {van der Schaaf}, L. and {van Heijningen}, J.~V. and {van Veggel}, A.~A. and {Vardaro}, M. and {Vass}, S. and {Vas{\'u}th}, M. and {Vaulin}, R. and {Vecchio}, A. and {Vedovato}, G. and {Veitch}, J. and {Veitch}, P.~J. and {Venkateswara}, K. and {Verkindt}, D. and {Vetrano}, F. and {Vicer{\'e}}, A. and {Vinciguerra}, S. and {Vine}, D.~J. and {Vinet}, J. -Y. and {Vitale}, S. and {Vo}, T. and {Vocca}, H. and {Vorvick}, C. and {Voss}, D. and {Vousden}, W.~D. and {Vyatchanin}, S.~P. and {Wade}, A.~R. and {Wade}, L.~E. and {Wade}, M. and {Waldman}, S.~J. and {Walker}, M. and {Wallace}, L. and {Walsh}, S. and {Wang}, G. and {Wang}, H. and {Wang}, M. and {Wang}, X. and {Wang}, Y. and {Ward}, H. and {Ward}, R.~L. and {Warner}, J. and {Was}, M. and {Weaver}, B. and {Wei}, L. -W. and {Weinert}, M. and {Weinstein}, A.~J. and {Weiss}, R. and {Welborn}, T. and {Wen}, L. and {We{\ss}els}, P. and {Westphal}, T. and {Wette}, K. and {Whelan}, J.~T. and {Whitcomb}, S.~E. and {White}, D.~J. and {Whiting}, B.~F. and {Wiesner}, K. and {Wilkinson}, C. and {Willems}, P.~A. and {Williams}, L. and {Williams}, R.~D. and {Williamson}, A.~R. and {Willis}, J.~L. and {Willke}, B. and {Wimmer}, M.~H. and {Winkelmann}, L. and {Winkler}, W. and {Wipf}, C.~C. and {Wiseman}, A.~G. and {Wittel}, H. and {Woan}, G. and {Worden}, J. and {Wright}, J.~L. and {Wu}, G. and {Yablon}, J. and {Yakushin}, I. and {Yam}, W. and {Yamamoto}, H. and {Yancey}, C.~C. and {Yap}, M.~J. and {Yu}, H. and {Yvert}, M. and {Zadro{\.Z}ny}, A. and {Zangrando}, L. and {Zanolin}, M. and {Zendri}, J. -P. and {Zevin}, M. and {Zhang}, F. and {Zhang}, L. and {Zhang}, M. and {Zhang}, Y. and {Zhao}, C. and {Zhou}, M. and {Zhou}, Z. and {Zhu}, X.~J. and {Zucker}, M.~E. and {Zuraw}, S.~E. and {Zweizig}, J. and {LIGO Scientific Collaboration} and {Virgo Collaboration}},
        title = "{Observation of Gravitational Waves from a Binary Black Hole Merger}",
      journal = {\prl},
     keywords = {General Relativity and Quantum Cosmology, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = feb,
       volume = {116},
       number = {6},
          eid = {061102},
        pages = {061102},
          doi = {10.1103/PhysRevLett.116.061102},
archivePrefix = {arXiv},
       eprint = {1602.03837},
 primaryClass = {gr-qc},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016PhRvL.116f1102A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bj,
       author = {{Bailer-Jones}, C.~A.~L. and {Rybizki}, J. and {Fouesneau}, M. and {Demleitner}, M. and {Andrae}, R.},
        title = "{Estimating distances from parallaxes. V: Geometric and photogeometric distances to 1.47 billion stars in Gaia Early Data Release 3}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.05220},
        pages = {arXiv:2012.05220},
archivePrefix = {arXiv},
       eprint = {2012.05220},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201205220B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shultz15,
       author = {{Shultz}, M. and {Wade}, G.~A. and {Alecian}, E. and {BinaMIcS Collaboration}},
        title = "{Detection of magnetic fields in both B-type components of the {\ensuremath{\in}} Lupi system: a new constraint on the origin of fossil fields?}",
      journal = {\mnras},
     keywords = {binaries: close, stars: early-type, stars: individual: {\ensuremath{\in}} Lupi, stars: magnetic field, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = nov,
       volume = {454},
       number = {1},
        pages = {L1-L5},
          doi = {10.1093/mnrasl/slv096},
archivePrefix = {arXiv},
       eprint = {1507.05084},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.454L...1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{doula,
       author = {{Ud-Doula}, Asif and {Owocki}, Stanley P. and {Townsend}, Richard H.~D.},
        title = "{Dynamical simulations of magnetically channelled line-driven stellar winds - II. The effects of field-aligned rotation}",
      journal = {\mnras},
     keywords = {MHD, stars: early-type, stars: magnetic fields, stars: mass-loss, stars: rotation, stars: winds, outflows, Astrophysics},
         year = 2008,
        month = mar,
       volume = {385},
       number = {1},
        pages = {97-108},
          doi = {10.1111/j.1365-2966.2008.12840.x},
archivePrefix = {arXiv},
       eprint = {0712.2780},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.385...97U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heavybh,
       author = {{Petit}, V. and {Keszthelyi}, Z. and {MacInnis}, R. and {Cohen}, D.~H. and {Townsend}, R.~H.~D. and {Wade}, G.~A. and {Thomas}, S.~L. and {Owocki}, S.~P. and {Puls}, J. and {ud-Doula}, A.},
        title = "{Magnetic massive stars as progenitors of `heavy' stellar-mass black holes}",
      journal = {\mnras},
     keywords = {stars: black holes, stars: early-type, stars: evolution, stars: magnetic field, stars: massive, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {466},
       number = {1},
        pages = {1052-1060},
          doi = {10.1093/mnras/stw3126},
archivePrefix = {arXiv},
       eprint = {1611.08964},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.1052P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shultz19,
       author = {{Shultz}, M.~E. and {Johnston}, C. and {Labadie-Bartz}, J. and {Petit}, V. and {David-Uraz}, A. and {Kochukhov}, {\O}. and {Wade}, G.~A. and {Pepper}, J. and {Stassun}, K.~G. and {Rodriguez}, J.~E. and {Lund}, M.~B. and {James}, D.~J.},
        title = "{MOBSTER - III. HD 62658: a magnetic Bp star in an eclipsing binary with a non-magnetic `identical twin'}",
      journal = {\mnras},
     keywords = {binaries: eclipsing, stars: chemically peculiar, stars: early-type, stars: individual: HD 62658, stars: magnetic field, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = dec,
       volume = {490},
       number = {3},
        pages = {4154-4165},
          doi = {10.1093/mnras/stz2846},
archivePrefix = {arXiv},
       eprint = {1910.02928},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.490.4154S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{domnat,
       author = {{Bowman}, Dominic M. and {Burssens}, Siemen and {Pedersen}, May G. and {Johnston}, Cole and {Aerts}, Conny and {Buysschaert}, Bram and {Michielsen}, Mathias and {Tkachenko}, Andrew and {Rogers}, Tamara M. and {Edelmann}, Philipp V.~F. and {Ratnasingam}, Rathish P. and {Sim{\'o}n-D{\'\i}az}, Sergio and {Castro}, Norberto and {Moravveji}, Ehsan and {Pope}, Benjamin J.~S. and {White}, Timothy R. and {De Cat}, Peter},
        title = "{Low-frequency gravity waves in blue supergiants revealed by high-precision space photometry}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = may,
       volume = {3},
        pages = {760-765},
          doi = {10.1038/s41550-019-0768-1},
archivePrefix = {arXiv},
       eprint = {1905.02120},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NatAs...3..760B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{domaa2020,
       author = {{Bowman}, D.~M. and {Burssens}, S. and {Sim{\'o}n-D{\'\i}az}, S. and {Edelmann}, P.~V.~F. and {Rogers}, T.~M. and {Horst}, L. and {R{\"o}pke}, F.~K. and {Aerts}, C.},
        title = "{Photometric detection of internal gravity waves in upper main-sequence stars. II. Combined TESS photometry and high-resolution spectroscopy}",
      journal = {\aap},
     keywords = {asteroseismology, stars: early-type, stars: oscillations, stars: evolution, stars: rotation, stars: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = aug,
       volume = {640},
          eid = {A36},
        pages = {A36},
          doi = {10.1051/0004-6361/202038224},
archivePrefix = {arXiv},
       eprint = {2006.03012},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...640A..36B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{deem,
       author = {{Deeming}, T.~J.},
        title = "{Fourier Analysis with Unequally-Spaced Data}",
      journal = {\apss},
         year = 1975,
        month = aug,
       volume = {36},
       number = {1},
        pages = {137-158},
          doi = {10.1007/BF00681947},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1975Ap&SS..36..137D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kurtz,
       author = {{Kurtz}, D.~W.},
        title = "{An algorithm for significantly reducing the time necessary to computea Discrete Fourier Transform periodogram of unequally spaced data.}",
      journal = {\mnras},
     keywords = {Algorithms, Fourier Transformation, Run Time (Computers), Stellar Oscillations, Discrete Functions, Fortran, Frequency Distribution, Light Curve, Astronomy},
         year = 1985,
        month = apr,
       volume = {213},
        pages = {773-776},
          doi = {10.1093/mnras/213.4.773},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985MNRAS.213..773K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{jenk,
       author = {{Jenkins}, Jon M. and {Twicken}, Joseph D. and {McCauliff}, Sean and {Campbell}, Jennifer and {Sanderfer}, Dwight and {Lung}, David and {Mansouri-Samani}, Masoud and {Girouard}, Forrest and {Tenenbaum}, Peter and {Klaus}, Todd and {Smith}, Jeffrey C. and {Caldwell}, Douglas A. and {Chacon}, A.~D. and {Henze}, Christopher and {Heiges}, Cory and {Latham}, David W. and {Morgan}, Edward and {Swade}, Daryl and {Rinehart}, Stephen and {Vanderspek}, Roland},
        title = "{The TESS science processing operations center}",
    booktitle = {Software and Cyberinfrastructure for Astronomy IV},
         year = 2016,
       editor = {{Chiozzi}, Gianluca and {Guzman}, Juan C.},
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {9913},
        month = aug,
          eid = {99133E},
        pages = {99133E},
          doi = {10.1117/12.2233418},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016SPIE.9913E..3EJ},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dr3,
       author = {{Bailer-Jones}, C.~A.~L. and {Rybizki}, J. and {Fouesneau}, M. and {Demleitner}, M. and {Andrae}, R.},
        title = "{Estimating distances from parallaxes. V: Geometric and photogeometric distances to 1.47 billion stars in Gaia Early Data Release 3}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.05220},
        pages = {arXiv:2012.05220},
archivePrefix = {arXiv},
       eprint = {2012.05220},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201205220B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cp70,
       author = {{Catchpole}, R.~M. and {Feast}, M.~W.},
        title = "{Nebulosities ejected from the star HD 148937}",
      journal = {The Observatory},
         year = 1970,
        month = aug,
       volume = {90},
        pages = {136-141},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1970Obs....90..136C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{vlti,
       author = {{Haguenauer}, Pierre and {Alonso}, Jaime and {Bourget}, Pierre and
         {Brillant}, Stephane and {Gitton}, Philippe and {Guisard}, Stephane and
         {Poupar}, S{\'e}bastien and {Schuhler}, Nicolas and {Abuter}, Roberto and
         {Andolfato}, Luigi and {Blanchard}, Guillaume and
         {Berger}, Jean-Philippe and {Cortes}, Angela and
         {D{\'e}rie}, Fr{\'e}d{\'e}ric and {Delplancke}, Fran{\c{c}}oise and
         {Di Lieto}, Nicola and {Dupuy}, Christophe and {Gilli}, Bruno and
         {Glindemann}, Andreas and {Guniat}, Serge and {Huedepohl}, Gerhard and
         {Kaufer}, Andreas and {Le Bouquin}, Jean-Baptiste and
         {L{\'e}vque}, Samuel and {M{\'e}nardi}, Serge and {M{\'e}rand
        }, Antoine and {Morel}, Sebastien and {Percheron}, Isabelle and
         {Phan Duc}, Than and {Pino}, Andres and {Ramirez}, Andres and
         {Rengaswamy}, Sridharan and {Richichi}, Andrea and {Rivinius}, Thomas and
         {Sahlmann}, Johannes and {Schoeller}, Markus and {Schmid}, Christian and
         {Stefl}, Stan and {Valdes}, Guillermo and {van Belle}, Gerard and
         {Wehner}, Stefan and {Wittkowski}, Markus},
        title = "{The very large telescope Interferometer: 2010 edition}",
    booktitle = {\procspie},
         year = 2010,
       series = {Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series},
       volume = {7734},
        month = jul,
          eid = {773404},
        pages = {773404},
          doi = {10.1117/12.857070},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010SPIE.7734E..04H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{pionier,
       author = {{Le Bouquin}, J. -B. and {Berger}, J. -P. and {Lazareff}, B. and
         {Zins}, G. and {Haguenauer}, P. and {Jocou}, L. and {Kern}, P. and
         {Millan-Gabet}, R. and {Traub}, W. and {Absil}, O. and
         {Augereau}, J. -C. and {Benisty}, M. and {Blind}, N. and {Bonfils}, X. and
         {Bourget}, P. and {Delboulbe}, A. and {Feautrier}, P. and
         {Germain}, M. and {Gitton}, P. and {Gillier}, D. and {Kiekebusch}, M. and
         {Kluska}, J. and {Knudstrup}, J. and {Labeye}, P. and {Lizon}, J. -L. and
         {Monin}, J. -L. and {Magnard}, Y. and {Malbet}, F. and {Maurel}, D. and
         {M{\'e}nard}, F. and {Micallef}, M. and {Michaud}, L. and
         {Montagnier}, G. and {Morel}, S. and {Moulin}, T. and {Perraut}, K. and
         {Popovic}, D. and {Rabou}, P. and {Rochat}, S. and {Rojas}, C. and
         {Roussel}, F. and {Roux}, A. and {Stadler}, E. and {Stefl}, S. and
         {Tatulli}, E. and {Ventura}, N.},
        title = "{PIONIER: a 4-telescope visitor instrument at VLTI}",
      journal = {\aap},
     keywords = {instrumentation: interferometers, techniques: interferometric, techniques: high angular resolution, instrumentation: high angular resolution, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = nov,
       volume = {535},
          eid = {A67},
        pages = {A67},
          doi = {10.1051/0004-6361/201117586},
archivePrefix = {arXiv},
       eprint = {1109.1918},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...535A..67L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@misc{tth, note = "The package is TTH, available at
http://hutchinson.belmont.ma.us/tth/ ."}

@misc{use2e, note = "As the mark-up of the \TeX\ source for this
document makes clear, your file should be coded in \LaTeX
2${\varepsilon}$, not \LaTeX\ 2.09 or an earlier release.  Also,
please use the \texttt{article} document class."}

@misc{inclme, note="Among whom are the author of this document.  The
``real'' references and notes contained herein were compiled using
B{\small{IB}}\TeX\ from the sample .bib file \texttt{scibib.bib}, the style
package \texttt{scicite.sty}, and the bibliography style file
\texttt{Science.bst}."}


@misc{nattex, note="One of the equation editors we use, Equation Magic
(MicroPress Inc., Forest Hills, NY; http://www.micropress-inc.com/),
interprets native \TeX\ source code and generates an equation as an
OLE picture object that can then be cut and pasted directly into Word.
This editor, however, does not handle \LaTeX\ environments (such as
\texttt{\{array\}} or \texttt{\{eqnarray\}}); it can interpret only
\TeX\ codes.  Thus, when there's a choice, we ask that you avoid these
\LaTeX\ calls in displayed math --- for example, that you use the
\TeX\ \verb+\matrix+ command for ordinary matrices, rather than the
\LaTeX\ \texttt{\{array\}} environment."}









